PIT: Optimization of Dynamic Sparse Deep Learning Models via Permutation Invariant Transformation

Dynamic sparsity, where the sparsity patterns are unknown until runtime, poses a significant challenge to deep learning. The state-of-the-art sparsity-aware deep learning solutions are restricted to pre-defined, static sparsity patterns due to significant overheads associated with preprocessing. Efficient execution of dynamic sparse computation often faces the misalignment between the GPU-friendly tile configuration for efficient execution and the sparsity-aware tile shape that minimizes coverage wastes (non-zero values in tensor). In this paper, we propose PIT, a deep-learning compiler for dynamic sparsity. PIT proposes a novel tiling mechanism that leverages Permutation Invariant Transformation (PIT), a mathematically proven property, to transform multiple sparsely located micro-tiles into a GPU-efficient dense tile without changing the computation results, thus achieving both high GPU utilization and low coverage waste. Given a model, PIT first finds feasible PIT rules for all its operators and generates efficient GPU kernels accordingly. At runtime, with the novel SRead and SWrite primitives, PIT rules can be executed extremely fast to support dynamic sparsity in an online manner. Extensive evaluation on diverse models shows that PIT can accelerate dynamic sparsity computation by up to 5.9x (average 2.43x) over state-of-the-art compilers.

==> Design2.tex <==
\subsection{PIT Transformation Mechanism} \label{sec:pitmechanism}

To achieve efficient execution of sparse operators, the key lies in transforming sparse computation into hardware-favored computation units while aligning the transformation with hardware. Before delving into the detailed design, we clarify the hardware abstraction on which the design relies. \sysname{} abstracts hardware accelerators as multi-level hierarchical devices. Each level has local memory for processing units, with the local memory of higher levels being much faster than that of lower levels. To efficiently process an operator, data is loaded from a lower level of memory to the local memory of a higher level processor and consumed by the processors. For example, we can abstract an NVIDIA GPU as a two-level hierarchical device, with level-1 being the GPU global memory and level-0 being the on-chip shared memory in an SM.

Each level of a hierarchical device has its granularity. For instance, the granularity of global memory is the size of read/write transactions, while the granularity of processors is an SM. However, due to the diverse and irregular nature of sparsity patterns, aligning them with accelerator granularities is challenging. Therefore, we introduce the micro-tile abstraction to bridge the gap between sparse computation and accelerator granularity.
%Hardware accelerators typically have multiple levels of memory hierarchies, with the higher memory hierarchies  being closer to the processing unit and faster. For efficient computation, tensor program compilation uses tiling to partition the computation into hardware-friendly small computation tiles. Each tile loads data from lower-level memory to higher-level memory and reuses it during computation to better saturate the processing units~\cite{tvm,zheng2020ansor,flextensor,roller}. Tiling is natural to dense computation because all the input tensors are continuous and dense. However, tiling sparse computation into hardware-friendly tiles is quite challenging(\S\ref{sec:motivation}).

% In dense computations, aligning each tile's computation with hardware-friendly computations is straightforward due to the continuous and dense nature of the data. However, sparse computation breaks such 

% As described in \S~\ref{subsec:motivation:tiling}, the key of efficient computation on hardware accelerators is to align with the hierarchy of the devices including the memory and the computation units.
% To align with the hierarchy, tile-based scheduling is widely used in tensor program compilation to saturate the high throughput higher level processors by reusing the data loaded in the local memory of higher level processors \cite{tvm,zheng2020ansor,flextensor,roller}. This is natural to dense tensor computation as the data is continuous and aligns with the tile-based computation paradigm.
%However, sparse tensor computation breaks the tile-based scheduling because the data is sparse and is hard to align with the concept of tiles, resulting in misalignment with the requirements of memory accessing and computation.

% \paragraph{Micro-Tile}
% Tiling is efficient for dense computation because the input data is dense and cont

%Traditional tensor compilation utilizes tiling to partition operators into hardware-friendly computation tiles, which is a natural approach given that the input data is continuous and dense. However, sparsity presents new challenges for tiling. As illustrated in \autoref{dilemma}, we observe that both sparsity-granularity aligned tiles and traditional GPU-friendly tiles are inefficient in dealing with dynamic sparsity (\S\ref{dilemma}).
%We find that reorganizing the sparse tensor at a certain granularity can both prevent wasteful computation and enable alignment with GPU-friendly computations. We define the granularity of restructuring sparse tensors as ``micro-tile''. The transformation of rearranging micro-tiles that allows performing efficient dense computation without affecting the correctness is PIT transformation. For example, the micro-tile in \autoref{fig:overview} is $1\times4$ and the PIT transformation used is an axis-wise PIT transformation policy(detailed in section\ref{sec:pit_policy}). 

\para{The micro-tile abstraction.}
Efficient computation depends on hardware-favored computation units, such as a tile of a well-optimized dense operator kernel or a tile based on sparse tensor core~\cite{}. A computation unit has a corresponding data format for its input and output tensors. For instance, a tile of a dense operator operates on dense matrices of a specific shape. Micro-tile establishes the mapping from sparse data to the data format of the computation unit. First, a micro-tile does not adhere to the granularity of the sparse data. Second, a micro-tile should align with the granularity of memory read/write (\ie read/write transaction which is 32 bytes for CUDA GPU). An example is shown on the right of \autoref{fig:overview}, where the input tensor has non-zero values in granularities of 1x1, 1x2, 1x3, and 1x4, while the size of the micro-tile is 1x4. The non-zero values are covered by the 1x4 micro-tiles.

\begin{figure} [t]
\centering
\begin{minted}[
breaklines=true,
frame=lines,
fontsize=\small,
linenos=true,
xleftmargin=2em,
escapeinside=!!
]{python}
class MicroTiledOp:
    input_microtile_size   # 1x4
    output_microtile_size  # None
    input_format     # 4x4 dense
    output_format    # 4x4 dense
    computation_unit # 4x4x4 dense tile
    def generate_kernel()
\end{minted}
%\vspace{-0.5cm}
\caption{The definition of micro-tiles for an operator. The comments are the values of those attributes for the example micro-tile on the right of \autoref{fig:overview}.}
\label{fig:stile}
\end{figure}

\autoref{fig:stile} illustrates the micro-tile definition of an operator. It encompasses the micro-tile sizes for the operator's input/output and the computation unit to which the micro-tiles are mapped. The attributes \texttt{input\_format} and \texttt{output\_format} represent the data format of the input(s) and output for \texttt{computation\_unit}. \texttt{computation\_unit} should be an efficient implementation of the operator, which is usually a dense tile. The micro-tiles are rearranged to the required data format through two primitives \sload{} and \swrite{}.

% Hardware accelerators typically have multiple levels of memory hierarchies, with the higher memory hierarchies  being closer to the processing unit and faster. The PIT transformation is performed when loading or storing data across memory hierarchies at the granularity of micro-tiles and will not introduce extra memory access overhead.
% Specifically, PIT transformation constructs the mapping relationship between micro-tiles at different memory hierarchies. Taking the axis-wise PIT transformation in \autoref{fig:overview} as an example, micro-tiles in the input tensor (global memory) are mapped one-to-one to corresponding micro-tiles in shared memory along the first axis. 
% The PIT transform maps micro-tiles from lower memory hierarchies to higher ones and rearranges them in the required format of the efficient dense computation tiles. The dense computation tile performs calculations in the higher memory hierarchy transparently without being aware of the actual position of loaded micro-tiles in the original sparse tensor. PIT transformation needs to ensure that the calculation before and after the transformation is mathematically equivalent and different operators need different PIT transformations. We have derived a set of PIT transformation policies for commonly used operators in deep learning(\S\ref{sec:pit_policy}).
% Micro-tile and PIT transformation decouple the data and computation in the sparse computation optimization and provide a new sparse computation paradigm: on-the-fly data rearrangement combined with efficient dense computation. The computation operates on dense data without traditional sparse indexes, which greatly improves the computation efficiency.
% Then dense computation tile performs the calculation on the r
% Different operators may have different PIT transformations. 
\begin{figure} [t]
\centering

\begin{minted}[
breaklines=true,
frame=lines,
fontsize=\small,
linenos=true,
xleftmargin=2em,
escapeinside=!!
]{c}
/*Generated Sparse Kernel*/
__global__ void SparseKernel( !\label{line:sparsekernel}!
    struct SparseTensors Inputs, 
    struct Tensor Output
){
    /* size and format of SinDense, SoutDense
       in shared memory are decided by
       DenseComputeTile
    */
    DeclareSharedMem(SinDense, SoutDense);
    SRead(Inputs, SinDense, blockIdx); 
    ComputationUnit(SinDense, SoutDense); !\label{line:densecomp}!
    SWrite(SoutDense, Output, blockIdx);
}
\end{minted}
\vspace{-0.5cm}
\caption{\sload{} and \swrite{} primitives and generated kernel example.}
\label{fig:stile_kernel}
\end{figure}

\paragraph{\sload{} and \swrite{}}
In contrast to dense tensor computations, where data tiles are loaded, processed, and stored continuously, the \sysname{} generated sparse kernel employs \sload{} and \swrite{} primitives to handle sparse data at the micro-tile level. Specifically, \sload{} retrieves scattered data in micro-tiles from lower-level memory and places them contiguously in higher-level local memory. Conversely, \swrite{} writes computed results back to lower-level memory at discrete addresses, as illustrated on the right of \autoref{fig:overview}. The data rearrangement is piggybacked on the data movement across different memory levels, resulting in no additional overhead and eliminating the need for traditional data rearrangement outside the sparse kernel (e.g., constructing CSR format for a sparse kernel).

\autoref{fig:stile_kernel} illustrates the template of the kernel generated by \sysname{}. The kernel consists of two phases: data management using \sload{} and \swrite{}, and the computation unit. Both \sload{} and \swrite{} depend on the online constructed index (\texttt{blockIdx}) for data rearrangement, which will be demonstrated in \S\ref{sec:fast_index}. This design effectively separates data encoding/decoding and computation in the sparse kernel, introducing a novel sparse computation paradigm that combines data rearrangement with a (dense) computation unit. Since the computation unit is small, it is feasible to assemble different computation units within the same sparse kernel to handle more intricate sparse patterns and achieve greater efficiency. We leave it in future work.
%The decoupled computation is performed on dense data in higher level local memory, eliminating the overhead of sparse index encoding and decoding.
%Because the Micro-Tile aligns with memory transactions(32 bytes for CUDA GPU), the \sload{} and the \swrite{} can efficiently load and store the sparse data in the Micro-Tile granularity.
% To perform the PIT transformation efficiently, we propose two memory primitives for the sparse kernel generator, namely \sload{} and \swrite{}.
% \autoref{fig:stile_kernel} shows the usage of \sload{} and \swrite{}(Line~\ref{line:sload}) and an example of generated sparse kernel(Line~\ref{line:sparsekernel}).
% As long as the size of Micro-Tile can fill a memory transaction(32 bytes for CUDA GPUs), \sload{} and \swrite{} can also saturate the memory bandwidth achieving the same performance as loading or writing dense data blocks.
% Additionally, \sload{} and \swrite{} further enable zero-copy of sparse data (\S\ref{sec:fast_index}). Because the required data blocks for computation can be directly loaded from the original Tensor into shared memory via \sload{}, no additional operator is required to transform the input Tensor format. 

%To bridge the gap between the sparse data and the hardware-friendly tile-based computation, \sysname{} proposes the abstraction of \textit{Micro-Tile}. There is a granularity that, if used to reorganize sparse tensors, can both prevent wasteful computation and enable alignment with GPU-friendly computations. We define such granularity as Micro-Tile. 
%In \sysname{}, the sparse tensor will be reassembled at the granularity of Micro-Tile. As shown in \autoref{fig:overview}, the sparse tensor is reorganized at the granularity of Micro-Tile($1\times4$).
%In \sysname{}, Micro-Tile is the minimum contiguous data unit and the sparse tensor will be reassembled at the granularity of Micro-Tile. For example, the Micro-Tile in \autoref{fig:overview} is $1\times4$.  %As long as the size of Micro-Tile can fill a memory transaction(32 bytes for CUDA GPUs), the cost of rearranging the sparse tensor into Micro-Tiles can be negligible(\S\ref{}).  
%As shown in \autoref{fig:overview}, assume we have an efficient and hardware-aligned 4x4 computational tile. If we rearrange the sparse tensor with a granularity of 1x4, we can achieve low computational waste and high efficiency.

\begin{comment}
\paragraph{\stile{}}
\stile{} is the hardware-friendly sparse computation tile built on Micro-Tiles. The right side of \autoref{fig:overview} shows an example of \stile{} generated by \sysname{}. \stile{} is composed of Micro-Tiles, PIT Transformation, and corresponding efficient computation tile. During the operation of \stile{}, sparse data is loaded from the lower memory hierarchy in Micro-Tile granularity and placed in the higher memory hierarchy according to the PIT transformation. The transformation that rearranges the discrete Micro-tiles from the lower memory hierarchy to the higher hierarchy and allows to perform dense computation without affecting the correctness is PIT Transformation. After the PIT transformation, we can align sparse data to the format required by the efficient dense computation tile. Then the dense computation tile in \stile{} performs the calculation in the higher memory hierarchy(shared memory in CUDA GPU) without the sparse data encoding and decoding overhead. The computation results are stored back in the lower memory hierarchy as Micro-Tiles. Therefore, Micro-Tile and \stile{} allow us to align the sparse computation to efficient dense computation, providing a new sparse computation paradigm: on-the-fly data rearrangement combined with efficient dense computation.

\paragraph{\sload{} and \swrite{}}
To leverage PIT Transformation and achieve efficient online dynamic data rearrangement, we propose two memory access primitives, namely \sload{} and \swrite{}. Specifically, \sload{} loads the scattered Micro-Tiles from the lower memory hierarchy and places them in the higher memory hierarchy according to the PIT transformation policy, while \swrite{} reverses the process by writing the computed results back to the lower memory hierarchy as discrete Micro-Tiles, as shown in \autoref{fig:overview}. \stile{} uses \sload{} and \swrite{} to efficiently apply the PIT transformation for data rearrangement. \sload{} and \swrite{} fuse the process of data rearrangement into the cross-memory-hierarchy data loading (e.g., from Global memory to shared memory) or writing, thus introducing almost no extra overhead. As long as the size of Micro-Tile can fill a memory transaction(32 bytes for CUDA GPUs), \sload{} and \swrite{} can also saturate the memory bandwidth achieving the same performance as loading or writing dense data blocks.
Additionally, \sload{} and \swrite{} further enable zero-copy of sparse data (\S\ref{sec:fast_index}). Because the required data blocks for computation can be directly loaded from the original Tensor into shared memory via \sload{}, no additional operator is required to transform the input Tensor format. \autoref{fig:stile_kernel} shows the kernel skeleton of \stile{} based on \sload{} and \swrite{} in \sysname{}.
\end{comment}

\begin{comment}
\begin{figure} [t]
\centering
\begin{minted}[
breaklines=true,
frame=lines,
fontsize=\footnotesize,
linenos=true,
xleftmargin=2em,
escapeinside=!!
]{python}
class STile:
    class stile_config:
        micro_tile_shape
        pit_trans_func
    expr # operator expression
    def SRead()
    def Compute()
    def SWrite()
\end{minted}
\vspace{-0.5cm}
\caption{The definition of \stile{}.}
\label{fig:stile}
\end{figure}


\paragraph{\stile{} and Micro-Tile} 
To bridge the gap between the sparse data and the hardware-friendly tile-based computation, \sysname{} proposes the concepts of \textit{Micro-Tile} and \textit{Sparse-Tile} (STile). 
Specifically, the Micro-Tile is defined as the minimal continuous data unit that aligns with the requirements of memory accessing and also provides the capability of aligning with the tile-based computation. In \sysname{}, the sparse data patterns should be organized in the granularity of Micro-Tiles.
\stile{} is defined as a group of Micro-Tiles so that it is a dense computation tile in logic for efficient tile-based computation but its data is stored in the granularity of Micro-Tiles in lower level memory.

When processing a \stile{}, the sparse data is loaded in the granularity of Micro-Tiles from lower level memory to a continuous dense tile in higher level local memory for tile-based computation. The tiles constructed in the local memory are the same as tiles in dense tensor computation. Then, the computed results are stored back to the lower level memory as Micro-Tiles.
Therefore, the concepts of \stile{} and Micro-Tile enable aligning sparse computation with the hierarchy of hardware accelerators for efficient computation.


%Specifically, \stile{} is defined as the data unit that stores sparse data but can be processed as efficient as tiles in dense tensor computation. To achieve computation efficiency, the key is to make the computation of \stile{} as the tiles in dense tensor computation. To achieve this, the sparse data should be organized as tiles for processing.
%For a processor, instead of loading a continuous data tile from lower level memory to higher level local memory, \stile{}



Figure~\ref{fig:stile} shows the definition and the interfaces of \stile{}. Specifically, \texttt{stile\_config} defines the shape of its Micro-Tile in \texttt{micro\_tile\_shape} and the mapping that describes how a \stile{} is constructed by those Micro-Tiles.
The \texttt{expr} describes the computation of this \stile{} with the operator expression.
The computation of a \stile{} is defined by \texttt{\sload{}}, \texttt{Compute} and \texttt{\swrite{}}. As Figure~\ref{fig:overview} shown, \texttt{\sload{}} loads the Micro-Tiles from lower level memory to a dense tile in the higher level local memory according to the \texttt{stile\_config}. Then, \texttt{Compute} processes the tile as the computation expressed in \texttt{expr}. Then, \texttt{\swrite{}} stores the output tile from higher level local memory to lower level memory as Micro-Tiles according to the \texttt{stile\_config}.

\paragraph{\sload{} and \swrite{}}
Different from dense tensor computation that data tiles are continuously loaded, processed and stored, \stile{} uses the \sload{} and \swrite{} primitives to load and store sparse data in Micro-Tile granularity.
Specifically, \sload{} loads the scattered data represented in Micro-Tile from lower level memory and places them contiguously in higher level local memory, while \swrite{} reverses the process by writing the computed results back to lower level memory at discrete addresses, as shown in \autoref{fig:overview}.

The design of \sload{} and \swrite{} naturally decouples data and computation in sparse computation, providing a new sparse computation paradigm: data rearrangement combined with dense computation.
The decoupled computation is performed on dense data in higher level local memory, eliminating the overhead of sparse index encoding and decoding.
Because the Micro-Tile aligns with memory transactions(32 bytes for CUDA GPU), the \sload{} and the \swrite{} can efficiently load and store the sparse data in the Micro-Tile granularity.

An example: Figure~\ref{fig:}

\end{comment}

% \subsection{PIT Transformation}
% A transformation that rearranges the discrete Micro-tiles from the lower memory hierarchy to the higher hierarchy and allows to perform dense computation without affecting the correctness is PIT Transformation.


%As sparsity continuously changes with input, \sysname{} performs online detection of sparsity and constructs a sparse index. To improve the efficiency of online sparsity detection, we propose an efficient dynamic sparse representation and a mechanism for quickly constructing sparse indexes.




% \paragraph{Sparse Index Construction}
% With \sload{} and \swrite{}, the sparse kernels generated by \sysname{} no longer require the sparse indices to be sorted along a certain axis. This greatly reduces the constraints on building sparse indices, allowing us to construct them with minimal synchronization overhead. For example, in the original BCSR format, the column indices of non-zero elements in the same row had to be sorted, which resulted in significant synchronization overhead, especially on GPU accelerators. However, in \sysname{}, after tiling, each tile only needs to traverse the corresponding region to check for non-zero values and write the unordered column indices to the corresponding position in the row through atomic operations. Therefore, \property{}, \sload{}, and \swrite{} enable \sysname{} to achieve efficient tiling and extremely low synchronization overhead. Furthermore, \sysname{} only builds sparse indices online without copying data. At runtime, sparse kernels use \sload{} to directly read from the original tensor based on the constructed sparse index. This greatly reduces the memory access overhead introduced by data format conversion (from dense to BCSR) and achieves zero-copy data rearrangement.

%The \stile{} abstraction exposes the capability of efficiently processing sparse computation by aligning with the hardware hierarchy. \sysname{} further builds the framework including online sparsity detector that detects the  and just-in-time (JIT) compiler.

%As sparsity continuously changes with input, 

% \subsection{Just-In-Time Compiling}

% For a given sparse pattern with sparse tensor samples, \sysname{} schedules the 


% setmicrotile
% set sp anno




\begin{comment}

# policy
policy(tensor_samples, op_type) -> stile_config
register_policy(policy)

struct micro_tile_config:
    micro_tile size
    dense_tile size

# online sparsity detector
detector.set_micro_tile(micro_tile_config)
detector.set_sparsity_annotation_meta(tensor_itself, auxiliary_sparsity_attr)
online: detector -> index

# sparse kernel generator
generator.set_stile_config(stile_config) -> sparse kernel
generator.gen_code()

# sparse kernel template
op_kernel_template(tensor, index) {
    dtensor = sread(tensor, index)
    dense_tile(dtensor)
    swrite(dtensor, index)
}
\end{comment}


==> Introduction.tex <==
\section{New Outline}

* Deep learning is computation intensive.

* Accelerator with massive parallel units to speed up DL computation.

* DL is computed on tensors. The common approach is to slice tensors into smaller pieces, known as tiles, and each computation unit in the accelerator computes on the tile in parallel.

As different tile shape (the length along each dimension) affects the computation efficiency of each parallel unit, finding a good tile shape becomes a key goal of tensor compilation for DL~\cite{tvm, roller, welder}.

* The above approach assumes critical statistics of input tensors are known at the compile time. 

Unfortunately, recent development of deep learning suggest this assumption is often violated.

% seems like a trivial case * First, the assumption of fixed tensor shape. Tensor shapes often changes over time. (1) e.g., In NLP, the length of a sentence is changing --> Sequence length of the token is changing. (2) Dynamic routing in DNN network, e.g., MoE, makes each expert handle different number of tokens each time.

The assumption of static tensor sparsity pattern. It is either dense or the positions of zeros in the tensor are known at the compile time. This often cannot be true due to 
(1) Dynamic routing in DNN network, e.g., MoE, each expert handles a set of tokens where zeroed tokens exist in some random positions.
(2) dynamic attention 
(3) dynamic pruning.
(4) Changing sparsity pattern due to changing neural architecture.

* Therefore, compile-time generated tile configurations are often suboptimal. Following such offline calculated configurations, the tile constructed at the runtime often contains unforeseen zeros that lead to waste of computation, or simply cannot meet the requirement of the calculated tile shape due to the changing input shape.

* Insights ...

\if 0
\section{Outline}
\YQ{remove this section later.}

**Background:**

In the era of large models, the efficiency of deep learning frameworks is becoming increasingly crucial to enable the scaling of larger models. Tiled computation is a key technique that enables high-efficiency deep neural network (DNN) frameworks. It takes full advantage of hardware acceleration, such as GPUs, which are optimized for processing small, parallelizable computations.

1. Tensor, which is the abstraction of a multi-dimensional array of numeric values, is a fundamental data structure in deep learning frameworks.

2. A tile of data is copied from the original tensor (often in GPU memory) to on-chip memory for high-efficiency kernel computing. The result is then stored back to the same tensor or a new tensor (also in GPU memory).

3. The dimension (axis) of the tile is a continuous portion (slice) of the corresponding dimension (axis) of the original tensor. The slicing relationship is crucial for loading and storing and is determined statically at compile time.

**Problem:**

Unfortunately, the computation efficiency of tiled computation can be largely reduced by redundancy (which is identical to sparsity) inside tensors, which is inevitable and prevalent in deep learning models. \YQ{one concern is that it seems not a new problem}% \NX{Maybe we should explain where such redundancy/sparsity comes from first? it comes from the sub-tensor level algorithm and the tensor-level deep learning infrastructure}

1. Redundant parts of tensors refer to elements that are not used in computations, such as the elements masked out by sparse masks in sparse attentions, and the padding caused by imbalanced sample sequences.

2. Redundancy wastes computation resources, which becomes more significant with larger tile sizes given a specific sparsity ratio.

3. Some redundancy patterns can only be detected at runtime, which can further impact the efficiency of tiled computation. This make the sparsity compiling system, which requires intensive ahead-of-time compiling, no longer workable.

- Many kinds of dynamic routed (activated) NN, exampled by MoE
- Dynamic sequence is also one, because of it’s input dependent
- Some of attention masks are dynamic, especially for the long range transformers (e.g., longformer), and also museformer for music
- Dynamic pruning, exampled by token pruning, can get the rid of the dependence of calibration dataset
- Dynamic sparse training (DST), which trains from a random initialized sparse NN, but change the topology NN during the training (MoE and pathways / PaLM can be thought of DST in some literature)

4. Some number of sparsity ratio (e.g., padding ratio, sparse attention ratio) may need to be added here.

The challenge is to find a way to map the tensor (or computation) to an accelerator that can achieve the following simultaneously:
(a) guarantee the correctness of the operator,
(b) skip redundancy to avoid wasted computation,
(c) keep the compute tile's shape unchanged to guarantee high hardware utilization, and
(d) be suitable for online execution due to dynamic applications.

**insights:**

Our insight on permutation invariant can help. It reveals that some of the tile dimensions (axes) are not necessarily continuous in the corresponding dimensions (axes) of origin tensor.

1. Such properties can be found in various types of operators. 

2. Such property can be formulated and proven.

3. The discontinuous slicing of origin tensor’s dimension can be independently applied to each tile

The permutation invariant property permits the aggregation of elements into efficient compute tiles based on sub-tensor heterogeneity. Permutation invariance along these axes ensures the correctness of such aggregation, while simultaneously skipping extraneous computational steps and maintaining the original compute tile size of dense computation. Therefore, the mapping (SLoad and SStore) achieves the aforementioned goals (1), (2), and (3). For the goal (4), we give an implementation of 1-D aggregation, like BCSR (or BCSC) converting, which can be conducted real time.

**solution:**

The insights imply the feasibility of skipping redundancy parts of the tensor when splitting it into tiles. 

1. We make it by the interface Sload and Sstore.

2. Sload and Sstore are friendly for reusing existing efficient dense computing kernels.

3. Online 1-D Sload and Sstore is implemented by leveraging the format BCSR.

\fi

\section{Introduction}
%Sparsity, especially dynamic sparsity, is the future.

% Sparsity has become the most important and efficient approach to accelerate neural networks by pulling out a large portion of computation without unraveling model accuracy~\cite{}. However, most commodity accelerators (e.g., GPUs and TPUs) are mainly designed for efficient dense computations with thousands of simultaneously active threads (i.e., SPMD~\cite{}) and large off-chip memory bandwidth. To fit sparse computation on these dense computation-efficient accelerators, existing solutions either specialize sparse computation kernels for certain sparsity patterns (\eg fine-grained sparsity or fixed sparsity) in an ahead-of-time manner~\cite{sparta} to alleviate the computation inefficiency, or fall back to more coarse-grained computation (\eg block sparse~\cite{} or dense computation) to align with hardware but with a large proportion of computation waste.

% Sparsity has become the most critical approach to explore for efficiency and scalability in deep learning. 

Sparsity has become the most important and efficient approach to accelerate neural networks by erasing a large portion of computation without unraveling model accuracy~\cite{Hoefler2021SparsityID}. However, most commodity accelerators (e.g., GPUs and TPUs) are mainly designed for efficient dense computations with thousands of simultaneously active threads and large off-chip memory bandwidth. To fit sparse computation on these dense computation-efficient accelerators, previous research works propose sparsity optimizations, which only work for fixed granularities (\eg OpenAI's block sparsity kernels and Sputnik~\cite{sputnik} for fine-grained sparsity)
%for some specific granularities. Such optimization only work for a specific sparsity granularity (\eg Sputnik~\cite{sputnik} for fine-grained sparsity) and 
 and perform badly when the granularity mismatches. The compiler-based approaches leverage time-consuming tuning to find special computation kernels in an ahead-of-time manner (e.g., SparTA~\cite{sparta}), which only works for prior known and fixed sparsity patterns. Although some accelerators have 
special hardware units for sparse computation, they are limited to highly-constrained sparsity rules (\eg 2:4 sparsity in Sparse TensorCore~\cite{choquette2021nvidia}).

\begin{comment}
Sparsity has become the most important and efficient approach to accelerate neural networks by pulling out a large portion of computation without unraveling model accuracy~\cite{Hoefler2021SparsityID}. However, most commodity accelerators (e.g., GPUs and TPUs) are mainly designed for efficient dense computations with thousands of simultaneously active threads and large off-chip memory bandwidth. To fit sparse computation on these dense computation-efficient accelerators, existing solutions have to leverage time-consuming approaches (e.g., SparTA~\cite{sparta}) to tune special computation kernels in an ahead-of-time manner, which only works for prior-known and fixed sparsity patterns. Although some accelerators have 
special units for sparse computation, they are limited to highly-constrained sparsity rules (\eg 2:4 sparsity in Sparse TensorCore~\cite{choquette2021nvidia}).
\end{comment}


% Challenge due to commodity accelerators. Existing solutions have to be limited to static patterns. Missed opportunity for dynamic sparsity. Examples of dynamic sparsity.

However, sparsity in real-world applications is naturally dynamic and diverse. For example, the input sentences of a natural language processing (NLP) model have varied lengths. Many dynamic neural networks conditionally compute the most informative regions, words, or parameters, \eg Mix-of-Expert (MoE)~\cite{shazeer2017outrageously}, Longformer~\cite{longformer}. Sparse training algorithms dynamically drop tokens/image pixels for better accuracy and efficiency~\cite{he2022masked}. All these dynamic sparsity patterns are derived from input data that is only known at runtime. Therefore, it is hard to compile efficient kernels for dynamic sparsity in an ahead-of-time manner due to unknown sparsity patterns or fit with pre-defined sparsity rules due to the diverse inputs. Dynamic and sparse activation has been proven to be an important feature for the biological brain to work efficiently. The more neurons a brain has, the sparser it gets~\cite{herculano2010connectivity}. Therefore, supporting dynamic sparsity is an unavoidable challenge to be solved on the road to Artificial General Intelligence (AGI), which is not well supported by commodity accelerators. %It is still an open problem to efficiently execute dynamic sparse computation with diverse sparsity patterns on commodity accelerators.

%However, sparsity in real-world applications is naturally dynamic and diverse. For example, a batch of sentences has varied lengths and thus pads a different number of zeros in a tensor. Many dynamic neural networks conditionally compute the most informative regions or words~\cite{}. All these dynamic sparsity patterns are derived from input data that is only known at runtime. Therefore, it is impossible to compile efficient kernels for dynamic sparsity in an ahead-of-time manner due to unknown sparsity patterns or fit with pre-defined sparsity rules due to the diverse inputs. It is still an open problem to efficiently execute dynamic sparse computation with arbitrary sparsity patterns on commodity accelerators.


%At its core is a key property we identified for most DL computation, i.e., computation invariance. 
%There exist some dimensions whose computation can be arbitrarily reordered without affecting the correctness of the output. 

In order to bridge the gap between dynamic sparse computation and commodity accelerators, we propose \sysname{} that can transform dynamic sparse computation into equivalent dense computation with extremely low overhead. Therefore, the sparse computation can directly benefit from efficient computation kernels or hardware units (e.g., Tensor Core) for dense computation. 

% introduce sparse-dense equivalence, because of permutation invariant of deep learning operations
% introduce stile, with tiling the effect of permutation invariant is significantly amplified, to produce finer grained irregular sparsity patterns
% the quivalence makes tile's computation into two separated stages: data rearrangement and dense computation
% out-of-order, zero-copy data rearrangement enabled by permutation invariant

The key insight of \sysname{} is an important property we identified for deep learning computations, called \emph{permutation invariant}. It means the values in a tensor can be permuted along a certain dimension(s) while the original computation on the permuted tensor is still mathematically correct. For example, in matrix multiplication (Matmul) whose tensor expression is $C[m,n]$+=$A[m,k]$*$B[k,n]$, the columns of $A$ along with the rows of $B$ (\ie the $k$ dimension) can be permuted to any order without affecting the computation result. The rows of $A$ along with the rows of $C$ (\ie the $m$ dimension) can also be permuted without affecting the computation. Permutation invariant in essence is enabled by two characteristics of the deep learning computations in tensor expression (\eg einsum~\cite{einsum}, TVM~\cite{tvm}): first, the computations of reduction (\eg the $k$ dimension in Matmul) is commutative; second, the computations of the values in an output tensor (\eg $C$ in Matmul) are spatially commutative (\eg along $m$ or $n$ dimension).
Permutation invariant establishes a natural connection between sparse computation and dense computation. For many sparse tensors, it is feasible to compact their non-zero values into a smaller dense tensor with permutation.

\sysname{} exploits the effect of permutation invariant to allow permutation on finer-grained granularity instead of the whole row or column of a tensor (\eg 32x1 instead of 1024x1 for a tensor of size [1024,1024]). This is achieved by combining permutation invariant with computation tiling, a technique widely used in high-performance computation~\cite{RaganKelley2017HalideDA}. By tiling an operator into small pieces of computation (\ie a computation tile), \sysname{} can apply permutation invariant on each computation tile independently. It implies that the sparsity could be more fine-grained and irregular, as long as the non-zero values can be compacted into multiple dense computation tiles. Formally, we define the sparsity pattern of the non-zero values and the compacted computation tile as sparse tile, \ie \stile{}. There are various sparsity patterns in \stile{}s depending on both the feasible permutations of an operator and the size of the computation tile. %Based on systematic study of permutation invariant on deep learning operators, we design \stile{} 

The design of \stile{} naturally splits sparse computation into two decoupled stages: data permutation and dense computation. The decoupling makes the computation stage free from handling the intricate encoding and decoding of sparse tensors, thus, the computation can more efficiently utilize the accelerators (\eg GPU). With the decoupled stages, \sysname{} can leverage a wide range of well-optimized implementation of dense computation, including hardware instructions (\eg TensorCore's wmma~\cite{wmma}), manually optimized kernels (\eg OpenAI's block sparse kernels), and automatically tuned kernels (\eg AutoTVM~\cite{chen2018learning}), which can be easily plugged in \stile{}. The data permutation stage transforms sparse data into a dense format with a new primitive \sload{}. After the computation, the produced dense data is transformed back to the required format (\eg sparse format) with the other primitive \swrite{}.

Dynamic sparsity requires efficient online processing of sparse tensors, as the tensors' sparsity is only known at runtime. The sparsity should be captured online and translated to efficient computation. \sysname{} can construct sparsity index (\eg CSR, BCSR~\cite{sparse_formats}) for the captured sparse tensors efficiently by leveraging permutation invariant. Permutation invariant allows the index to be constructed in an out-of-order manner, eliminating heavy synchronization. The computation is performed following the index, with \stile{}s being constructed online. No additional data conversion and copy are performed, leading to very efficient online processing.
%With \stile{}, the computation is directly applied on the sparse tensors. No additional data conversion is required, because the data permutation happens on-the-fly when the data is moving across different memory hierarchies (\eg global memory to shared memory in GPU). With these optimizations, \sysname{} makes dynamic sparsity almost as efficient as static sparsity.

%With \stile{}, \sysname{} can capture and handle sparsity in an online manner efficiently. First, the property of permutation invariant in \stile{} fully parallelizes the online extraction of sparsity, the sparse index can be constructed and written into a sparse format (\eg CSR, BCSR~\cite{}) in an out-of-order manner, eliminating heavy synchronization across parallel threads. Second, the data permutation in \stile{} happens on-the-fly when the data is moving across different memory hierarchies (\eg global memory to shared memory in GPU). It eliminates the overhead of data copy in the online data conversion (\eg data rearrangement in MoE~\cite{}). Thus, \sysname{} transforms dynamic sparsity with negligible overhead, making dynamic sparsity almost as efficient as static sparsity.

% The key insight of \sysname{} is an important property we identified for most deep learning computations, called \emph{computation invariance}. It builds a special connection between sparse computation and dense computation. With computation invariance, squeezing the non-zero elements of a sparse tensor together into a dense one, the dense computation can be directly applied on it without affecting correctness. It complies two constraints: first, the elements can be reordered without affecting mathematical correctness; second, the reordering achieves the same \textit{computation I/O ratio}~\cite{} as the dense computation. Not arbitrary reordering meets the two requirements, thus, we systematically studied the operators in deep learning and propose a list of rules to identify feasible reordering of different operators that satisfies computation invariance.

% % The key insight of \sysname{} is an important property we identified for most deep learning computation, called \emph{computation invariance}. It reveals the fact that, for most deep learning operators, there exist some dimensions whose computation can be arbitrarily reordered without affecting the correctness. To explain this property, we show a simple example with the multiplication of two 1-D matrixes. 
% % \[ [a_1, ..., a_n] \times [b_1, ..., b_n]^T = [\sum_{i=1}^n a_i*b_i]\] 
% % \begin{multline}\label{eq:1dmm}
% % [a_1, 0, a_3, 0, a_5] \times [b_1, b_2, b_3, b_4, b_5]^T = [a_1b_1 + a_3b_3 + a_5b_5] \\
% % \Rightarrow{} [a_3, a_1, a_5] \times [b_3, b_1, a_5]^T = [a_1b_1+a_3b_3+a_5b_5]
% % \end{multline}
% % The computation invariance happens in the reduction axis, i.e., the computation order of $a_i\cdot b_i$ does not affect the result of summation. Meanwhile, it achieves the same efficiency of dense computation.

% \sysname{} exploits the computation invariance property in two folds. First, \sysname{} applies computation invariance at the granularity of computation tiles to produce various sparse tiles, called \stile{}. Tiling is a common optimization technique in commodity devices such as GPU, which improves computation efficiency by increasing computation I/O ratio~\cite{}. The computation of an operator is tiled into a group of tiles. Similarly, \sysname{} tiles sparse computation into a group of sparse tiles, each of which has the same computation efficiency as its corresponding dense tile. 
% As tile is much smaller than the original computation, \sysname{} enables much finer-grained sparsity granularities, while making them as efficient as dense computation. The special connection between sparse tile and dense tile make it feasible to partition the sparse computation into clearly separated two stages: data rearrangement and dense computation. We propose two primitives \sload{} and \swrite{} to manage the data rearrangement. With them, \sysname{} can simply plug in a wide range of dense computation tiles, including hardware instructions (\eg TensorCore's wmma~\cite{}), manually optimized kernels (\eg OpenAI's block sparse kernels), and automatically tuned kernels (\eg AutoTVM~\cite{}).

% Second, computation invariance makes capturing and handling sparsity in an online manner much more efficient. In dynamic sparsity, tensors' sparsity is only known at runtime. Given an input (or activation) tensor at forward pass, \sysname{} can quickly extract its sparsity pattern to fill into a sparse format (\eg CSR, BCSR~\cite{}). Because of the reordering property in computation invariance, the sparsity index can be constructed in an out-of-order manner, which is much more friendly for accelerators to parallelize threads without heavy synchronization. The index construction further benefits from zero-copy of the non-zero elements, \ie the constructed index can directly reference the non-zero elements stored in the original tensor. This is enabled by the design of \stile{} which does on-the-fly data rearrangement in \sload{} and \swrite{} when data is moving across different memory hierarchies (\eg global memory to shared memory in GPUs). Thus, \sysname{} transforms dynamic sparsity with negligible overhead, making dynamic sparsity almost as efficient as static sparsity.

% % \sysname{} exploits the computation invariance property in two folds. First, different from static sparsity whose pattern is prior given, dynamic sparsity is only known at runtime. Given an input tensor at inference, \sysname{} can quickly extract its sparsity pattern (usually in the form sparse formats like CSR, BSR~\cite{}) in an online manner. Existing approaches builds sparse format usually with a fixed order (e.g., row-major), which has a low SPMD utilization due to order dependency. However, if we know the dimensions that satisfy computation invariance in the following computations. The order of these dimensions in the sparse format can be arbitrary, which is much more friendly for accelerators to parallel process. It allows \sysname{} to extract sparse patterns an order of magnitude faster. Second, when there are zeros in the matrixes, the computation invariance allows \sysname{} to rebuild equivalent dense computation with non-zero values while retaining the correctness of the result. As shown in \autoref{eq:1dmm}, the order of values along the computation invariant dimensions can also be arbitrary in the transformed dense computation, thus providing same efficiency of dense computation for sparse inputs. In \sysname{}, we propose a list of rules to identify computation invariant dimensions for DL operators. We have verified xxx among xxx computation operators in TVM (PrimTorch?) satisfying this property.

% %How can we leverage this property for efficient dynamic sparsity computation? First, different from static sparsity whose pattern is prior given, dynamic sparsity is only known at runtime. We need to quickly extract it from tensors at runtime. How can the property help extraction? Second, with the extracted sparsity patterns of tensors, \sysname{} quickly transforms their sparse computation into the equivalent dense computation, whose computation kernels can be easily found/built on commodity accelerators. How can the property help the transformation?

% % How to build efficient dense kernels suitable for sparse computation? 

% % To transform sparse computation to the most efficient dense computation kernels, \sysname{} manipulates data at the granularity of tiles. \sysname{} introduces a data arrangement format called \emph{\stile{}} that defines a group of data tiles of sparse data, which can be condensed to a predefined dense computation tile. The computation invariance guarantees the data rearrangement of \stile{} preserves the mathematical correctness. \sysname{} supports converting a wide range of dense computation kernels for sparse computation, including hardware instructions (e.g., TensorCore's wmma~\cite{}), manually optimized kernels (e.g., OpenAI's block sparse kernels), and automatically tuned kernels (e.g., AutoTVM~\cite{}).

We have implemented \sysname{} on PyTorch. We extensively evaluate \sysname{} on four representative scenarios and the results show that \sysname{} achieves significant speedup on model inference latency with fewer memory footprints, compared to current state-of-art solutions. Specifically, \sysname{} achieves up to 9.4x speedup on the MoE inference over current state-of-art solutions, up to 3.5x speedup on the NLP model inference by leveraging the dynamic sparsity caused by different sequence lengths, and up to 2.4x speedup on the dynamic sparse model inference. In addition, we also use \sysname{} to speed up sparse training by leveraging the dynamic sparsity and achieve up to 4.6x speedup. Dynamic sparsity is an important trend in deep-learning models. We will open source \sysname{} and hope it will inspire more dynamic sparsity optimization and algorithm research works.

% As the deep-learning models continues to become larger and more complex, sparsity is arguably the most important direction to explore the efficiency and scalability. To better trade off the accuracy and efficiency, the algorithm researchers also develop various sparsity patterns, from the fine-grained pattern~\cite{} to the block-wise pattern~\cite{} and the coarse-grained pattern~\cite{}. Such sparsity patterns are static and fixed for all input data. However, this is contrary to the biological neural network, which is dynamically sparse. In the biological neural network, different input data will activate different regions of brain accordingly. Learned from biological neural networks, deep learning algorithm researchers have proposed lots of dynamic sparsity patterns\cite{wan2013regularization,zehui2019dropattention,rao2021dynamicvit}. In such dynamic sparse models, the sparsity pattern of the model will change according to input data to achieve better accuracy with a smaller memory footprint and lower computation. For example, Figure~\ref{fig:longformer} shows the sparsity pattern of the Longformer\cite{}. As shown in the Figure,the yellow blocks means the static attention window and the green ones are the dynamic global attention whose position is determined online based on the input. \NX{maybe need one more example?}

% \begin{figure}[htbp]
% 	\centering
% 	\includegraphics[width=0.3\columnwidth]{Figure/longformer.pdf}
% 	\caption{\label{fig:longformer}Sparsity pattern of the Longformer.}
% \end{figure}


% % mention other potential scenarios
% In addition to the dynamic sparse algorithm mentioned above, there are actually many other scenarios with potential dynamic sparsity. For example, during the model pruning, pruning algorithm generates a mask for weights based on the current states of the model. By multiplying the weight by mask, pruning algorithms simulate the pruning behaviour. Such simulation fails to leverage the sparsity generated by the pruning algorithm and even slow down the original pruning progress. Even if there is a large amount of sparsity during the pruning progress, such sparsity are hard to be leveraged. Because at each iteration during the pruning, the position of mask may change over time. Therefor dynamic sparsity are widely existed in current deep-learning models and we will give more examples that have potential dynamic sparsity in Section~\ref{sec:eval}.
% \NX{Describe other potential scenarios: such as nnpruning and sequence length.}

% Unfortunately, current deep-learning systems are not effective in exploiting such dynamic sparsity. First, the performance of general sparse library such as cuSparse~\cite{} is far from optimal. Because the dynamic sparse pattern is constantly changing, we need re-build the sparse indexes based on current sparse pattern each time. Table shows the performance of cuSparse with different sparsity ratios under the shape of $1024\times1024\times1024$, where the $Convert$ means the time overhead of sparse index construction, and $SPMM$ represents the matrix multiplication time. The latency of cuBlas(dense computation) of matrix multiplication with the same shape is xxxus. As shown in the table, the convert overhead is non-negligible and cuSparse can be faster than dense computation only when the sparsity ratio is higher than xx.xx\%.
% In contrast to the general sparse library, previous works~\cite{sparta,sparsetir,sputnik} propose to specialize sparse kernels according to given sparsity to achieve better performance. However, such specialization is usually time-consuming and will be invalid once the sparsity pattern changes. Therefore such specialization based sparsity optimization is not applicable to dynamic sparsity.

% Therefore we propose \sysname{}, a new dynamic sparsity optimization framework. \NX{Brief introdution of \sysname{} design here}.

% \begin{table}%[htbp]
%     \small
% 	\caption{Speed of sparse matrix multiplication(SPMM) and sparse index construction(Convert) ($1024\times1024\times1024$) in cuSPARSE on NVIDIA A100 (unit: us).}
% 	\vspace{-0.5cm}
% 	\label{tab:cusparse}
% 	\begin{center}
% 		%\scriptsize
% 		\begin{tabular}{c|c|c|c|c}
% 			\hline
% 			Sparsity Ratio & 50\% & 90\% & 95\% & 99\% \\
% 			\hline
% 			Convert &  &  &  &  \\
% 			%\hline
% 			SPMM &  &  &  &  \\
% 			\hline
% 		\end{tabular}
% 	\end{center}
% 	\vspace{-0.6cm}
% \end{table}

==> Motivation.tex <==
\section{Background and Motivation}\label{sec:moti}

\para{Sparse computations in modern deep learning networks are irregular and dynamic.}
% 1) implicit redundant computations, e.g., sparse activation tensors. 2) the intrinsic dynamics in LLM inference.
Deep learning networks commonly exhibit sparsity, especially in modern large language models (LLMs) which consist of Feed Forward Network (FFN) and multi-head attention (MHA). The FFN contains a Multiple-of-Expert (MoE) layer which dynamically dispatches input sentence tokens to the most appropriate expert(s). As a result, each token only activates a small portion of the MoE layer's weight, allowing the model to recall a vast amount of knowledge while activating only the relevant information for a given task. In Fig. XX, it is evident that each expert handles a varying number of tokens selected randomly from the input sentences.
In addition to the sparse weight, the token in the FFN is also sparse, with some tokens being entirely zero while others have a large proportion of zero values, sometimes exceeding 95\%. Furthermore, this sparsity is dynamic and fine-grained, as shown in Fig. XX.

In the MHA, the tokens of each sentence self-attend to one another, resulting in $O(L^2)$ computation and memory consumption where $L$ represents the sentence length. Sparse attention is an effective technique that reduces the computation and memory cost of LLMs like GPT-3, GPT-3.5. Fig. XX illustrates a sample sparse pattern of sparse attention that varies in computation granularity. Additionally, it is natural in language that sentences vary in length, necessitating padding of zero tokens to align them. This padding dynamically changes depending on the batches.
Similar to sparse attention, many deep learning networks are dynamically attentive to input data. This dynamic attention mechanism enables the network to focus more on informative regions of the data, leading to improved performance. An example of such a network is the dynamic sparse network depicted in Fig. XX. By selectively masking out irrelevant background, this model can achieve higher accuracy with less computational cost.

\para{Misalignment between the irregular computation and regular operator-based deep learning frameworks.}
% 1) manually rearrange data to adapt to regular computation with the cost of data transformation, movement, and copy. 2) using mask tensors to filter effective computation.
Existing deep learning frameworks mainly focus on operators with regular shape (\ie without sparsity), as the regular computation can be easily and efficiently mapped to SIMD accelerators. The 
The common characteristics of the sparsity demonstrated above are 1) the data of the computation . Existing deep learning frameworks mainly focus on operators with regular shape which can be easily accelerated on SIMD accelerators. To leverage 

existing efforts... (the reason frameworks work on regular operators)

\para{Misalignment between irregular computation and SIMD accelerators.}
faithfully following data granuarity to do the computation leads to inefficient computation. covering sparse data with larger granularity as demonstrated in SparTA waste computation, which is aligned with hardware.
1) computation granularity is not aligned with hardware e.g., wmma. 2) data encoding/decoding overhead. 3) data read/write does not saturate transactions, bank conflict.

\para{opportunity: Unleashing the potential of SIMD accelerators for irregular computations.}
1) efficient/fast computation reconstruction (transformation/stile) to align with hardware. 2) 

% Dynamic Sparsity is very common and important but hard to be optimized. We find three obstacles in the dynamic sparsity optimization.

% \begin{figure}[htbp]
% 	\centering
% 	\includegraphics[width=\columnwidth]{Figure/experiments/dynamic_sparse_cases.pdf}
% 	\caption{\label{fig:dynamic_sparse_case}Dynamic sparsity examples.}
% \end{figure}

\begin{figure}[t]
  \centering
  % \captionsetup[subfigure]{labelformat=empty}
  \subfloat[Dynamic Sparse Networks]{
    \label{fig:dynamic_sparse_case_dynamic_algorithm}
    \includegraphics[height=2.3cm]{Figure/experiments/dynamic_sparse_cases_c.pdf}} 
  \subfloat[Mixture-of-Experts]{
    \label{fig:dynamic_sparse_case_moe}
    \includegraphics[height=2.3cm]{Figure/experiments/dynamic_sparse_cases_a.pdf}} \\
  \subfloat[Dynamic Sequence Length]{
    \label{fig:dynamic_sparse_case_seq_len}
    \includegraphics[height=2.3cm]{Figure/experiments/dynamic_sparse_cases_b.pdf}} 
  \subfloat[Sparse Training]{
    \label{fig:dynamic_sparse_case_dynamic_training}
    \includegraphics[height=2.2cm]{Figure/experiments/dynamic_sparse_cases_d.pdf}} 
  \caption{Examples of dynamic sparsity in deep learning.}
  \label{fig:dynamic_sparse_case}
\end{figure}



%Dynamic sparsity widely exists in modern deep-learning models. Promising future.
Inspired by biological neural networks, modern deep-learning models have evolved to be dynamically sparse. The model will activate different regions according to different inputs, just like the human brain. Various dynamically sparse models emerge in deep learning, here we introduce four representative categories as shown in \autoref{fig:dynamic_sparse_case}.
%illustrates four widely existing dynamic sparse scenarios. 

\para{Dynamically sparse networks.}
A large category of deep-learning models\cite{han2021dynamic,habibian2021skip,fedus2021switch,zoph2022designing,hwang2022tutel,wang2021spatten,zhou2022energon,rao2021dynamicvit,zhou2021informer,kitaev2020reformer,liu2021transformer} are dynamically attentive to the input data. Such dynamic attention allows the model to focus more on the informative region of the data to achieve better performance. \autoref{fig:dynamic_sparse_case_dynamic_algorithm} illustrates an example of dynamic sparse network\cite{habibian2021skip}. By masking out the irrelevant background, the model can achieve higher accuracy with less computation. The mask is online produced by several dedicated layers of the network.

\para{Mixture-of-Experts (MoE).}
MoE is a typical dynamically sparse network that is widely used in popular large models, such as Switch Transformer~\cite{fedus2021switch}, V-MoE~\cite{riquelme2021scaling}. As shown in \autoref{fig:dynamic_sparse_case_moe}, a sequence of tokens passes through a gating function (\ie Router) which assigns each token to an expert(s) in an online manner. 
%Each expert is usually a multi-layer perceptron (MLP) network. 
Semantically, an expert only takes a proportion of the tokens that are located in its mastered domain (\eg two out of four in \autoref{fig:dynamic_sparse_case_moe}). Thus, the computation of each expert is dynamically sparse depending on the input tokens.
%shows an example of an MoE layer. The MoE layer consists of multiple expert sub-modules and each expert is good at a different field. Given an input sequence, each token(word) is dispatched to the corresponding expert sub-module. In contrast to computing all the tokens, each expert only computes the received ones sparsely. Therefore, the calculation of each expert is dynamically sparse according to the input.

\para{Dynamic sequence length.}
In natural language processing\cite{bert,ouyang2022training,raffel2020exploring} and multi-modality models~\cite{radford2021learning,ramesh2022hierarchical}, sequences naturally have varied lengths. Processing such sequences in batch requires padding them the same sequence length(typically the maximum length in the batch), as shown in \autoref{fig:dynamic_sparse_case_seq_len}. Such padding leads to unnecessary computation and can be treated as dynamic sparsity.
\begin{comment}
In natural language processing (NLP), sentences naturally have varied lengths. When training an NLP model\cite{bert,ouyang2022training,raffel2020exploring} or multi-modality model\cite{radford2021learning,ramesh2022hierarchical}, the sentences should be grouped into batches. The computation of the model requires a batch of sentences to be padded to the same length (\ie the maximum length of the sentences) with a regular shape as shown in \autoref{fig:dynamic_sparse_case_seq_len}. Such padding, as an approach to deal with the dynamic sparsity, leads to unnecessary computation waste.
%To saturate computation resources, the sentences should be batched together and padded to feed in the model. The batch mechanism is always used to better saturate the computation resource. However, sentences in the same batch need to be padded to the same length, as shown in \autoref{fig:dynamic_sparse_case_seq_len}. Such padding will lead to unnecessary computation waste.
\end{comment}

\para{Sparse training.}
Sparse training is critical and widely used in many fields of deep learning, such as MAE~\cite{he2022masked}, pruning~\cite{nn_pruning} and supernet training\cite{cai2019once, chen2021autoformer}. Take pruning as an example, \autoref{fig:dynamic_sparse_case_dynamic_training} illustrates the process of spare training in pruning. In each step, the algorithm will mask out a portion of the weight according to the current model state.
The mask position of each step is constantly changing during pruning.

\begin{comment}
\autoref{fig:dynamic_sparse_case_dynamic_training} illustrates an important training process using masks (e.g., MAE~\cite{he2022masked}, NNPruning~\cite{nn_pruning}).
By randomly masking the input patches/tokens, value of the weight matrix, or activation, the generalization of the model can be effectively improved and the accuracy can be increased.
% Several approaches have proposed different strategies to decide which data to mask. All of them decide the mask at inference, introducing the dynamic sparsity to input tensors or weight matrixes. 
Sparse training is critical and widely used in many fields of deep learning
(learning with masked\cite{he2022masked,li2022scaling,bao2020unilmv2,ding2022cogview2}, model compression\cite{nn_pruning, han2015learning, li2020train}, dropout\cite{wan2013regularization}, supernet training\cite{cai2019once, chen2021autoformer}). 
\autoref{fig:dynamic_sparse_case_dynamic_training} illustrates the process of sparse training. In each step, the algorithm will mask out a portion of the input, activation, or weight accordingly.
The mask position for each step may be generated randomly or according to the sampling strategy.
\end{comment}

\begin{comment}
To mimic how the human brain works, modern DL models often introduce dynamic sparsity to improve efficiency. \autoref{fig:dynamic_sparse_case} illustrates four popular DL models with dynamic sparsity. Usually, they introduce padding or masks to express the sparsity in the input or activation tensors. However, if the padded/masked tensor participates in computation using dense kernels, they still have to be computed due to SPMD instructions on accelerators leading to inefficient computation due to wastes of accelerator cycles and energy. % Similar to dynamic sequence length, using dense computation kernels for the sparsely activated experts is often inefficient due to waste on padding.
\paragraph{Dynamic sequence length.} As shown in \autoref{fig:dynamic_sparse_case_seq_len}, language tasks usually do training or inference with multiple sentences in a batch, to improve the throughput. The sentences will naturally have different sequence lengths. To form a tensor, the short sentences have to be padded to the length of the longest sentence in the batch. 

\paragraph{Mixture-of-Experts (MoE).} \autoref{fig:dynamic_sparse_case_moe} shows a Mixture-of-Experts (MoE) layer in Switch Transformer~\cite{}. By dynamically routing tokens among multiple expert sub-networks, MoE can scale the Transformer model to trillion parameters without increasing the inference cost. The key advantage comes from its sparse routing that dynamically dispatches input tokens to the most suited expert(s). Router usually makes the routing decision based on the token value, thus can only be done at runtime. The experts are naturally sparsely activated that different experts receive different numbers of tokens and some experts even receive zero tokens. E.g., the first expert only receives two tokens (``Token1'' and ``Token3'') and bypasses the rest. 
%he router computes the probability distribution of experts using each token as input, thus deciding which expert each token should be dispatched to at runtime

\paragraph{Dynamic Sparse Networks.} A large category of deep learning architectures leverage the intrinsic sparsity of the input or task. As the example shown in \autoref{fig:dynamic_sparse_case_moe}, the classification of bird types only requires the foreground content and computation on non-relevant content can be skipped. Typical approaches use an extra branch to generate a spatial mask to decide the execution of convolution on each pixel~\cite{habibian2021skip}. Some approaches generate high-quality results by applying extra layers on salient pixels~\cite{almahairi2016dynamic,hua2019channel}, which are also dynamic and sparse.

\paragraph{Sparse training.} \autoref{fig:dynamic_sparse_case_dynamic_training} illustrates an important training process using masks (e.g., MAE~\cite{}, NNPruning~\cite{nn_pruning}). By masking random patches of the input image or values in the weight matrix, the training of a supervised model can be accelerated and lead to improved accuracy. Several approaches have proposed different strategies to decide which data to mask. All of them decide the mask at inference, introducing the dynamic sparsity to input tensors or weight matrixes. 
\end{comment}
%Summarize some categories; then foresee the potential of dynamic sparsity in deep learning; explain how the sparsity is specified online.

% \para{Existing support of dynamic sparsity is inefficient.} Introduce the existing supports and analyze where the inefficiency is. One inefficiency is sparse data construction (or index construction), because of fine-grained sparsity.; Specialization (or compiling) of high-efficient kernels is time-consuming; what about sparse data construction with block sparse?


% \textbf{Current framework cannot understand/be aware of the dynamic sparsity(no appropriate abstraction/interface)}
% \para{Lack of suitable data representation for tracking dynamic sparsity.} It limits optimization opportunities. 1) static plus dynamic, 2) mask is inefficient.

% \textbf{Gap between Pruning and Sparse Kernel, data block -> computation tile.}
% The gap between data tile and the computation tile.
% \para{Inefficient mapping of sparse computation to hardware computation unit.}

\subsection{Limitations of Existing Solutions} 
\label{sec:moti_limitation}
% (1) no unified/systematic solution  
% (2) cannot apply optimization to better saturate the GPU like dense computation
% (3) computation waste

\para{Diversed dynamic sparsity.} Dynamic sparsity has become a new trend and is widely used in various scenarios recently, as mentioned above. Compared to static sparsity, the dynamic sparsity pattern in different scenarios is quite diverse and complex. The main reason is that the dynamic sparsity pattern is closely related to the scenario and input. The four popular scenarios mentioned above have totally different dynamic sparsity patterns. Even with the same scenario, dynamic sparsity patterns are also very diverse and complex. For example, the sparsity pattern in \autoref{fig:dynamic_sparse_case_dynamic_algorithm} is in the shape of a bird. As the input image changes, the next sparsity pattern may change to a puppy suddenly. There is no systematic optimization methodology for all various and complex dynamic sparsity patterns.

\para{Gap between data granularity and computation granularity.} Optimizing such complex dynamic sparsity patterns requires flexibility between the data granularity and computation granularity. Plenty of sparse optimization libraries are proposed in the past few years, including the fine-grained sparse library~\cite{cusparse, sputnik}, block sparse library~\cite{triton}, and coarse-grained sparse library\cite{sparta, nn_pruning}. However, such sparse libraries are all proposed for specific data granularities and perform badly on the other granularities. Given a sparsity pattern, using fine-grained data granularity to cover all remained values is highly efficient and will not cause computation waste. However, fine-grained computation kernels cannot well saturate hardware due to the random memory access caused by fine-grained data. In contrast, block sparse kernels have a relatively high efficiency but covering remaining values with data blocks(\eg $32\times32$) may lead to significant computation waste. The key to optimizing such dynamic sparsity is to perform the calculations with and efficient kernel without computation waste at the same time. Therefore, optimizing such complex dynamic sparsity patterns requires breaking the binding between the data granularity and computation granularity.
It is worth noting that previous sparse tensor compilers (such as SparTA\cite{sparta}) may take hours to generate the sparse kernel for a specific sparsity pattern. Therefore such ahead-of-time compilers do not work for dynamic sparsity.
%Take the bird shape mask as an example.
% Optimizing such complex dynamic sparsity requires flexibility between the computation and data granularity.

\para{Efficient online detection.} As the dynamic sparsity changes ceaselessly, how to detect the sparsity on the fly efficiently is challenging. The sparse index constructed based on the current sparsity pattern will become invalid once the sparsity pattern changes. Previous sparse libraries, such as cuSPRAESE, Triton, may provide a sparse index construction methodology for a specific data granularity. However, an efficient general index construction mechanism for all kinds of data granularities is still missing. In addition, the performance of previous sparse index construction methodology is also poor due to the constraint of sparse computation kernels. For example, Sputnik requires the indexes in each row to be ordered for better local reusability.


\begin{comment}
Commodity accelerators have primarily focused on accelerating computationally intensive dense computations like matrix multiplication and convolutions, which have highly regular computation patterns. The diverse and irregular sparse computation introduces new challenges for commodity accelerators. We review the state-of-the-art sparsity solutions and discuss their limitations when handling dynamic sparsity. %This is a huge gap to efficiently execute the irregular and dynamic sparsity patterns on commodity accelerators. Existing approaches to running sparsity computation on commodity accelerators vendor-provided libraries (e.g., cuSPARSE), tuning efficient computation kernels (e.g., SparTA), or special hardware units for sparsity (e.g., Sparse Tensor Core).

\paragraph{Constrained granularity in sparsity libraries.} The most straightforward way to conduct sparse computation on commodity accelerators is to leverage the pre-built computation kernels of sparsity libraries, e.g., cuSPARSE, OpenAI, Sputnik for Nvidia GPUs~\cite{} and rocSPARSE for AMD GPUs~\cite{}. The computation kernels are designed for efficient execution on specific sparsity patterns. E.g., OpenAI's kernel is efficient for 32x32 or 16x16 block sparsity; However, the sparsity granularity at runtime is dynamic and diverse, which may not always match the design size. Accelerators will suffer from low utilization if the data sparsity is larger than designed granularity, or wasted computation on the other hand. Although cuSPRASE and Sputnik support general sparsity, their kernels are limited to too fine-grained computation that fails to exploit accelerators efficiently. They can only outperform equivalent dense computation when sparsity is higher than 90\%. [xxx: how fine-grained is too fine-grained?]

\paragraph{Constrained patterns in sparsity hardware.} To better support sparsity on accelerators, several architectures are proposed for running sparse computation. E.g., Nvidia Ampere GPUs provide hardware acceleration for a special 2:4 structured sparsity. BBS uses FPGA to accelerate LSTM networks with a bank-balanced sparsity pattern. These hardware acceleration for sparsity requires a fixed sparsity pattern, which are efficient for specially tuned weight matrix but can only cover a very limited size of dynamic sparsity at runtime.

\paragraph{Time-consuming sparse kernel generation.} To better fit the sparsity pattern to commodity accelerators, existing solutions have been proposed to generate sparse computation kernels via compilation. For example, SparTA~\cite{} can generate the most efficient kernels by taking into account the
execution efficiency of different sparsity patterns on different sparsity-aware hardware. However, kernel generation is a time-consuming searching procedure and requires a static sparsity pattern prior known before deployment. As we have shown in \autoref{fig:dynamic_sparse_case}, dynamic sparsity is only known at runtime. It would take too long to compile efficient sparse kernels for every sparsity pattern that appeared at runtime. 

% \textbf{No fast index construction mechanism.}
% \para{High overhead of online sparse data conversion.}
\end{comment}
\begin{figure}[t]
	\centering
	\includegraphics[width=1.0\columnwidth]{Figure/stile.pdf}
	\caption{\label{fig:stile} Four examples of sparse matrix multiplication $C=A*B$. The four different sparse data tiles are mapped to the same dense computation tile.}
\end{figure}
\subsection{Leveraging Dense Kernels for Sparsity}
Given that commodity accelerators are very good at regular computation, can we leverage their efficient dense computation kernels for computations with dynamic sparsity? We find many sparse computations in deep learning computations can be conducted in dense kernels. \autoref{fig:stile} shows four examples of matrix multiplication. The shaded area has non-zero values and the rest are zeros. By rearranging the non-zero rows, columns, or small blocks, the sparse computation can be ``condensed'' into an equivalent dense matrix multiplication. Moreover, the data of some dimensions can be rearranged in an arbitrary order, which is very friendly to commodity accelerators for parallel calculation. We call this property, \emph{permutation invariant}, which is formally defined in \S\ref{sec:permutation}. All these motivate \sysname{} to systematically exploit the {permutation invariant} property for efficiently dealing with dynamic sparsity patterns known at runtime.
%find an extremely fast approach to leverage the {permutation invariant} property, 
%thus we can transform sparse computation into the most efficient dense computation even for dynamic sparsity patterns known at runtime.

% \para{Aligning dynamic computation to hardware.}

% \textbf{No scheduling policies for dynamic sparsity scenarios.(each sample in the batch may have different sparsity pattern)}

==> design_backup.tex <==
\section{\sysname{} Design}

\label{sec:design}


To address the abovementioned challenges, we design \sysname{}, its architecture is shown in \autoref{fig:overview}. First, we extend TeSA~\cite{sparta}, a sparse data format, to a new online-parsing friendly format called \dtesa{}. A deep-learning model of dynamic sparsity annotates its tensors' sparsity waith \dtesa{}. \sysname{} has two stages to optimize the execution of the sparse model. The first stage is ahead of time compilation optimization. It analyzes the dynamically changed sparsity of an operator's input/output tensors to determine the most suitable tiling strategy for this operator. Unlike the traditional tiling technique~\cite{}, 
\sysname{} introduces much more flexibility on data arrangement of a tile, called \stile{}. \stile{} maps sparse data into a dense data block and relies on traditional dense computation tile to do the computation. With the selected \stile{}, \sysname{} generates a sparse kernel for this operator. This stage can be executed periodically to deal with sparsity pattern shifting. The second stage is applying the generated sparse kernel in runtime execution. To deal with the dynamically changed sparsity, the sparse kernel encapsulates three components. Online index constructor builds the index of the sparse data following the \stile{}. The second component rearranges the sparse data into dense format when loading data across hierarchical memory levels (\eg from global memory to shared memory of GPU). At last, the dense computation tile is applied to the condensed data without knowing their indices. The property of \stile{} makes such computation correct, which is called \textit{computation invariance}.

% To enable optimization of dynamic sparsity in the model, we propose \sysname{}, as shown in Figure~\ref{fig:overview}. The two key abstractions of \sysname{} are \dtesa{} and \stile{}. \dtesa{} enhances the expressiveness of tensor in terms of dynamic sparse pattern compared with \tesa{}~\cite{SparTA}. An algorithm designer can specify arbitrary static and dynamic sparse pattern through \dtesa{}. \stile{} decouples the model sparsity granularity and the underlying computation granularity. With \stile{}, \sysname{} can bridge the small sparsity granularity and large computation tile to achieve better performance.

% Algorithm~\ref{alg:overview} shows the workflow overview of \sysname{}. Given initial \dtesa{} attributes of a model, \sysname{} first separates the static and dynamic sparsity pattern. \sysname{} optimizes the static sparsity offline. Offline optimization overhead of static sparsity pattern can be amortized because static sparsity does not change subsequently.
% The dynamic sparsity pattern in the model changes over time, therefore the indexes of the dynamic sparsity pattern need to be built online accordingly. However, we find that though the positions of sparsity changes frequently, the granularity of sparsity is relatively stable. Based on this finding, \sysname{} searches the appropriate Sparse Computation Tile (\stile{}) according to the granularity of the dynamic sparsity on the fly. The \stile{} reorganize the discrete sparse computation into a dense computation to leverage various highly efficient manually designed dense kernel.

% Once the appropriate \stile{} is determined, \sysname{} will generate efficient sparse kernel accordingly. Whenever a new input data or sparse pattern arrives, \sysname{} will quickly build the sparse indexes for current input data. The generated sparse kernel will dynamically skip unnecessary calculation based on the sparse index. %With both static and dynamic sparsity optimized kernel, \sysname{} can 
\begin{figure}[t]
	\centering
	\includegraphics[width=0.95\columnwidth]{Figure/architecture.pdf}
	\caption{\label{fig:overview} Architecture overview of \sysname{}.}
\end{figure}

\subsection{Dynamic Sparsity Representation} \label{sec:dtesarepr}

%statistic granularity and online sparsity attributes, reasons. provided online by user. the granularity can be a variable.

To optimize the deep learning model with changing sparsity, users should specify the sparsity of the sparse tensors in an online manner during model execution. Unlike SparTA, which uses the sparsity attribute (\ie TeSA) only at compile time, in dynamic sparsity the attribute tensors for expressing changing sparsity become a part of the model, which is located in the critical path of model execution. It requires the sparsity attribute to be efficiently constructed and parsed, while consuming less memory. Thus, we design \dtesa{} to combine the sparsity attribute matrix with  sparsity granularity. With sparsity granularity, each value in the attribute matrix represents the existence of a data block instead of an element. \dtesa{} can express different types of dynamic sparsity. One type is that the location of sparse values keeps changing while the granularity is the same (\eg in model pruning~\cite{}). In another type, the granularity could also change. For example, in language model the sequence length of input data samples is different. Padding them to the maximum length induces sparsity, where sparsity granularity in \dtesa{} could efficiently express this sparsity, \ie each sample has its own sparsity granularity as large as its sequence length. Formally, the sparsity granularity is in the form of $(S_{dim1}, S_{dim2})$, where $S_{dim}$ is the size of the granularity along dimension $dim$. The granularity not only makes the sparsity attribute much smaller, but also aligns with the \stile{} abstraction which will be demonstrated below.

%For optimizing the dynamically changed sparse model, the model's sparsity should be specified, \ie annotating tensors' sparsity attribute. Dynamic sparsity requires the sparsity to be annotated online by users, which brings more stringent requirement on the efficiency of sparsity optimization as it is located in the critical path of model execution. We extend TeSA by adding sparsity granularity, which changes from element-wise attribute to block-wise attribute. The granularity is specified with $(S_{dim1}, S_{dim2})$, where $S_{dim}$ is the size of the granularity along dimension $dim$. The granularity could be the same (\eg model pruning) and could also keep changing (\eg dynamic sequence length of language models) along the model execution. The granularity not only makes the sparsity attribute much smaller, but also aligns with the \stile{} abstraction which will be demonstrated below.

% \dtesa{} enables users to specify arbitrary sparsity pattern for given model including both static and dynamic sparsity. Figure~\ref{fig:dtesa} shows an example of \dtesa{}. \dtesa{} consists of two parts: elementwise static sparsity attribute and dynamic sparsity annotations. \dtesa{} first enhances the original value tensor with an extra tensor with the same shape, where each element represents the static sparsity attribute of the corresponding values\cite{sparta}. In addition, \dtesa{} also includes the dynamic sparsity annotation to describe the dynamic sparsity pattern as shown in the right side of the Figure~\ref{fig:dtesa}. Specifically, \sysname{} provides two kinds of dynamic sparsity annotations: (1) $Granularity$ to describe the granularity of the dynamic sparsity (2) $Range$: to describe the position constraint. Both kinds of annotation are optional and can be annotated on any dimension or combination of dimensions. The \dtesa{} in Figure~\ref{fig:dtesa} means the upper left corner of the tensor is always 0 and some dynamic sparsity with granularity of $1\times 1$ are randomly distributed. In addition, user can also use variable in the $Granularity$ and $Range$ annotation. For example, in the case of dynamic sparsity caused by different sequence length, shown in Section~\ref{sec:eval_seqlen}, the $Granularity$ of dynamic sparsity is $seqlen\times seqlen$ and the $Range$ is $0:seqlen, 0:seqlen$. Here, $seqlen$ is a variable that represents the effective length of input sequences. Therefore, this \dtesa{} means we only need to calculate the submatrix of $seqlen\times seqlen$ in the upper left corner.

% \dtesa{} allows the user to specify arbitrary static and dynamic sparsity pattern and reveals the optimization opportunity of dynamic sparsity, especially for scenarios with potential dynamic sparsity, such as the dynamic sparsity in the pruning progress and caused by different sequence lengths (evaluated in Section~\ref{sec:eval_pruning}, \ref{sec:eval_seqlen}). More importantly, with \dtesa{}, \sysname{} can understand the characteristics of both the static and dynamic sparsity at the compile time, which enables corresponding sparsity optimizations. 


% \begin{figure}[htbp]
% 	\hfill
% 	\includegraphics[width=0.9\columnwidth]{Figure/DTeSA.pdf}
% 	\caption{\label{fig:dtesa} Example of \dtesa{}.}
% \end{figure}

\subsection{\stile{} Abstraction}\label{sec:stileabs}

%\QL{We can try the following logic flow to introduce \stile{}: 1) Efficient execution of (dynamic) sparsity requires fully utilizing hardware; 2) Making sparse computation aligned to hardware is the principle to achieve high efficiency; 3) We propose \stile{}, an abstraction that systematically opens up the effective mappings/alignments of various sparsity patterns to hardware; 4) the effective computation on hardware is abstracted by computation tile which has been well optimized and aligned to hardware; 5) The mapping can be online constructed for supporting dynamic sparsity.}

%\NX{Explain the stile abstraction and give several examples here}.
%\NX{For dynamic sparsity, the memory load efficiency actually need support from the converter.}

% one paragraph to introduce the necessary of stile
Sparse computation, especially unstructured sparsity, can hardly well utilize the modern hardware which has increasing number of cores with SPMD instructions provisioned (\eg GPU). Its irregular data access makes data movement across memory hierarchies (\eg global memory to shared memory in GPU) less efficient. Its computations can hardly be grouped into SPMD instructions. Existing optimizations for sparse computation leverage special data layouts to mitigate the effect of the irregularity. However, their computation efficiency still lags far behind that of the dense computation of the same FLOPs, because of the intrinsic misalignment between sparse computation and modern vectorized hardware design. To bridge the gap, we design sparse computation tile \ie \stile{}. It starts from basic computation granularity (\eg warp, read/write transaction) of hardware, derives diverse sparsity patterns that can be aligned to the granularity with proper transformation. The key is decoupling sparse data access and computation, \ie preparing sparse data to be a regular dense format, making the following computation free from index decoding/encoding.

\label{sec:design}


An \stile{} is a group of data tiles with a specific type of placement, associated with a dense computation tile. Those data tiles can be condensed to become the computation tile. \autoref{fig:stile} shows four example \stile{}s which are corresponding to the same dense computation tile. Assuming the dense tile is $T_C=T_A*T_B$, whose shapes are $[4, 3]=[4, 5]*[5, 3]$ respectively. The \stile{} on the top left of \autoref{fig:stile} allows the rows of $T_A$ to be scattered in non-continuous rows of matrix $A$. The data tile of this \stile{} is the size of $T_A$'s one row (\ie $1\times5$), which can be seen as the effective sparsity granularity. The data tiles can be condensed to a dense tensor during loading from lower level to upper level memory (\eg from global memory to shared memory), then the computation is executed on the dense tile. Similarly, the data tile can be vertical in matrix $A$ (\ie $4\times1$) as shown on the top right of \autoref{fig:stile}, where the data tiles in $A$ and $B$ are aligned in the dimension $k$. More aggressively, the data tile could be smaller like the bottom two \stile{}s in \autoref{fig:stile}. Their data tiles follow special placement, \ie the data tiles in $A$ are aligned on both dimension $k$ and $m$.

\stile{} decouples sparse data (\ie the data tiles) encoding/decoding and computation. The computation (\ie computation tile) operates on the dense data without traditional sparse data index, which greatly improves computation efficiency. The preparation of the dense data happens on the fly during data movement across memory hierarchies. This decoupling is enabled by a concept called \textit{computation invariance} which is demonstrated below.

%As long as the read/write of data tile aligns memory transaction, the on-the-fly data rearrangement across memory hierarchies between scattered data tiles and the condensed format induces no overhead.

\para{Computation invariance.} The example \stile{}s in \autoref{fig:stile} imply that the size and placement of data tiles cannot be arbitrary. They follow a constraint, \ie after the data tiles are condensed along their dimensions to be a dense matrix, the dense computation should be able to run on the dense matrix correctly. Formally, for a dense operator $C=op(A,B)$, the implementation of $op$ can be applied on the condensed data $T_A$, $T_B$ from scattered data tiles without any change. This is defined as computation invariance. Then, the problem is \textit{what kind of data rearrangements (\ie \stile{}) satisfies computation invariance.}

%To unveil all the \stile{}s systematically, 
We derive feasible data rearrangements from operator expression (\eg einsum~\cite{}). An operator expression specifies how the output value is computed from the values of input tensors, \eg $C[m,n]$+=$A[m,k]*B[k,n]$ of Matmul. To guarantee computation invariance, sparse matrix (\eg $A$ becomes sparse) can only be rearranged along dimensions (\eg $M$ dimension). That is, the indices of the kept elements on a dimension can be mapped with a function $f$ to a dense sequence $0 \sim (l-1)$, where $l$ is the number of the kept elements. After data rearranged with the mapping function $f$, the computation on the data still follows the operator expression.

\begin{table}[t]
    {\centering
    \footnotesize{
    \begin{tabular}{l|c}
    \Xhline{2\arrayrulewidth}
    \textbf{Operator} & \textbf{Operator Expression} \\ \hline
    ReduceSum & $C[p]$ += $A[p, l]$ \\
    Addition & $C[p]$ = $A[p]$ + $B[p]$ \\
    BatchMatmul & $C[b,m,n]$ += $A[b,m,k]$ * $B[b,k,n]$ \\
    Convolution & $C[n,f,x,y]$ += $A[n,m,x+i,y+j]$ * $B[f,m,i,j]$ \\ \hline
    \end{tabular}}
    \par}
    \caption{Example operator expressions.\label{tab:expression}}
     %\vspace{-0.5cm}
\end{table}

\begin{table}[t]
    {\centering
    \footnotesize{
    \begin{tabular}{l|c|c}
    \Xhline{2\arrayrulewidth}
    \textbf{Dimension Type} & \textbf{Description} & \textbf{Exp.} \\ \hline
    Solo reduction $R_s$ & \makecell[l]{The reduction dimension that exists in \\ only one tensor} & $l$ \\
    Cross reduction $R_c$ & \makecell[l]{The reduction dimension that spans in \\ multiple tensors} & $k$ \\
    Prevalent spatial $S_p$ & \makecell[l]{The dimension that exists in all the \\ tensors} & $b$,$p$ \\
    Sporadic spatial $S_s$ & \makecell[l]{The spatial dimension that co-exists \\ with $R_c$ in the same tensor and is not $S_p$} & $m$,$n$,$f$ \\
    Compound $C_p$ & \makecell[l]{The dimensions in a compound \\ dimension (\eg $x+i$, $y+j$)} & $x$,$y$,$i$,$j$ \\ \hline
    \end{tabular}}
    \par}
    \caption{Five categories of dimensions in operator expressions. The ``Exp.'' column is the example dimensions from \autoref{tab:expression}. \label{tab:dimension}}
     %\vspace{-0.5cm}
\end{table}

The mapping functions cannot be arbitrarily applied on tensor dimensions. We classify tensor dimensions into five categories as shown in \autoref{tab:dimension}. Different type of dimension has different constraints on applying the mapping functions. We summarize the four rules below, which could derive all the \stile{}s.

\begin{itemize}[leftmargin=*]
  \setlength\itemsep{-0.4em}
  \item For a multi-dimension tensor $T$ which has an $S_p$ dimension, the mapping function $f$ of the sparse matrix (or vector) $T[:,x,:]$ can be different for different $x$ values, where $x$ is on $S_p$ dimension.
  \item For a multi-dimension tensor $T$ which has a $R_s$ dimension, the mapping function $f$ of the sparse vector $T[x,y,:]$ can be different for different values of $x,y$, where ``:'' is the $R_s$ dimension.
  \item For a multi-dimension tensor $T$ which has $R_c$ and $S_s$ dimensions, the mapping function $f$ of sparse vector $T[x,:]$ should be the same for different values of $x$, where $x$ is on $S_s$ dimension and ``:'' is $R_c$ dimension.
  \item Mapping function $f$ cannot be applied on $C_p$ dimension.
\end{itemize}

To obtain the most efficient \stile{}s, the operator expression and its sparsity should be preprocessed. The operator expression should be simplified by merging logically the same dimensions. For example, multi-dimension tensor for element-wise operator can be simplified to a single dimension tensor, which makes \stile{} constrained by a single dimension instead of multiple. The sparsity on the tensors of the operator expression should be fully propagated by the approach in SparTA~\cite{sparta}. [XXX: shall we elaborate the approach in SparTA for this part?]

%Computation invariance is intrinsically aligned with tensor expression (). When an operator is Computation invariance means in tensor expression (\eg einsum~\cite{}) the dimensions can be transformed with a mapping function. Most operators in deep learning can be expressed with tensor expression (\eg einsum~\cite{})

\subsection{\stile{} Kernel Generation}
\begin{comment}
\begin{algorithm}[t]
\caption{The kernel skeleton based on \stile{}.\label{alg:stile_kernel}}
\KwData{$G_{sparseIn}$: Sparse input tensors stored in global memory.}
\KwResult{$G_{Out}$: Output tensor stored in global memory.}
\SetKwProg{Fn}{Function}{:}{}

\Fn{SparseKernel($G_{sparseIn}$, $G_{Out}$)}{ \label{line:sparsekernel}
    \tcc{\footnotesize size and format of $S_{denseIn}$, $S_{denseOut}$ in shared memory are decided by \textit{DenseComputeTile}}
    \_\_shared\_\_ $S_{denseIn}$, $S_{denseOut}$\;
    \sload{}($G_{sparseIn}$, $S_{denseIn}$, $blockIdx$) \tcp*{one thread block}
    DenseComputeTile($S_{denseIn}$, $S_{denseOut}$)\; \label{line:densecomp}
    \swrite{}($S_{denseOut}$, $G_{Out}$, $blockIdx$)\;
}
\end{algorithm}
\end{comment}
% \begin{comment}
\begin{figure} [ht]
\centering
\begin{minted}[
breaklines=true,frame=lines
]{c}
/*Inputs and Output are in global memory*/
__global__ void SparseKernel(
    struct SparseTensors Inputs, 
    struct Tensor Output
){
    /* size and format of SinDense, SoutDense
       in shared memory are decided by
       DenseComputeTile
    */
    DeclareSharedMem(SinDense, SoutDense);
    SLoad(Inputs, SinDense, blockIdx); 
    DenseComputeTile(SinDense, SoutDense);
    Swrite(SoutDense, Output, blockIdx);
}
\end{minted}
\vspace{-0.5cm}
\caption{The kernel skeleton based on \stile{}.}
\label{fig:stile_kernel}
\end{figure}
% \end{comment}

\stile{} enables a new kernel skeleton of sparse computation, where the sparse computation is decomposed to separated data rearrangement phase and dense computation phase. We introduce two primitives \sload{} and \swrite{} for the data rearrangement. \sload{} maps sparse data tiles in input tensors to dense data block, while \swrite{} writes the output dense data block to the specified output data format, could be sparse or dense. The kernel skeleton is shown in \autoref{fig:stile_kernel} in CUDA~\cite{} style. \sload{} and \swrite{} are the additional overhead in the sparse kernel ($SparseKernel$ in Figure~\ref{fig:stile_kernel}) compared to the dense computation ($DenseComputeTile$ in Figure~\ref{fig:stile_kernel}). However, we can eliminate the overhead leveraging memory hierarchy of modern devices.

% the granularity of sparse data that is friendly to hardware read transaction (in some cases, the data is more aligned after sparse index reconstruction)
% reduce the overhead of data rearrangement, directly pick out the effective data
% SLoad and SWrite can be independently implemented and connected to the dense tile computation

\para{On-the-fly data rearrangement.} \sload{} and \swrite{} works on data rearrangement when the data is moving from global memory to shared memory and in reverse. As long as data tile could saturate read/write transaction of the memory (\eg 32 bytes in CUDA GPUs), the data rearrangement would introduce little overhead, because the loading of sparse data tiles does not waste memory bandwidth. Thus, its performance almost equals to that of moving data across memory hierarchies in traditional dense computation. This property further enables \textit{zero-copy} of sparse data in online dynamic sparsity scenario (\eg MoE evaluated in \S\ref{sec:eval}), because the effective data tiles can be directly selected from their original (sparse) data format and written to the higher level memory with the desired format (\ie dense in our system).

\para{Optimizing \stile{} kernel.}
As demonstrated in \S\ref{sec:stileabs}, there are various \stile{}s. The most efficient \stile{} for a sparse operator is determined by three factors, \ie the efficiency of dense computation tile, the operator's sparsity, and the size of memory's read/write transaction. For the first factor, though different sized computation tiles are all dense, they have different computation efficiency. Usually, the smaller is the computation tile, the less efficient it is. Because it is harder to saturate all the available cores (\eg number of cores in an SM~\cite{}). Some carefully designed coordination of threads could greatly improve computation efficiency of small computation tiles, leading to many efficient small computation tile~\cite{}. These well optimized computation tiles are stored in the tile database of \sysname{} and serve as the base of \stile{}s.

%For the second factor, 
For a given sparsity, all the \stile{}s can be applied to it but with different computation efficiency. If the data tile of an \stile{} is larger than the granularity of the given sparsity, a proportion of the computation is wasted. Determining the most suitable \stile{} is trading off between \stile{}'s computation efficiency and wasted computation with the following formula: $$(Compute_{wasted}+Compute_{effective}) \times Cost_{stile}$$
, where $Compute_{wasted}$ means the number of FLOPS that are wasted by covering the non-zero values with data tile.
%Thus, different sparsity granularity has its most suitable \stile{}. For example, small granularity may prefer the \stile{} with smaller data tile. Though the corresponding dense computation tile is slightly less efficient, the wasted computation is also smaller. The granularity is not necessarily the same as the data tile of the chosen \stile{}.

\begin{algorithm}[t]
\caption{Optimizing \stile{} kernel for a dynamic sparse operator.} \label{alg:stileopt}
\KwData{$D_{Sparse}$: A list of $n$ sparse matrices of a sparse operator,\newline
        $Op$: The operator type}
\KwResult{$S_{tile}$: The best \stile{} for this sparse operator}
\SetKwProg{Fn}{Function}{:}{}

\Fn{ChooseStile($D_{Sparse}$, $Op$)}{ \label{alg:dynamic_opt}
    $Best_{stile}$ = NULL; $Cost_{optimal}$ = inf\;
    \ForEach{$s \in$ GetStilesFromTileDB($Op$)}{
        $Cost$ = 0\;
        \ForEach{$d \in D_{Sparse}$}{
            $Num_{tiles}$ = CoverAlgo($d$, $s.data\_tile$)\; \label{line:coveralgo}
            $Cost$ += $Num_{tiles} * s.tile\_cost$\;
        }
        \If{$Cost$ < $Cost_{optimal}$}{
            $Best_{stile}$ = $s$\;
            $Cost_{optimal}$ = $Cost$\;
        }
    }
    \KwRet $Best_{stile}$\;
}
\end{algorithm}

The complete process of choosing \stile{} for a dynamic sparse operator is shown in \autoref{alg:stileopt}. As the sparsity is dynamically changing, it first picks several represented sparse patterns. Then, it traverses all the \stile{}s in tile database to compute their cost on the given dynamic sparse operator. \texttt{CoverAlgo} (\autoref{line:coveralgo}) outputs the number of stiles that are needed to cover all the non-zero values.

% The essence of model pruning is sparsifying data blocks in the tensor. However how to translate sparse data blocks into efficient sparse computation is quite challenging. As introduced in Section~\ref{sec:moti}, the computation kernel on GPU are made up of two levels of parallel units: threads and thread blocks. Threads are grouped into large set of threads called thread block and the set of thread block that make up a kernel is called a grid. %Therefore, the sparse computation kernel also have two different sparse ways: sparse grid or the sparse thread block.
% If the sparse computation is sparsified at the thread level, then the kernel will launch all the thread blocks and each thread block perform a sparse computation based on corresponding sparse indexes. In this way, threads within the same block may perform different execution due to the sparse indices which may cause the divergence and lead to performance degradation. More importantly, sparse indices within the thread block also causes lots of random memory access and lead to poor memory bandwidth utilization and serious memory bank conflicts. In contrast, sparsifying the computation kernel at the thread-block level will skip the sparse thread block and the remaining blocks are calculated in dense. In this case, though the computation within the thread block is contiguous and efficient, the computation tile size of thread blocks is limited by the granularity of sparsity blocks. \NX{Explain why the block size is limited here?}. Small computation tile sizes may not be able to saturate the SM and lead to poor performance. To solve the problems above, we therefore propose the sparse computation tile(\stile{}) to bridges sparsity granularity and sparse computation efficiently.

% \begin{figure*}[htbp]
% 	\centering
% 	\includegraphics[width=1.98\columnwidth]{Figure/stile_k_axis_exp.pdf}
% 	\caption{\label{fig:stile_k_axis} Example of matrix multiplication \stile{} on K axis.}
% \end{figure*}
% %\begin{figure}[htbp]
% %	\centering
% %	\includegraphics[width=0.95\columnwidth]{Figure/stile_k_axis.pdf}
% %	\caption{\label{fig:stile_k_axis} Example of matrix multiplication \stile{} on K axis.}
% %\end{figure}
% %\begin{figure}[htbp]
% %	\centering
% %	\includegraphics[width=0.9\columnwidth]{Figure/stile_m_axis.pdf}
% %	\caption{\label{fig:stile_m_axis} Example of matrix multiplication \stile{} on M axis.}
% %\end{figure}
% \begin{figure*}[htbp]
% 	\centering
% 	\includegraphics[width=1.98\columnwidth]{Figure/stile_m_axis_exp.pdf}
% 	\caption{\label{fig:stile_m_axis} Example of matrix multiplication \stile{} on M axis.}
% \end{figure*}

% Figure~\ref{fig:stile_k_axis} shows an example of \stile{} of matrix multiplication on the K reduction axis. In this example, the shape of matrix A and B are $M\times K$ and $K\times N$ respectively. Besides. the matrix A is sparse and the green blocks represent the remaining non-zero values given by the pruning algorithm. Each thread block is responsible for computing a portion of the C matrix (marked in red). In general, \stile{} loads the data from global memory according to the sparse indexes and store the data in shared memory continuously. Leveraging the original dense computation tile, \stile{} then compute the corresponding output efficiently and write the results back to the global memory. There are two main factors that affect the performance of \stile{}: computation efficiency and read or write efficiency of the global memory. By remaining the original dense computation logic, the computation of \stile{} can be as efficient as the original dense tile. For the efficiency of global memory loading and writing, as long as the size of sparsity granularity can saturate the memory transaction, we can achieve the memory load or write performance close to original dense computation tiles, It's worth noting that for the skinny sparsity granularity, such as $32\times 1$, we can still saturate the memory transaction by changing the layout of A (from row-major to column major) or inserting a transpose operator. 

% To generate the code of \stile{} efficiently, we introduce two primitives: \sload{} and \swrite{} to represent the sparse memory loading or storing according to the sparse indexes. Line \ref{alg:sload_interface}, \ref{alg:swrite_interface} in Algorithms~\ref{alg:stile_construct} shows the interfaces of \sload{} and \swrite{}, where $dst$ and $src$ are the destination and source memory address respectively, and $loop$ represents the loop axis annotated to sparse.
% During the code generation, \sload{} and \swrite{} will translate memory address based on the sparse indexes automatically. As shown in the Figure~\ref{fig:stile_k_axis}, after applying \sload{} on the k-axis of the original dense matrix multiplication, \sysname{} replace the original dense loop accordingly when loading data from the global memory, as shown in the right side of the Figure~\ref{fig:stile_k_axis}.
% %\NX{shall we give an code generation example here?}

% \NX{introduce the computation consistency here?}
% \textbf{Calculation consistency}. \stile{}s should have the same calculation logic with corresponding dense computation tile to reuse the computation part in these efficient dense tiles. We call this \stile{} remains the calculation consistency with its corresponding dense tile. 
% To leverage the original dense computation tile, we need to maintain the consistency with its original calculation logic after applying \sload{} and \swrite{}. Which axes can be annotated with \sload{} or \swrite{} to ensure the calculation consistency is determined by the calculation logic of the original dense tiles. 
% As shown in Figure~\ref{fig:stile_k_axis}, matrix multiplication can apply \sload{} on the K-axis and leverage original dense computation without affecting the correctness. The middle of Figure~\ref{fig:stile_m_axis} shows a dense computation tile where each thread block compute submatrix multiplication of $BLOCK\_M\times BLOCK\_K \times BLOCK\_N$. Compared with the dense computation tile in Figure~\ref{fig:stile_k_axis}, the dense computation tile in Figure~\ref{fig:stile_m_axis} is further tiled on the K reduction axis and each thread block only traverses a part of the k-axis. As shown in the right side of Figure~\ref{fig:stile_m_axis}, \stile{} can still leverage the efficient dense computation by applying the \sload{} and \swrite{} on the M axis at the same time.
% Therefore different computation dense tiles may generate different \stile{}s accordingly.

% \textbf{Generating \stile{}s}. Algorithm~\ref{alg:stile_construct} shows the details of the \stile{} construction in \sysname{}. \sysname{} first builds a computation tile database that consists of manually designed dense computation tiles (such as openai\cite{}) or the dense tiles generated by the compilers, such as TVM\cite{tvm}. \sysname{} loads all dense computation tiles from database offline. For each dense computation tile, \sysname{} first parse out all axes in this tile and try to annotate \sload{} or \swrite{} on all possible combinations of axes. \sysname{} will check whether the \stile{} still remains calculation consistency with original dense computation tile. If so, the current \stile{} can reuse the efficient dense calculation part with original dense computation tile. \sysname{} use random data and random sparse indexes to verify whether the generated \stile{} still remains the calculation consistency with original dense tile. Specifically, \sysname{} generate and compile the code for \stile{} and corresponding dense tile. It then runs the dense operator and sparse operator with random data and sparse indexes. If the output of two operators is always the same under different random data and sparse indexes, then the generated \stile{} is legal.


% \NX{The implementation of the function $remainConsist$: random data driven based or the rule based}.
%\NX{Given the efficient dense tiles, how to generate the sparse tiles from the given dense computation tiles.}
%\stile{} is constructed of the efficient dense computation tile and \sload{} and \swrite{} primitives. \sload{} and \swrite{} build the memory address mapping from the global memory to the shared memory according to the sparse indexes. Specifically, when \sload{} or \swrite{} is applied to a dense loop, . By remaining the original dense computation logic, \stile{} can be as efficient as the original dense tile. \stile{}. 

%\NX{Sparse grid vs sparse block.}
%The essence of model pruning is setting (or removing) some data blocks to zero in the tensor and sparse kernels skip these data blocks during the calculation. However, calculation. After pruning, the data blocks in the origin tensors that need to be calculated are discrete and randomly distributed. Such discrete and randomly distributed data blocks make sparse kernel quite hard to be optimized: First, random memory access leads to underutilization of memory transaction size and wastes the memory bandwidth.
% \NX{Stile also access in the random pattern}

% \begin{algorithm}[t]
% \caption{\stile{} Construction \label{alg:stile_construct}}
% \KwData{$D_{Tile}$: Dense computation tiles loaded from the database}
% \KwResult{$S_{Tile}$: Sparse computation tiles generated from $D_{Tile}$}
% \SetKwProg{Fn}{Function}{:}{}
% \
% parse\_axes($dense_{tile}$); // parse out all axes in dense tiles \;
% remainConsist($Tile_d$, axes, stype);// check if the \stile{}s can remain the computation consistency\;
% \sload{}(dst, src, loop) \; \label{alg:sload_interface}
% \swrite{}(dst, src, loop) \; \label{alg:swrite_interface}
% \
% \Fn{Generate\stile{}($D_{Tile}$)}{ \label{alg:generate_stile}
%     $S_{set}$ = set()\;
%     \ForEach{$d \in D_{Tile}$}{
%         axes = parse\_axes($d$)\;
%         \ForEach{$S_a \in$ permutation(axes)}{
%             \If{remainConsist($d$, $S_a$, \sload{})}{
%                 $S_{set}$.insert(\stile{}($d$, $S_a$, \sload{}))            
%             }
%             \If{remainConsist($d$, $S_a$, \swrite{})}{
%                 $S_{set}$.insert(\stile{}($d$, $S_a$, \swrite{}))            
%             }
%             \If{remainConsist($d$, $S_a$, \sload{} \textbf{ and } \swrite{})}{
%                 $S_{set}$.insert(\stile{}($d$, $S_a$, \sload{} \textbf{ and } \swrite{}))            
%             }
%         }
%     }
%     \KwRet $S_{set}$
% }
% \end{algorithm}

\subsection{Online Sparsity Detection}\label{sec:fast_index}

In dynamic deep learning model sparsity, tensors' sparsity changes in every forward pass of the model. To deal with dynamic sparsity, it is critical to capture sparsity efficiently in an online manner. \sysname{} uses \dtesa{} to reduce the overhead of annotating sparsity as demonstrated in \S\ref{sec:dtesarepr}. During online model execution, \sysname{} detects the sparsity from the associated \dtesa{}, and builds the index of the non-zero blocks in the sparse tensor. The non-zero blocks are in the granularity of the data tile of the chosen \stile{} in \autoref{alg:stileopt}, thus, they are aligned with the \stile{} and can be efficiently parsed by \sload{} and \swrite{}. The constructed index can be any sparsity format, \eg BCSR~\cite{} used in our system.

Computation invariance of \stile{} enables two techniques for fast index construction: \textit{out-of-order index construction} and \textit{zero-copy data rearrangement}. Out-of-order index construction relaxes the order of the indices in the sparsity format. For example in BCSR, the column indices of non-zero elements in each row should be ordered, which induces considerable synchronization overhead especially in GPU devices. The computation invariance allows the column indices to be written out-of-order, thus, eliminates the synchronization overhead. On the other hand, with zero-copy data rearrangement, we can only build the index without copying the non-zero values. This is different from the traditional sparse data conversion where the non-zero values should be copies into the value region of the BCSR format. In our index construction, the index directly references the data blocks of the original tensor. It has no impact on the follow-up computation, because the data tiles are aligned with memory's read/write transaction. With the two optimization techniques, the index construction becomes very efficient. Though located in the critical path, it induces little overhead to the execution of dynamic sparsity.
% zero-copy; out of order

% \begin{figure}[htbp]
% 	\centering
% 	\includegraphics[width=0.95\columnwidth]{Figure/converter.pdf}
% 	\caption{Workflow of the fast index constructor.}
% \end{figure}


% \NX{Give the online optimization policy details here}.


==> design_backup2.tex <==
\section{\sysname{} Design} \label{sec:design}

\begin{comment}
To address the abovementioned challenges, we design \sysname{}, a compiling framework for dynamic sparsity. 
We first formulate the key concept of permutation invariant, then deduce 
% properties of it, such as being ubiquitous in deep learning and well compatible with existing dense optimizations. By applying it to the sparse computes, we show the feasibility of 
\property{} by applying permutation invariant on sparse data to build the connection between sparse computation and dense computation (\S\ref{sec:permutation}). Based on \property{}, \sysname{} introduces a new type of computation tile called \stile{} (\S\ref{sec:stileabs}), and builds a compiling framework for dynamic sparsity as shown in \autoref{fig:overview}.

There are two stages in \sysname{} to optimize the execution of a dynamically sparse model.
% The two stages all require the sparsity of the model to be annotated with the sparsity representation in \sysname{}. 
The first stage is to learn the sparsity distribution from only a few samples.
% The first stage is ahead-of-time compiling (\S\ref{sec:stilegen}). It has constructed a large set of \stile{}s. Each \stile{} supports a specific sparsity pattern
%in the granularity of data tile 
% and is connected to a well-optimized dense computation tile. 
The \stile{} optimizer analyzes the sparsity of each operator and selects the most suitable \stile{} from a set of pre-constructed \stile{}s, each of which is connected to a well-optimized dense computation tile.
\sysname{} generates a sparse kernel for the operator based on the selected \stile{}. 
This stage can be executed during the initialization, and also can be executed periodically to deal with possible shifting of sparsity distribution.
%In the second stage, \sysname{} detects the online sparsity with a high-efficient sparsity index constructor to capture effective computations. \sysname{} then feeds the effective computations indicated by the sparsity index into the generated sparse kernel. In the sparse kernel, the effective data are rearranged online into a dense format and consumed by the dense computation tile (\S\ref{sec:fast_index}).
The second stage is applying the generated sparse kernel at runtime (\S\ref{sec:fast_index}). To deal with the dynamically changed sparsity, \sysname{} detects the sparsity online and builds the index of the sparse data following the requirement of the \stile{}. There are two components in the sparse kernel, the first one rearranges the sparse data into dense format when loading data across different memory hierarchies (\eg from global memory to shared memory of GPU). The second one applies the dense computation on the condensed data without knowing their indices.
\end{comment}
% The sparsity of a model is online annotated with a new sparsity representation in \sysname{}.
% %\stile{} decouples the representation of dynamic sparsity and the computation. 
% %First, For the dynamic sparsity representation, we pay special attention on its efficiency of online processing. We extend TeSA~\cite{sparta}, a sparse data format, to a new online-parsing friendly format called \dtesa{}. 
% %A deep-learning model of dynamic sparsity annotates its tensors' sparsity with \dtesa{}. 
% There are two stages in \sysname{} to optimize the execution of a dynamically sparse model. The first stage is ahead of time compilation. It analyzes the dynamically changed sparsity of an operator's input/output tensors to determine the most suitable \stile{} for this operator. 
% For the computation, 
% \stile{} condenses sparse data into a dense data block with permutation and relies on traditional dense computation tiles to do the computation. With the selected \stile{}, \sysname{} generates a sparse kernel for this operator. This stage can be executed periodically to deal with possible shifting of sparsity patterns.

% The second stage is applying the generated sparse kernel at runtime. To deal with the dynamically changed sparsity, the sparse kernel encapsulates three components. Online index constructor builds the index of the sparse data following the \stile{}. The second component rearranges the sparse data into dense format when loading data across hierarchical memory levels (\eg from global memory to shared memory of GPU). At last, the dense computation tile is applied to the condensed data without knowing their indices.
% %The property of \stile{} makes such computation correct, which is called \textit{computation invariance}.

% To enable optimization of dynamic sparsity in the model, we propose \sysname{}, as shown in Figure~\ref{fig:overview}. The two key abstractions of \sysname{} are \dtesa{} and \stile{}. \dtesa{} enhances the expressiveness of tensor in terms of dynamic sparse pattern compared with \tesa{}~\cite{SparTA}. An algorithm designer can specify arbitrary static and dynamic sparse pattern through \dtesa{}. \stile{} decouples the model sparsity granularity and the underlying computation granularity. With \stile{}, \sysname{} can bridge the small sparsity granularity and large computation tile to achieve better performance.

% Algorithm~\ref{alg:overview} shows the workflow overview of \sysname{}. Given initial \dtesa{} attributes of a model, \sysname{} first separates the static and dynamic sparsity pattern. \sysname{} optimizes the static sparsity offline. Offline optimization overhead of static sparsity pattern can be amortized because static sparsity does not change subsequently.
% The dynamic sparsity pattern in the model changes over time, therefore the indexes of the dynamic sparsity pattern need to be built online accordingly. However, we find that though the positions of sparsity changes frequently, the granularity of sparsity is relatively stable. Based on this finding, \sysname{} searches the appropriate Sparse Computation Tile (\stile{}) according to the granularity of the dynamic sparsity on the fly. The \stile{} reorganize the discrete sparse computation into a dense computation to leverage various highly efficient manually designed dense kernel.

% Once the appropriate \stile{} is determined, \sysname{} will generate efficient sparse kernel accordingly. Whenever a new input data or sparse pattern arrives, \sysname{} will quickly build the sparse indexes for current input data. The generated sparse kernel will dynamically skip unnecessary calculation based on the sparse index. %With both static and dynamic sparsity optimized kernel, \sysname{} can 


%\textcolor{red}{To tackle the aforementioned challenges, we have devised a novel dynamic sparse compilation framework named \sysname{}. Central to \sysname{} is its sparse-to-dense transform, which enables \sysname{} to rearrange sparse tensors into micro-tiles and compute efficiently. Figure \autoref{fig:overview} illustrates the framework of PIT. \sysname{} consists of two parts: Just-in-time (JIT) compiling and online sparse computation.}

To tackle the aforementioned challenges, we have devised a novel dynamic sparsity compilation framework named \sysname{}. Central to \sysname{} is its PIT transformation, which can convert sparse tensors into the computation-efficient dense format in an online manner with minimal overhead. An overview of the \sysname{} architecture is illustrated in \autoref{fig:overview}. The framework comprises two major components: just-in-time (JIT) compiling and online sparse computation, both of which are based on the key abstraction of ``micro-tile'' (\S\ref{sec:pitmechanism}).
%\textcolor{black}{Micro-tile is the granularity of reassembling sparse tensors into dense tensors during sparse-to-dense transform}.

The JIT compiling process identifies the most efficient micro-tile for a given set of sparse tensor samples through the PIT transformation policy (\S\ref{sec:pit_policy}). All feasible micro-tiles are derived from PIT rules, which are mathematical equivalent computation transformations of deep learning operators. The sparse kernel generator then creates the sparse kernel based on the selected micro-tile. Unlike traditional (sparse) kernel generation frameworks (\eg TVM~\cite{}, TACO~\cite{}), \sysname{} separates sparse data encoding/decoding and computation in the generated kernel. The encoding/decoding process handles sparsity, while the computation part focues on dense calculations. This separation is enabled by two primitives \sload{} and \swrite{}. \sload{} reorganizes discrete sparse data into a dense format when transferring data across hierarchical memory levels, such as moving from global memory to shared memory in a GPU. \swrite{} performs the reverse process. In contrast to traditional approaches that adapt computation to a specific sparse data format (\eg CSR~\cite{}, COO~\cite{}), the computation in \sysname{} is purely dense. %\NX{maybe we should explain micro-tile and PIT property first?  the granularity to reorganize the sparse tensor? }

For online sparse computation, the online sparsity detector identifies non-zero values at the granularity of the selected micro-tile, meaning that non-zero values are encompassed by micro-tiles (\S\ref{sec:fast_index}). The indices of the non-zero micro-tiles are constructed online and fed into the generated sparse kernel. The PIT property enables full parallelism in sparsity detection and index construction, thus, minimizes the overhead in the online execution. The online sparsity detector also periodically samples sparse tensors and feed the tensors to the JIT compiling process in response to possible sparsity distribution shifts.

%and the high-performance memory access primitives, \sload{} and \swrite{}(\S\ref{sec:sload}). 
%These primitives enable \sysname{} to dynamically rearrange scattered sparse data in the input, thus resulting in more efficient computations. Meanwhile, the Sparse-Dense Transform property guarantees the mathematical equivalence of the computation logic before and after data rearrangement.

% As illustrated in \autoref{fig:overview}, \sysname{} comprises three major components, \sysname{} generator, online sparsity detection, and kernel selection policy. Given a computational expression with annotated dynamic sparsity, \sysname{} first leverages the Sparse-Dense Transform to generate an efficient sparse kernel. Specifically, \sysname{} selects a dense macro kernel from the database and endeavors to apply Sparse-Dense Transform on different axes, resulting in a corresponding sparse kernel.

% At runtime, \sysname{} swiftly detects the portions of the input that require computation and constructs the index needed for \sload{} and \swrite{}. The generated sparse kernel employs \sload{} and \swrite{} to reorganize the discrete sparse data into a dense format when loading data across hierarchical memory levels (\eg from global memory to shared memory of GPU). Thereafter, the efficient dense macro kernel performs computation directly on the compacted data. The online kernel selection strategy periodically generates new sparse kernels in response to input data distribution shifts.

% \begin{figure*}[t]
% 	\centering
% 	\includegraphics[width=1.6\columnwidth]{Figure/architecture_v4.pdf}
% 	\caption{\label{fig:overview} Architecture overview of \sysname{}.}
% \end{figure*}

\input{Design2}
\begin{comment}
    
\subsection{The Micro-tile Abstraction}
Figure 4 illustrates an example of matrix multiplication with Tiling. In previous Tensor-based compilers such as TVM and SparTA, each Tile calculation accessed a continuous slice of the original input Tensor (as shown in Figure 4), and the data accessed and computed by each Tile was fixed after compilation. However, we found that such constraints could not satisfy the increasingly complex and flexible algorithm expressions (see Section \ref{sec:motivation}). Drawing inspiration from memory management in traditional operating systems, \sysname{} proposes a new data mapping mechanism called Dynamic Data Virtualization, as shown in Figure 4b.

In operating systems, the operating system maps a process's contiguous virtual addresses to non-contiguous physical address spaces through a memory page table. Inspired by this, \sysname{} proposes a dynamic virtualization mechanism from shared memory to global memory. With dynamic data virtualization, the data accessed by each computation tile is no longer a fixed continuous slice of the input Tensor, but is composed of different discrete data blocks (as shown in the figure). Dynamic data virtualization breaks the constraints of accessing data, providing flexibility for efficient online rearrangement of computations. Such flexibility is crucial for today's flexible and complex deep learning algorithms. After the data is loaded into shared memory, the computation tiles can perform computations in a continuous and transparent address space (similar to virtual addresses in operating systems). By reusing the efficient memory access and computation patterns in the Dense Macro Kernel, \sysname{} can achieve the same efficiency in shared memory as in the original Dense computation kernel. The mapping relationship between the two layers of data is dynamically calculated online based on the input features. Therefore, \sysname{} can efficiently reorganize computations and skip unnecessary calculations based on different inputs. We propose memory access primitives \sload{} and \swrite{} to efficiently implement dynamic data virtualization (\S\ref{sec:sload}). \sysname{} utilizes Sparse-Dense Transform to ensure the correctness of GPU kernel computations before and after dynamic virtualization.

Previous papers\cite{} have attempted to achieve efficient computation in shared memory by rearranging data in global memory. However, these methods require extensive offline preprocessing and lack the flexibility to dynamically rearrange data based on input features.

\end{comment}

\begin{comment}
    
\subsection{\sload{} and \swrite{}}\label{sec:sload}
In order to leverage Sparse-Dense Transformation and achieve efficient online dynamic data rearrangement, we propose a set of memory access primitives, namely \sload{} and \swrite{}. \sload{} and \swrite{} fuse the process of data rearrangement into the cross-memory-hierarchy data loading (e.g., from Global memory to shared memory) or writing, thus introducing almost no extra overhead. Specifically, \sload{} loads the scattered data blocks from Global memory and places them contiguously in shared memory, while \swrite{} reverses the process by writing the computed results back to Global memory at discrete addresses in blocks, as shown in \autoref{fig:overview}. Given an expression of a Dense Kernel, \sysname{} first identifies all axes that can exhibit the properties of Sparse-Dense Transformation and applies \sload{} and \swrite{} on the corresponding axes to generate the corresponding sparse kernels. When \sload{} or \swrite{} is applied on an axis, \sysname{} replaces the Global memory address with a newly computed address by the sparse index, while keeping the address of the written Shared memory unchanged.
\begin{figure} [t]
\centering

\begin{minted}[
breaklines=true,
frame=lines,
fontsize=\footnotesize,
linenos=true,
xleftmargin=2em,
escapeinside=!!
]{c}
/*Inputs and Output are in global memory*/
__global__ void SparseKernel( !\label{line:sparsekernel}!
    struct SparseTensors Inputs, 
    struct Tensor Output
){
    /* size and format of SinDense, SoutDense
       in shared memory are decided by
       DenseComputeTile
    */
    DeclareSharedMem(SinDense, SoutDense);
    SLoad(Inputs, SinDense, blockIdx); 
    DenseComputeTile(SinDense, SoutDense); !\label{line:densecomp}!
    Swrite(SoutDense, Output, blockIdx);
}
\end{minted}
\vspace{-0.5cm}
\caption{The kernel skeleton based on \sload{} and \swrite{}.}
\label{fig:stile_kernel}
\end{figure}

The design of \sload{} and \swrite{} naturally decouples data and computation in sparse kernels, providing a new sparse computation paradigm: data rearrangement combined with dense computation, as shown in Figure \ref{fig:stile_kernel}. The decoupled computation is performed on dense data in shared memory, eliminating the overhead of sparse index encoding and decoding. Additionally, within a Tile, the efficient memory access patterns of Dense Macro Kernels can be reused to avoid bank conflicts during the shared memory access. Compared to the original Dense computation (line \ref{line:densecomp}), the additional overhead of the new sparse  kernel is only \sload{} and \swrite{} (line \ref{line:sparsekernel}). However, the data rearrangement process in \sload{} and \swrite{} is fused into data movement across memory hierarchies. As long as the granularity of the moved data block can saturate a memory transaction (32 bytes for CUDA GPU), data rearrangement incurs almost no additional overhead. In this case, reading and writing sparse data blocks does not waste memory bandwidth, and the performance is almost consistent with reading or writing dense data blocks. Additionally, \sload{} and \swrite{} further enable zero-copy of sparse data (\S\ref{sec:fast_index}). Because the required data blocks for computation can be directly loaded from the original Tensor into shared memory via \sload{}, no additional operator is required to transform the input Tensor format.
\end{comment}
%As long as the read/write of data tile aligns memory transaction, the on-the-fly data rearrangement across memory hierarchies between scattered data tiles and the condensed format induces no overhead.

% \para{Computation invariance.} The example \stile{}s in \autoref{fig:stile} imply that the size and placement of data tiles cannot be arbitrary. They follow a constraint, \ie after the data tiles are condensed along their dimensions to be a dense matrix, the dense computation should be able to run on the dense matrix correctly. Formally, for a dense operator $C=op(A,B)$, the implementation of $op$ can be applied on the condensed data $T_A$, $T_B$ from scattered data tiles without any change. This is defined as computation invariance. Then, the problem is \textit{what kind of data rearrangements (\ie \stile{}) satisfies computation invariance.}

% %To unveil all the \stile{}s systematically, 
% We derive feasible data rearrangements from operator expression (\eg einsum~\cite{}). An operator expression specifies how the output value is computed from the values of input tensors, \eg $C[m,n]$+=$A[m,k]*B[k,n]$ of Matmul. To guarantee computation invariance, sparse matrix (\eg $A$ becomes sparse) can only be rearranged along dimensions (\eg $M$ dimension). That is, the indices of the kept elements on a dimension can be mapped with a function $f$ to a dense sequence $0 \sim (l-1)$, where $l$ is the number of the kept elements. After data rearranged with the mapping function $f$, the computation on the data still follows the operator expression.



% The mapping functions cannot be arbitrarily applied on tensor dimensions. 

% To obtain the most efficient \stile{}s, the operator expression and its sparsity should be preprocessed. The operator expression should be simplified by merging logically the same dimensions. For example, multi-dimension tensor for element-wise operator can be simplified to a single dimension tensor, which makes \stile{} constrained by a single dimension instead of multiple. The sparsity on the tensors of the operator expression should be fully propagated by the approach in SparTA~\cite{sparta}. [XXX: shall we elaborate the approach in SparTA for this part?]

% %Computation invariance is intrinsically aligned with tensor expression (). When an operator is Computation invariance means in tensor expression (\eg einsum~\cite{}) the dimensions can be transformed with a mapping function. Most operators in deep learning can be expressed with tensor expression (\eg einsum~\cite{})


\begin{comment}
\begin{algorithm}[t]
\caption{The kernel skeleton based on \stile{}.\label{alg:stile_kernel}}
\KwData{$G_{sparseIn}$: Sparse input tensors stored in global memory.}
\KwResult{$G_{Out}$: Output tensor stored in global memory.}
\SetKwProg{Fn}{Function}{:}{}

\Fn{SparseKernel($G_{sparseIn}$, $G_{Out}$)}{ \label{line:sparsekernel}
    \tcc{\footnotesize size and format of $S_{denseIn}$, $S_{denseOut}$ in shared memory are decided by \textit{DenseComputeTile}}
    \_\_shared\_\_ $S_{denseIn}$, $S_{denseOut}$\;
    \sload{}($G_{sparseIn}$, $S_{denseIn}$, $blockIdx$) \tcp*{one thread block}
    DenseComputeTile($S_{denseIn}$, $S_{denseOut}$)\; \label{line:densecomp}
    \swrite{}($S_{denseOut}$, $G_{Out}$, $blockIdx$)\;
}
\end{algorithm}
\end{comment}
% \begin{comment}
% \end{comment}

% the granularity of sparse data that is friendly to hardware read transaction (in some cases, the data is more aligned after sparse index reconstruction)
% reduce the overhead of data rearrangement, directly pick out the effective data
% SLoad and SWrite can be independently implemented and connected to the dense tile computation

%\para{On-the-fly data rearrangement.} \sload{} and \swrite{} works on data rearrangement when the data is moving from global memory to shared memory and in reverse. As long as the data tile could saturate read/write transaction of the memory (\eg 32 bytes in CUDA GPUs), the data rearrangement would introduce little overhead, because the loading of sparse data tiles does not waste memory bandwidth. Thus, its performance almost equals to that of moving data across memory hierarchies in traditional dense computation. This property further enables \textit{zero-copy} of sparse data in online dynamic sparsity scenario (detailed in \S\ref{sec:fast_index}), because the effective data tiles can be directly selected from their original data format and written to the higher level memory with the desired format.

% \sysname{} determines the most suitable \stile{} by balancing its computation efficiency and the wasted computations.
% Determining the most suitable \stile{} is balancing \stile{}'s computation efficiency and the wasted computation.
% with the following formula: $$(Compute_{wasted}+Compute_{effective}) \times Cost_{stile},$$
% where $Compute_{wasted}$ means the number of FLOPS that are wasted by covering the non-zero values with the chosen data tile.
%Thus, different sparsity granularity has its most suitable \stile{}. For example, small granularity may prefer the \stile{} with smaller data tile. Though the corresponding dense computation tile is slightly less efficient, the wasted computation is also smaller. The granularity is not necessarily the same as the data tile of the chosen \stile{}.

% The essence of model pruning is sparsifying data blocks in the tensor. However how to translate sparse data blocks into efficient sparse computation is quite challenging. As introduced in Section~\ref{sec:moti}, the computation kernel on GPU are made up of two levels of parallel units: threads and thread blocks. Threads are grouped into large set of threads called thread block and the set of thread block that make up a kernel is called a grid. %Therefore, the sparse computation kernel also have two different sparse ways: sparse grid or the sparse thread block.
% If the sparse computation is sparsified at the thread level, then the kernel will launch all the thread blocks and each thread block perform a sparse computation based on corresponding sparse indexes. In this way, threads within the same block may perform different execution due to the sparse indices which may cause the divergence and lead to performance degradation. More importantly, sparse indices within the thread block also causes lots of random memory access and lead to poor memory bandwidth utilization and serious memory bank conflicts. In contrast, sparsifying the computation kernel at the thread-block level will skip the sparse thread block and the remaining blocks are calculated in dense. In this case, though the computation within the thread block is contiguous and efficient, the computation tile size of thread blocks is limited by the granularity of sparsity blocks. \NX{Explain why the block size is limited here?}. Small computation tile sizes may not be able to saturate the SM and lead to poor performance. To solve the problems above, we therefore propose the sparse computation tile(\stile{}) to bridges sparsity granularity and sparse computation efficiently.

% \begin{figure*}[htbp]
% 	\centering
% 	\includegraphics[width=1.98\columnwidth]{Figure/stile_k_axis_exp.pdf}
% 	\caption{\label{fig:stile_k_axis} Example of matrix multiplication \stile{} on K axis.}
% \end{figure*}
% %\begin{figure}[htbp]
% %	\centering
% %	\includegraphics[width=0.95\columnwidth]{Figure/stile_k_axis.pdf}
% %	\caption{\label{fig:stile_k_axis} Example of matrix multiplication \stile{} on K axis.}
% %\end{figure}
% %\begin{figure}[htbp]
% %	\centering
% %	\includegraphics[width=0.9\columnwidth]{Figure/stile_m_axis.pdf}
% %	\caption{\label{fig:stile_m_axis} Example of matrix multiplication \stile{} on M axis.}
% %\end{figure}
% \begin{figure*}[htbp]
% 	\centering
% 	\includegraphics[width=1.98\columnwidth]{Figure/stile_m_axis_exp.pdf}
% 	\caption{\label{fig:stile_m_axis} Example of matrix multiplication \stile{} on M axis.}
% \end{figure*}

% Figure~\ref{fig:stile_k_axis} shows an example of \stile{} of matrix multiplication on the K reduction axis. In this example, the shape of matrix A and B are $M\times K$ and $K\times N$ respectively. Besides. the matrix A is sparse and the green blocks represent the remaining non-zero values given by the pruning algorithm. Each thread block is responsible for computing a portion of the C matrix (marked in red). In general, \stile{} loads the data from global memory according to the sparse indexes and store the data in shared memory continuously. Leveraging the original dense computation tile, \stile{} then compute the corresponding output efficiently and write the results back to the global memory. There are two main factors that affect the performance of \stile{}: computation efficiency and read or write efficiency of the global memory. By remaining the original dense computation logic, the computation of \stile{} can be as efficient as the original dense tile. For the efficiency of global memory loading and writing, as long as the size of sparsity granularity can saturate the memory transaction, we can achieve the memory load or write performance close to original dense computation tiles, It's worth noting that for the skinny sparsity granularity, such as $32\times 1$, we can still saturate the memory transaction by changing the layout of A (from row-major to column major) or inserting a transpose operator. 

% To generate the code of \stile{} efficiently, we introduce two primitives: \sload{} and \swrite{} to represent the sparse memory loading or storing according to the sparse indexes. Line \ref{alg:sload_interface}, \ref{alg:swrite_interface} in Algorithms~\ref{alg:stile_construct} shows the interfaces of \sload{} and \swrite{}, where $dst$ and $src$ are the destination and source memory address respectively, and $loop$ represents the loop axis annotated to sparse.
% During the code generation, \sload{} and \swrite{} will translate memory address based on the sparse indexes automatically. As shown in the Figure~\ref{fig:stile_k_axis}, after applying \sload{} on the k-axis of the original dense matrix multiplication, \sysname{} replace the original dense loop accordingly when loading data from the global memory, as shown in the right side of the Figure~\ref{fig:stile_k_axis}.
% %\NX{shall we give an code generation example here?}

% \NX{introduce the computation consistency here?}
% \textbf{Calculation consistency}. \stile{}s should have the same calculation logic with corresponding dense computation tile to reuse the computation part in these efficient dense tiles. We call this \stile{} remains the calculation consistency with its corresponding dense tile. 
% To leverage the original dense computation tile, we need to maintain the consistency with its original calculation logic after applying \sload{} and \swrite{}. Which axes can be annotated with \sload{} or \swrite{} to ensure the calculation consistency is determined by the calculation logic of the original dense tiles. 
% As shown in Figure~\ref{fig:stile_k_axis}, matrix multiplication can apply \sload{} on the K-axis and leverage original dense computation without affecting the correctness. The middle of Figure~\ref{fig:stile_m_axis} shows a dense computation tile where each thread block compute submatrix multiplication of $BLOCK\_M\times BLOCK\_K \times BLOCK\_N$. Compared with the dense computation tile in Figure~\ref{fig:stile_k_axis}, the dense computation tile in Figure~\ref{fig:stile_m_axis} is further tiled on the K reduction axis and each thread block only traverses a part of the k-axis. As shown in the right side of Figure~\ref{fig:stile_m_axis}, \stile{} can still leverage the efficient dense computation by applying the \sload{} and \swrite{} on the M axis at the same time.
% Therefore different computation dense tiles may generate different \stile{}s accordingly.

% \textbf{Generating \stile{}s}. Algorithm~\ref{alg:stile_construct} shows the details of the \stile{} construction in \sysname{}. \sysname{} first builds a computation tile database that consists of manually designed dense computation tiles (such as openai\cite{}) or the dense tiles generated by the compilers, such as TVM\cite{tvm}. \sysname{} loads all dense computation tiles from database offline. For each dense computation tile, \sysname{} first parse out all axes in this tile and try to annotate \sload{} or \swrite{} on all possible combinations of axes. \sysname{} will check whether the \stile{} still remains calculation consistency with original dense computation tile. If so, the current \stile{} can reuse the efficient dense calculation part with original dense computation tile. \sysname{} use random data and random sparse indexes to verify whether the generated \stile{} still remains the calculation consistency with original dense tile. Specifically, \sysname{} generate and compile the code for \stile{} and corresponding dense tile. It then runs the dense operator and sparse operator with random data and sparse indexes. If the output of two operators is always the same under different random data and sparse indexes, then the generated \stile{} is legal.


% \NX{The implementation of the function $remainConsist$: random data driven based or the rule based}.
%\NX{Given the efficient dense tiles, how to generate the sparse tiles from the given dense computation tiles.}
%\stile{} is constructed of the efficient dense computation tile and \sload{} and \swrite{} primitives. \sload{} and \swrite{} build the memory address mapping from the global memory to the shared memory according to the sparse indexes. Specifically, when \sload{} or \swrite{} is applied to a dense loop, . By remaining the original dense computation logic, \stile{} can be as efficient as the original dense tile. \stile{}. 

%\NX{Sparse grid vs sparse block.}
%The essence of model pruning is setting (or removing) some data blocks to zero in the tensor and sparse kernels skip these data blocks during the calculation. However, calculation. After pruning, the data blocks in the origin tensors that need to be calculated are discrete and randomly distributed. Such discrete and randomly distributed data blocks make sparse kernel quite hard to be optimized: First, random memory access leads to underutilization of memory transaction size and wastes the memory bandwidth.
% \NX{Stile also access in the random pattern}

% \begin{algorithm}[t]
% \caption{\stile{} Construction \label{alg:stile_construct}}
% \KwData{$D_{Tile}$: Dense computation tiles loaded from the database}
% \KwResult{$S_{Tile}$: Sparse computation tiles generated from $D_{Tile}$}
% \SetKwProg{Fn}{Function}{:}{}
% \
% parse\_axes($dense_{tile}$); // parse out all axes in dense tiles \;
% remainConsist($Tile_d$, axes, stype);// check if the \stile{}s can remain the computation consistency\;
% \sload{}(dst, src, loop) \; \label{alg:sload_interface}
% \swrite{}(dst, src, loop) \; \label{alg:swrite_interface}
% \
% \Fn{Generate\stile{}($D_{Tile}$)}{ \label{alg:generate_stile}
%     $S_{set}$ = set()\;
%     \ForEach{$d \in D_{Tile}$}{
%         axes = parse\_axes($d$)\;
%         \ForEach{$S_a \in$ permutation(axes)}{
%             \If{remainConsist($d$, $S_a$, \sload{})}{
%                 $S_{set}$.insert(\stile{}($d$, $S_a$, \sload{}))            
%             }
%             \If{remainConsist($d$, $S_a$, \swrite{})}{
%                 $S_{set}$.insert(\stile{}($d$, $S_a$, \swrite{}))            
%             }
%             \If{remainConsist($d$, $S_a$, \sload{} \textbf{ and } \swrite{})}{
%                 $S_{set}$.insert(\stile{}($d$, $S_a$, \sload{} \textbf{ and } \swrite{}))            
%             }
%         }
%     }
%     \KwRet $S_{set}$
% }
% \end{algorithm}
\begin{comment}
    
\subsection{Online Sparsity Detection}\label{sec:fast_index}\label{sec:design_online}

As sparsity continuously changes with input, \sysname{} performs online detection of sparsity and constructs a sparse index. To improve the efficiency of online sparsity detection, we propose an efficient dynamic sparse representation and a mechanism for quickly constructing sparse indexes.

%\stile{} is the building block of the computation. To deal with dynamically changing sparsity, the sparsity should be captured online and translated to \stile{}. To facilitate this online process, we propose an enhanced representation of dynamic sparsity, which is for users to specify the sparsity of the tensors in each forward pass of model execution.

\para{Representation of dynamic sparsity.}
Our dynamic sparse representation comprises two parts: sparsity granularity and a binary sparsity attribute matrix. This representation can be annotated to any axis or combination of axes in a tensor. Each value in the sparse attribute matrix corresponds to a data block of the same size as the annotated sparsity granularity. Notably, multiple sparsity granularities can be used in the same dynamic sparse representation, such as when specifying sparsity for sentences of different lengths in the same batch. Assuming the input tensor has shape $[B, M, H]$, where $B$ is the batch size, M is the length of the longest sentence in the batch, and H is the hidden dimension size, we can annotate an array of length $B$ on the first dimension: [$(S_{dim1}, \ldots , S_{dimN})$], where $S_{dimN}$) represents the length of the Nth sentence. This sparse representation is flexible enough to efficiently represent dynamic sparsity while using less memory and naturally fits the property of \property{} that rearrange data along an axis.

\para{Sparse Index Construction}
With \property{}, \sload{}, and \swrite{}, the sparse kernels generated by \sysname{} no longer require the sparse indices to be sorted along a certain axis. This greatly reduces the constraints on building sparse indices, allowing us to construct them with minimal synchronization overhead. For example, in the original BCSR format, the column indices of non-zero elements in the same row had to be sorted, which resulted in significant synchronization overhead, especially on GPU accelerators. However, in \sysname{}, after tiling, each tile only needs to traverse the corresponding region to check for non-zero values and write the unordered column indices to the corresponding position in the row through atomic operations. Therefore, \property{}, \sload{}, and \swrite{} enable \sysname{} to achieve efficient tiling and extremely low synchronization overhead. Furthermore, \sysname{} only builds sparse indices online without copying data. At runtime, sparse kernels use \sload{} to directly read from the original tensor based on the constructed sparse index. This greatly reduces the memory access overhead introduced by data format conversion (from dense to BCSR) and achieves zero-copy data rearrangement.

\end{comment}

%The representation is a sparsity attribute that can be efficiently constructed and parsed while consuming less memory. The sparsity attribute combines a 0-1 attribute matrix along with a sparsity granularity. Each value in the attribute matrix represents the existence of a data block which is the size of the sparsity granularity. It can express different types of dynamic sparsity. One type is that the location of sparse values keeps changing while the granularity is the same (\eg in model pruning~\cite{nn_pruning, li2020train}). Another type allows the granularity to change. For example, to specify the sparsity of a batch of sentences with different lengths, the sparsity attribute of \sysname{} allows each sentence to have its own granularity, \ie $1 \times L$ where $L$ is the length of this sentence. Formally, the sparsity granularity is in the form of $(S_{dim1}, \ldots , S_{dimN})$, where $S_{dim}$ is the size of the granularity on dimension $dim$. The representation not only makes the sparsity attribute much smaller, but also aligns with the design of \property{} which transforms data along dimensions.

% To optimize the deep learning model with changing sparsity, users should specify the sparsity of the sparse tensors in an online manner during model execution. Unlike SparTA, which uses the sparsity attribute (\ie TeSA) only at compile time, in dynamic sparsity the attribute tensors for expressing changing sparsity become a part of the model, which is located in the critical path of model execution. It requires the sparsity attribute to be efficiently constructed and parsed, while consuming less memory. Thus, we design \dtesa{} to combine the sparsity attribute matrix with  sparsity granularity. With sparsity granularity, each value in the attribute matrix represents the existence of a data block instead of an element. \dtesa{} can express different types of dynamic sparsity. One type is that the location of sparse values keeps changing while the granularity is the same (\eg in model pruning~\cite{nn_pruning, li2020train}). In another type, the granularity could also change. For example, in the language models the sequence length of input data samples is different. Padding them to the maximum length induces sparsity, where sparsity granularity in \dtesa{} could efficiently express this sparsity, \ie each sample has its own sparsity granularity as large as its sequence length. Formally, the sparsity granularity is in the form of $(S_{dim1}, S_{dim2})$, where $S_{dim}$ is the size of the granularity along dimension $dim$. The granularity not only makes the sparsity attribute much smaller, but also aligns with the \stile{} abstraction which will be demonstrated below.

%\para{Translating dynamic sparsity to \stile{}.}
%During online model execution, \sysname{} detects the annotated sparsity and builds the index of the non-zero blocks in every sparse tensor. The non-zero blocks are in the granularity of the data tile of the chosen \stile{} in \autoref{alg:stileopt}. The blocks are translated into a bunch of \stile{}s in an online manner. The design of \stile{} accelerates the index construction and the computation translation.
%and efficiently parsed by \sload{} and \swrite{}. The constructed index can be in any sparse data format, \eg BCSR~\cite{sparse_formats} used in our system.
%\sysname{} constructs the sparsity index in an out-of-order manner, because the permutation invariant property relaxes the order of the indices in a sparse data format. For example in BCSR~\cite{sparse_formats}, the column indices of non-zero elements in each row should be ordered, which induces considerable synchronization overhead especially in GPU accelerators. Permutation invariant allows the column indices to be written in any order, thus, eliminates the synchronization overhead. Unlike traditional sparse data format which has data in it, \sysname{} only constructs index while leaving the data as is. The index directly references the data blocks in their original tensor. \stile{} uses the index to load the data blocks across memory hierarchies (\eg from global memory to shared memory in GPU) and rearranges the data blocks on-the-fly into the dense format. It greatly reduces the overhead of data conversion (\eg from dense format to BCSR), enabling zero-copy data rearrangement.
%On the other hand, with zero-copy data rearrangement, we can only build the index without copying the non-zero values. This is different from the traditional sparse data conversion where the non-zero values should be copies into the value region of the BCSR format. In our index construction, the index directly references the data blocks of the original tensor. It has no impact on the follow-up computation, because the data tiles are aligned with memory's read/write transaction. With the two optimization techniques, the index construction becomes very efficient. Though located in the critical path, it induces little overhead to the execution of dynamic sparsity.
% zero-copy; out of order

% \begin{figure}[htbp]
% 	\centering
% 	\includegraphics[width=0.95\columnwidth]{Figure/converter.pdf}
% 	\caption{Workflow of the fast index constructor.}
% \end{figure}

\subsection{PIT Transformation Policy}\label{sec:pit_policy}

The PIT transformation policy aims to find an optimal transformation for a given sparse operator by creating a mapping between sparse data and a hardware-favored computation unit. To address online sparse computation requirements, the transformation must achieve low data conversion overhead and high hardware utilization. Consequently, we develop an axis-wise PIT transformation policy that meets both criteria, based on the permutation invariant property~\cite{lee2019set}. By analyzing the permutation invariant property of deep learning operators, we determine all feasible permutations for each operator. These permutations result in various micro-tile configurations, and we design a micro-tile selection policy to choose the most suitable configuration for each sparse operator.

%\sysname{} is a generic compiling framework for dynamic sparsity, that transforms sparse computation into hardware efficient dense computation. To make the transformation efficient, we propose permutation invariant transformation that is generally applicable to deep learning operators. It generates permutation rules for each operator. For the candidate permutation rules, the transformation policy pick the best permutation rules depending on the operator type and sparse tensor samples.

% In this chapter, we first introduce a mathematical property called \adjp{}~\cite{balan2022permutation}, and use it to derive a related property called \property{} in Tensor Expressions (abbreviated as TE).

%\subsection{Axis-wise Permutation Invariant Transformation} \label{sec:permutation}

\begin{table}[t]
    {\centering
    \footnotesize{
    \begin{tabular}{l|c}
    \Xhline{2\arrayrulewidth}
    \textbf{Operator} & \textbf{Tensor Expression} \\ \hline
    ReduceSum & $C[p]$ += $A[p, l]$ \\
    Vector Addition & $C[p]$ = $A[p]$ + $B[p]$ \\
    MatMul & $C[m,n]$ += $A[m,k]$ * $B[k,n]$ \\
    BatchMatmul & $C[b,m,n]$ += $A[b,m,k]$ * $B[b,k,n]$ \\
    Convolution & $C[n,f,x,y]$ += $A[n,m,x+i,y+j]$ * $B[f,m,i,j]$ \\ \hline
    \end{tabular}}
    \par}
    \caption{Example tensor expressions.\label{tab:expression}}
     %\vspace{-0.5cm}
\end{table}

\para{Axis-wise Permutation Invariant Transformation}
The computation of deep learning operators primarily revolves around tensor axes. Most of the operators can be represented using Einstein summation (einsum) notation~\cite{}, which expresses the operations along tensor axes.
\autoref{tab:expression} lists some common operators in deep learning and their corresponding einsum notation.
We observe that shuffling the indices along certain axes does not affect the correctness of the operator. For example, in Vector Addition, we can permute the $p$-axis arbitrarily and still obtain the same result. We refer to such axes as having the \adjp{} property. We introduce \adjp{} into einsum notation and formally define it as follows:

\begin{definition}
\label{defn:adjp}
In a tensor expression $Y \leftarrow f(X_1,\ldots,X_n)$, where $f$ is an operator, $X_i$ and $Y$ are its input and output tensors respectively. An axis $k$ in the operator is \adjp{} if it satisfies:
\begin{equation}
\label{eq:PI}
\begin{aligned}
    &\forall~\mathcal{P}\in \Phi_{k}, ~\exists~\mathcal{P^\prime} \in \Phi_{k}\\
    s.t.~~&\mathcal{P^\prime}(f(\mathcal{P}(X_1),\ldots,\mathcal{P}(X_n)) = Y,
\end{aligned}
\end{equation}
where $\Phi_{k}$ is the set of all permutation functions on $k$ axis. $\mathcal{P}(X)$ means a permutation function $\mathcal{P}$ is applied on the $k$ axis of the tensor $X$, to shuffle the elements on $k$ axis to a new order. If $k$ axis does not exist in $X$, $\mathcal{P}(X)=X$.
\end{definition}

The intuitive explanation of this definition is that for an axis $k$ that is \adjp{}, if we permute the $k$ axis of the input tensor, there must exist a corresponding inverse permutation on the $k$ axis of the output tensor to ensure that the input-output tensors remain the same before and after the permutation. 
This definition implies that applying a permutation does not necessitate altering $f$'s specific computation implementation, thereby preserving computation efficiency. Sparse operators can exploit this property to consolidate sparsely located non-zero values, enabling the use of kernel implementations designed for dense tensors.
% Given a dimension $k$ of a tensor expression, if some of its elements are dropped (masked), this dimension is defined as a sparse dimension and the dropped elements are called redundant elements. With permutation invariant, we can construct a permutation function $\mathcal{P}$ to move all the redundant elements to the end while all the non-redundant elements to the front. The redundant elements can be safely removed to build a shorter $k$ dimension.
% Such transformation is denoted as \property{}, it builds a connection between sparse and dense computation, brings the opportunity of leveraging dense computation kernels for sparse computation.

%Permutation invariant dimensions are ubiquitous in deep learning computations. 
We conduct a systematic study of all possible axis-wise permutations for deep learning operators that can be represented using one or multiple einsum notations. For clarity, we focus on simplified einsum notation, which involves removing common axes present in all tensors (\eg $p$ and $b$ in \autoref{tab:expression}) and merging duplicate axes into one (\eg $m$ and $k$ in $C[m,k,n]$ += $A[m,k,l]$ * $B[l,n]$). In simplified einsum notations, there are two types of axes: the spatial axis, which appears in the output tensor, and the reduction axis, which is absent from the output tensor. The following theorem identifies the axes that are permutation invariant.

\begin{theorem}\label{theorem:commutative}
    An axis is permutation invariant, if and only if the computation on the axis is commutative and associative.
\end{theorem}
\noindent The theorem is mostly self-evident, and we omit the proof due to space constraints. Most computations on the reduction axis are commutative and associative (\eg sum, multiply, max, min). The spatial axis is also commutative and associative, as it only controls data layout and does not involve computation. However, some axes are not commutative, such as the axis "$x+i$" and "$y+j$" of Convolution in \autoref{tab:expression}. These two axes and the involved $x$, $i$, $y$, and $j$ axes are not permutation invariant.

\begin{figure}[t]
	\centering
	\includegraphics[width=1.0\columnwidth]{Figure/pit.pdf}
	\caption{\label{fig:pit} Permutation on two axes of a tensor $T$. $p_i^k$ means the $i$-th permutation function on $k$ axis. To maintain computation efficiency, one axis allows only one permutation function, while different pieces of the tensor could have their own permutation functions.}
\end{figure}

For a multi-axis einsum notation, various permutation options may exist. As illustrated on the left of \autoref{fig:pit}, multiple axes (\eg $m$ and $k$ axes) can undergo permutations jointly. One axis could have multiple permutation functions (\eg $p_1^k$ and $p_2^k$ on $k$ axis). \autoref{theorem:efficiency} identifies all the permutations that maintain the computation efficiency of $f$. In modern accelerators, computation efficiency is essentially determined by the ratio of FLOPs to memory access. Since permutation does not alter an operator's FLOPs, we use memory access $R_A:R_B:W_C$ to represent computation efficiency for simplicity, where $R_A$ and $R_B$ are the amounts of data read from operands $A$ and $B$, respectively, and $W_C$ is the amount of data written to the output tensor $C$.

\begin{theorem}\label{theorem:efficiency}
    To maintain the computation efficiency of $f$, each permutable axis of an einsum notation can have at most one permutation function.
\end{theorem}
\begin{proof}[Sketch Proof]
\autoref{theorem:commutative} suggests that each permutable axis can have a permutation function while maintaining the ratio $R_A:R_B:W_C$. By applying permutations to permutable axes sequentially, it becomes evident that multiple axes can have their own permutation functions simultaneously. Each permutable axis can have at most one permutation function. If a reduction axis has two permutation functions (\eg $p_1^k$ and $p_2^k$ on the $k$ axis in \autoref{fig:pit}), the combination of these functions spans more indices on the $k$ axis than a single function, resulting in the need to read more elements from the indices of the other operand. This changes the ratio $R_A:R_B$. Similarly, combining two permutation functions on a spatial axis leads to writing more elements in the output tensor, which alters the ratio $R_A:W_C$.
\end{proof}

The axes removed during notation simplification are not constrained by \autoref{theorem:efficiency}, allowing elements on the removed axes to have independent permutation functions. For instance, in \autoref{tab:expression}, the matrix $A[i,:,:]$ in BatchMatmul can be independently permuted, \eg having its own permutation functions on the $m$ and $k$ axes. Similarly, in ReduceSum, each $A[i,:]$ vector can have its own permutation function on the $l$ axis.

Crucially, when combining \autoref{theorem:efficiency} with the tiling technique in deep learning compilers, each tile can possess unique permutation functions. The tile size and corresponding permutations dictate the micro-tile size. For instance, a 32x32 tile with a permutation function on its first axis results in a 1x32 micro-tile, while a 64x64 tile yields a 1x64 micro-tile. When permutations are applied to both axes, micro-tiles become smaller (\eg 1x1) and must align along the axes, as illustrated on the right of \autoref{fig:pit}. It is essential to select the most suitable micro-tile for a given sparse operator.

% We study the permutation invariant of tensor dimensions by classifying the dimensions into three categories: sporadic dimension, prevalent dimension, and compound dimension. 1) Sporadic dimension is the dimension that exists in one or more tensors of a tensor expression, but does not span in all tensors. For example, $m$, $n$, $k$, $f$, $l$ of the tensor expressions in \autoref{tab:expression} are sporadic dimension. 2) Prevalent dimension is the dimension that exists in all the tensors (\ie input and output tensors) of a tensor expression. Examples of prevalent dimension are $p$ and $b$ in \autoref{tab:expression}. 3) Compound dimension is the dimension that is involved in an arithmetic expression. For example in \autoref{tab:expression}, $x$ and $i$ in Convolution are involved in the arithmetic expression $x+i$. Similarly, $y$ and $j$ are involved in $y+j$. Thus, $x$, $y$, $i$, and $j$ are compound dimension.

% Permutation invariant has different application rules for different types of dimension. First, when permutation invariant is applied on only one dimension of a tensor expression, the dimension can be sporadic dimension or prevalent dimension, but not compound dimension. Because permuting a compound dimension violates its corresponding arithmetic expression. Second, when permutation invariant is applied on multiple dimensions of a tensor expression, there are two application rules: 1) When the permuted dimensions are all sporadic dimension, each dimension can only have a single permutation function. For example, a tensor $X[i,j]$ where $i$ and $j$ are sporadic dimension, the permutation function for each vector $X[i,:]$ (\ie on $j$ dimension) should be the same. 2) When the permuted dimensions include a prevalent dimension, the permutation function on each element of the prevalent dimension could be different. For example, a tensor $X[i,j]$ where $i$ is prevalent dimension, the permutation function for each vector $X[i,:]$ can be different. This is because the computation on each element of prevalent dimension has no data dependency.

% \para{\property{}.} The permutation invariant offers extra opportunities to efficiently handle sparsity. Given a dimension $k$ of a tensor expression, if some of its elements are dropped (masked), this dimension is defined as a sparse dimension and the dropped elements are called redundant elements. With permutation invariant, we can construct a permutation function $\mathcal{P}$ to move all the redundant elements to the end while all the non-redundant elements to the front. The redundant elements can be safely removed to build a shorter $k$ dimension.
% Such transformation is denoted as \property{}, it builds a connection between sparse and dense computation, brings the opportunity of leveraging dense computation kernels for sparse computation.

% \subsection{Dynamic Sparsity Representation} \label{sec:dtesarepr}

%statistic granularity and online sparsity attributes, reasons. provided online by user. the granularity can be a variable.

% To optimize the deep learning model with changing sparsity, users should specify the sparsity of the sparse tensors in an online manner during model execution. Unlike SparTA, which uses the sparsity attribute (\ie TeSA) only at compile time, in dynamic sparsity the attribute tensors for expressing changing sparsity become a part of the model, which is located in the critical path of model execution. It requires the sparsity attribute to be efficiently constructed and parsed, while consuming less memory. Thus, we design \dtesa{} to combine the sparsity attribute matrix with  sparsity granularity. With sparsity granularity, each value in the attribute matrix represents the existence of a data block instead of an element. \dtesa{} can express different types of dynamic sparsity. One type is that the location of sparse values keeps changing while the granularity is the same (\eg in model pruning~\cite{}). In another type, the granularity could also change. For example, in language model the sequence length of input data samples is different. Padding them to the maximum length induces sparsity, where sparsity granularity in \dtesa{} could efficiently express this sparsity, \ie each sample has its own sparsity granularity as large as its sequence length. Formally, the sparsity granularity is in the form of $(S_{dim1}, S_{dim2})$, where $S_{dim}$ is the size of the granularity along dimension $dim$. The granularity not only makes the sparsity attribute much smaller, but also aligns with the \stile{} abstraction which will be demonstrated below.

%For optimizing the dynamically changed sparse model, the model's sparsity should be specified, \ie annotating tensors' sparsity attribute. Dynamic sparsity requires the sparsity to be annotated online by users, which brings more stringent requirement on the efficiency of sparsity optimization as it is located in the critical path of model execution. We extend TeSA by adding sparsity granularity, which changes from element-wise attribute to block-wise attribute. The granularity is specified with $(S_{dim1}, S_{dim2})$, where $S_{dim}$ is the size of the granularity along dimension $dim$. The granularity could be the same (\eg model pruning) and could also keep changing (\eg dynamic sequence length of language models) along the model execution. The granularity not only makes the sparsity attribute much smaller, but also aligns with the \stile{} abstraction which will be demonstrated below.

% \dtesa{} enables users to specify arbitrary sparsity pattern for given model including both static and dynamic sparsity. Figure~\ref{fig:dtesa} shows an example of \dtesa{}. \dtesa{} consists of two parts: elementwise static sparsity attribute and dynamic sparsity notations. \dtesa{} first enhances the original value tensor with an extra tensor with the same shape, where each element represents the static sparsity attribute of the corresponding values\cite{sparta}. In addition, \dtesa{} also includes the dynamic sparsity annotation to describe the dynamic sparsity pattern as shown in the right side of the Figure~\ref{fig:dtesa}. Specifically, \sysname{} provides two kinds of dynamic sparsity annotations: (1) $Granularity$ to describe the granularity of the dynamic sparsity (2) $Range$: to describe the position constraint. Both kinds of annotation are optional and can be annotated on any dimension or combination of dimensions. The \dtesa{} in Figure~\ref{fig:dtesa} means the upper left corner of the tensor is always 0 and some dynamic sparsity with granularity of $1\times 1$ are randomly distributed. In addition, user can also use variable in the $Granularity$ and $Range$ annotation. For example, in the case of dynamic sparsity caused by different sequence length, shown in Section~\ref{sec:eval_seqlen}, the $Granularity$ of dynamic sparsity is $seqlen\times seqlen$ and the $Range$ is $0:seqlen, 0:seqlen$. Here, $seqlen$ is a variable that represents the effective length of input sequences. Therefore, this \dtesa{} means we only need to calculate the submatrix of $seqlen\times seqlen$ in the upper left corner.

% \dtesa{} allows the user to specify arbitrary static and dynamic sparsity pattern and reveals the optimization opportunity of dynamic sparsity, especially for scenarios with potential dynamic sparsity, such as the dynamic sparsity in the pruning progress and caused by different sequence lengths (evaluated in Section~\ref{sec:eval_pruning}, \ref{sec:eval_seqlen}). More importantly, with \dtesa{}, \sysname{} can understand the characteristics of both the static and dynamic sparsity at the compile time, which enables corresponding sparsity optimizations. 


% \begin{figure}[htbp]
% 	\hfill
% 	\includegraphics[width=0.9\columnwidth]{Figure/DTeSA.pdf}
% 	\caption{\label{fig:dtesa} Example of \dtesa{}.}
% \end{figure}


%\QL{We can try the following logic flow to introduce \stile{}: 1) Efficient execution of (dynamic) sparsity requires fully utilizing hardware; 2) Making sparse computation aligned to hardware is the principle to achieve high efficiency; 3) We propose \stile{}, an abstraction that systematically opens up the effective mappings/alignments of various sparsity patterns to hardware; 4) the effective computation on hardware is abstracted by computation tile which has been well optimized and aligned to hardware; 5) The mapping can be online constructed for supporting dynamic sparsity.}

%\NX{Explain the stile abstraction and give several examples here}.
%\NX{For dynamic sparsity, the memory load efficiency actually need support from the converter.}

% one paragraph to introduce the necessary of stile
%Sparse computation, especially unstructured sparsity, can hardly well utilize the modern hardware which has increasing number of cores with SPMD instructions provisioned (\eg GPU). Its irregular data access makes data movement across memory hierarchies (\eg global memory to shared memory in GPU) less efficient. Its computations can hardly be grouped into SPMD instructions. Existing optimizations for sparse computation leverage special data layouts to mitigate the effect of the irregularity. However, their computation efficiency still lags far behind that of the dense computation of the same FLOPs, because of the intrinsic misalignment between sparse computation and modern vectorized hardware design. 

\para{Micro-tile Selection Policy}%\label{sec:selectionpolicy}
% \para{Optimizing \stile{} kernel.}
%The efficiency of the sparse kernel generated by \sysname{} is mainly determined by two factors: the efficiency of the dense kernel before applying \sload{} and \swrite{}, and the efficiency of converting dynamic sparsity in the input tensor to the target dense kernel. The computational efficiency of the dense kernel is mainly determined by the size of the computation tile and the access pattern of shared memory. A smaller computation tile may not fully saturate the computing resources. Carefully designed thread coordination can achieve data reading and writing without bank conflict on shared memory, greatly improving the efficiency of dense tiles. For different dense tiles, \sysname{} pre-builds a performance lookup table as a reference for selecting the dense kernel (see \section{implementation} for details).
\sysname{} first constructs a sparse kernel database offline, where each sparse kernel is obtained by applying PIT transformations on all possible combinations of permutation-invariant axes of the corresponding dense kernel. Specifically, assuming we have a dense Matmul kernel template that performs $[M, K]\times[K, N]$ matrix multiplication. The dense Matmul kernel has three permutation-invariant axes (\S\ref{sec:pit_policy}), therefore, we can derive $2^3-1=7$ corresponding sparse kernels from the target dense kernel. Each generated sparse kernel has its corresponding micro-tile granularity. To assist with the micro-tile online selection, \sysname{} builds performance lookup tables for the generated sparse kernels beforehand. (\S\ref{sec:implementation}).
%The efficiency of \sysname{}'s sparse kernel depends on two factors: the effectiveness of the dense kernel before using \sload{} and \swrite{}, and the efficiency of converting dynamic sparsity in the input tensor to the desired dense kernel. The efficiency of the dense kernel depends on the size of the computation tile and the access pattern of shared memory. Smaller tiles may underutilize computing resources, but carefully designed thread coordination can minimize bank conflicts when accessing shared memory and improve dense tile efficiency. To aid in selecting the dense kernel, \sysname{} pre-builds a performance lookup table for different dense tiles (\S\ref{sec:implementation}).

\begin{algorithm}[t]
\caption{Kernel selection for a dynamic sparsity operator.} \label{alg:selection}
\KwData{$Op$: A dynamically sparse operator,\newline
        $D_{sparse}$: A list of $n$ sparsity samples of $Op$.}
\KwResult{$Best$: The best computation tile for $Op$.}
\SetKwProg{Fn}{Function}{:}{}

\Fn{ChooseStile($D_{sparse}$, $Op$)}{ \label{alg:dynamic_opt}
    $Best$ = null; $Cost_{optimal}$ = inf\;
    \ForEach{$T \in$ GetTilesFromTileDB($Op$)}{
        \ForEach{$A \in$ GetPITAxis($T$)}{ \label{line:get_pit_axes}
            $Cost$ = 0\;
            \ForEach{$D \in D_{sparse}$}{
                $Num_{tiles}$ = CoverAlgo($D$, $T.micro\_tile$, $A$)\; \label{line:coveralgo}
                $Cost$ += $Num_{tiles} * T.tile\_cost$\;
            }
            \If{$Cost$ < $Cost_{optimal}$}{
                $Best$ = $S$\;
                $Cost_{optimal}$ = $Cost$\;
            }
        }
    }
    \KwRet $Best$\;
}
\end{algorithm}
\autoref{alg:selection} shows how \sysname{} selects the appropriate micro-tile and corresponding generated sparse kernel. \sysname{} iterates through the generated sparse kernels in the database and gets their axes where the PIT transformations are applied~\ref{line:get_pit_axes}. \texttt{CoverAlgo} (\autoref{line:coveralgo}) calculates the number of micro-tiles required to cover all non-zero values in the sparse tensor(denoted as $Num_{tiles}$). The time cost of the generated sparse kernel is estimated as $Num_{tiles}\times T.tile\_cost$ where $T.tile\_cost$ is the running time of the corresponding sparse kernel profiled offline. \sysname{} selects the sparse kernel with the smallest time cost and its corresponding micro-tile to perform the sparse computation online.
%For the second factor, if the input tensor has a small sparse granularity and the target dense computation tile is relatively large, some calculations may be wasted. Taking the matrix multiplication $A \times B$ as an example where $A$ has a shape of $M\times K$ and B has a shape of $K\times N$. Suppose the sparse granularity of $A$ is $16\times 1$. If we choose a dense tile of size $16\times32\times32$, i.e., each tile is computed on a $16\times32$, $32\times32$ sub-matrix and \sload{} and \swrite{} are applied on the M-axis. Then no calculations will be wasted when converting the dynamic sparsity in $A$ to the target dense tile. However, if we choose a dense tile of size $32\times32\times32$ and still apply \sload{} and \swrite{} on the M-axis, it requires using data blocks of size $32\times1$ to cover all non-zero blocks in A (shape 16x1), resulting in waste. Although larger tiles often saturate computing resources more easily, some waste may occur when converting sparsity to dense computation. \autoref{alg:selection} shows how \sysname{} selects the appropriate dense tile from the kernel database based on representative input samples. Specifically, \sysname{} traverses all dense computation tiles and calculates their cost. \texttt{CoverAlgo} (\autoref{line:coveralgo}) calculates the number of data blocks required to cover all non-zero values.

%As demonstrated in \S\ref{sec:stileabs}, there are various \stile{}s. The most efficient \stile{} for a sparse operator is determined mainly by two factors, \ie the efficiency of its associated dense computation tile and the operator's dynamic sparsity. For the first factor, though different-sized computation tiles are all dense, they have different computation efficiency. Usually, the smaller the computation tile is, the less efficient it is. Because it is harder to saturate all the available cores (\eg the cores in a SM~\cite{a100}). Some carefully designed coordination of threads could greatly improve the computation efficiency of small computation tiles, leading to many efficient small computation tiles~\cite{cuda}. These well-optimized computation tiles are stored in a tile database of \sysname{} and serve as the base of \stile{}s.

%For the second factor, all the \stile{}s can be applied to a given sparsity but lead to varied computation efficiency. If the data tile of an \stile{} is larger than the granularity of the given sparsity, a proportion of the computation is wasted. While if the data tile is much smaller than the sparsity granularity, the computation tile is not efficient. 
% \begin{algorithm}[t]
% \caption{Optimizing \stile{} kernel for a dynamically sparse operator.} \label{alg:stileopt}
% \KwData{$Op$: A dynamically sparse operator,\newline
%         $D_{sparse}$: A list of $n$ sparsity samples of $Op$.}
% \KwResult{$Best_{stile}$: The best \stile{} for $Op$.}
% \SetKwProg{Fn}{Function}{:}{}

% \Fn{ChooseStile($D_{sparse}$, $Op$)}{ \label{alg:dynamic_opt}
%     $Best_{stile}$ = null; $Cost_{optimal}$ = inf\;
%     \ForEach{$S \in$ GetStilesFromTileDB($Op$)}{
%         $Cost$ = 0\;
%         \ForEach{$D \in D_{sparse}$}{
%             $Num_{stiles}$ = CoverAlgo($D$, $S.data\_tile$)\; \label{line:coveralgo}
%             $Cost$ += $Num_{stiles} * S.tile\_cost$\;
%         }
%         \If{$Cost$ < $Cost_{optimal}$}{
%             $Best_{stile}$ = $S$\;
%             $Cost_{optimal}$ = $Cost$\;
%         }
%     }
%     \KwRet $Best_{stile}$\;
% }
% \end{algorithm}

% In online dynamic sparsity, the most suitable \stile{} is chosen based on several representative sparsity samples. \autoref{alg:stileopt} shows the complete optimization process. It traverses all the \stile{}s in the tile database to compute their cost on the given dynamically sparse operator and picks the best. Specifically, \texttt{CoverAlgo} (\autoref{line:coveralgo}) outputs the number of \stile{}s needed to cover all the non-zero values of a given sparsity sample. The cost is the sum of the $n$ sparsity samples.

\subsection{Online Sparsity Detection}\label{sec:fast_index}
With the PIT transformation, \sysname{} can handle different sparse patterns by generating the corresponding index for\sload{} and \swrite{} based on the input. Constructing sparse indexes on the fly is quite challenging. As shown in \autoref{fig:convert_computation}, the conversion overhead of cuSparse can be much higher than the computation time, especially when the sparsity is high. %\MLX{[challenge: cusparse sparse index construction is slow]}

We first propose an efficient representation for dynamic sparsity annotation. Our sparse representation comprises two parts: sparsity granularity and a binary sparsity attribute matrix. This representation can be annotated to any axis or combination of axes in a tensor. Each value in the sparse attribute matrix corresponds to a data block of the same size as the annotated sparsity granularity. Notably, multiple sparsity granularities can be used in the same dynamic sparse representation, such as when specifying sparsity for sentences of different lengths in the same batch. Assuming the input tensor has shape $[B, M, H]$, where $B$ is the batch size, M is the length of the longest sentence in the batch, and H is the hidden dimension size, we can annotate an array of length $B$ on the first dimension: [$(S_{dim1}, \ldots , S_{dimN})$], where $S_{dimN}$) represents the length of the Nth sentence. This sparse representation is flexible enough to efficiently represent dynamic sparsity while using less memory%. and naturally fits the property of \property{} that rearrange data along an axis.

To improve the efficiency of online sparse detection, we propose an effective mechanism for constructing sparse indexes online. 
PIT transformation allows \sysname{} to perform the computation when an axis is permutated or unordered(\S\ref{sec:pit_policy}).
With \property{}, \sysname{} no longer requires the sparse indices to be sorted along a certain axis. 
This greatly reduces the constraints on building sparse indices, allowing us to construct them with minimal synchronization overhead.
\sysname{} constructs sparse indexes at the granularity of Micro-tiles in an unordered manner. After tiling, each thread block only traverses the corresponding region of the input tensor and checks for the Micro-tiles with non-zero values. Each thread block uses "atomicadd" to determine where to write the index of its Micro-tile. However, the scheduling order of thread blocks is unpredictable, resulting in unordered global micro-tile indices.
Therefore, \sysname{} can achieve efficient tiling and extremely low synchronization overhead using \property{}, \sload{}, and \swrite{}. Furthermore, \sysname{} only builds sparse indices online without copying data. At runtime, sparse kernels use \sload{} to read directly from the original tensor based on the constructed sparse index. This greatly reduces the memory access overhead introduced by data format conversion (from dense to BCSR) and achieves zero-copy data rearrangement.

==> permutation_policy.tex <==
\subsection{Transformation Policy} \label{sec:permutation}

\textit{Tensor Expression} (TE) is widely used to describe deep learning computation in existing deep learning compilers~\cite{tvm,zheng2020ansor}. It describes how each element in the output tensor is computed from the corresponding elements of input tensors. Tensor expression can cover most operators for deep learning models. \autoref{tab:expression} lists some commonly used TEs for deep learning computation. Next, we elaborate permutation invariant and the deduced concept \property{} based on tensor expressions.

\begin{table}[h]
    {\centering
    \footnotesize{
    \begin{tabular}{l|c}
    \Xhline{2\arrayrulewidth}
    \textbf{Operator} & \textbf{Tensor Expression} \\ \hline
    ReduceSum & $C[p]$ += $A[p, l]$ \\
    Addition & $C[p]$ = $A[p]$ + $B[p]$ \\
    MatMul & $C[m,n]$ += $A[m,k]$ * $B[k,n]$ \\
    BatchMatmul & $C[b,m,n]$ += $A[b,m,k]$ * $B[b,k,n]$ \\
    Convolution & $C[n,f,x,y]$ += $A[n,m,x+i,y+j]$ * $B[f,m,i,j]$ \\ \hline
    \end{tabular}}
    \par}
    \caption{Example tensor expressions.\label{tab:expression}}
     %\vspace{-0.5cm}
\end{table}
\para{Permutation invariant.}
Dimension (\eg $m,n,k$ of MatMul) is one of the key concepts in tensor expression. It implies the way how data is accessed, which is often assumed to be consecutively iterated. However, we argue that in many cases, the order of data access along a dimension does not affect computation correctness. This type of dimension is called \adjp{} dimension. 
We formally define \adjp{} as follows.
%by the operation of permutation (data shuffle) along a dimension. 
% A definition can be formulated by the operation of permutation (data shuffle) along a dimension. 
\begin{definition}
\label{defn:adjp}
In a tensor expression $Y \leftarrow f(X_1,\ldots,X_n)$, where $f$ is an operator, $X_i$ and $Y$ are its input and output tensors respectively. A dimension $k$ in the operator is \adjp{} if it satisfies:
\begin{equation}
\label{eq:PI}
\begin{aligned}
    &\forall~\mathcal{P}\in \Phi_{k}, ~\exists~\mathcal{P^\prime} \in \Phi_{k}\\
    s.t.~~&\mathcal{P^\prime}(f(\mathcal{P}(X_1),\ldots,\mathcal{P}(X_n)) = Y,
\end{aligned}
\end{equation}
where $\Phi_{k}$ is the set of all permutation functions on $k$ dimension. $\mathcal{P}(X)$ means a permutation function $\mathcal{P}$ is applied on the $k$ dimension of the tensor $X$, to shuffle the elements on $k$ dimension to a new order. If $k$ dimension does not exist in $X$, $\mathcal{P}(X)=X$.
\end{definition}

An intuitive explanation of this definition is that, for a permutation invariant dimension (\eg $m$ in Matmul), when permutation is applied on this dimension of the input tensors (\eg $A$ in Matmul), there exists a reverse permutation on the output tensor (\eg $C$ in Matmul) to make the result the same as the original computation.
% \begin{definition}
% \label{defn:adjp}
% In a tensor expression $Y \leftarrow f(X_1,\ldots,X_n)$, a dimension $k$ is \adjp{} if it satisfies:
% \begin{equation}
% \label{eq:PI}
% \begin{aligned}
%     &\forall~\alpha\in \mathcal{P}(d_k), ~\exists~\beta \in \mathcal{P}(d_k)\\
%     s.t.~~&\mathcal{S}_{k,\beta}(f(\mathcal{S}_{k,\alpha}(X_1),\ldots,\mathcal{S}_{k,\alpha}(X_n)) = Y,
% \end{aligned}
% \end{equation} where $d_k$ is the length of the dimension $k$, $\mathcal{P}(x)$ is the set of all permutations of the sequence $[0,\ldots,x-1]$, and $\alpha, \beta$ are two sampled sequence of $\mathcal{P}(d_k)$. $\mathcal{S}_{k,\alpha}(X)$ denotes the data shuffle of tensor $X$ along dimension $k$ with the sequence $\alpha$. If $k$ is not $X$'s dimension, $\mathcal{S}_{k,\alpha}(X)=X$. %Without loss of generality, if $k$ is not $X$'s dimension (\eg $m$ is not $B$'s dimension in MatMul), $P_{k,\alpha}(X)=X$.
% \end{definition}
% Let $k$ be a dimension of length $d_k$ in a given tensor expression $Y \leftarrow f(X_1,\ldots,X_n)$ and satisfy 

% then dimension $k$ is \adjp{}.

%Here $\mathcal{P}(x)$ denotes all the possible permutation of sequence $[0,\ldots,x-1]$ and $\alpha, \beta$ are two sampled sequence of $\mathcal{P}(d_k)$. The operation $\mathcal{S}_{k,\alpha}(X)$ denote the data shuffle of tensor $X$ along dimension $k$ with the sequence $\alpha$. Without loss of generality, if $k$ is not $X$'s dimension (\eg $m$ is not $B$'s dimension in MatMul), $P_{k,\alpha}(X)=X$.
% \begin{table}[t]
%     {\centering
%     \footnotesize{
%     \begin{tabular}{l|c|c}
%     \Xhline{2\arrayrulewidth}
%     \textbf{Dimension Type} & \textbf{Description} & \textbf{Exp.} \\ \hline
%     Solo reduction $R_s$ & \makecell[l]{The reduction dimension that exists in \\ only one tensor} & $l$ \\
%     Cross reduction $R_c$ & \makecell[l]{The reduction dimension that spans in \\ multiple tensors} & $k$ \\
%     Prevalent spatial $S_p$ & \makecell[l]{The dimension that exists in all the \\ tensors} & $b$,$p$ \\
%     Sporadic spatial $S_s$ & \makecell[l]{The spatial dimension that co-exists \\ with $R_c$ in the same tensor and is not $S_p$} & $m$,$n$,$f$ \\
%     Compound $C_p$ & \makecell[l]{The dimensions in a compound \\ dimension (\eg $x+i$, $y+j$)} & $x$,$y$,$i$,$j$ \\ \hline
%     \end{tabular}}
%     \par}
%     \caption{Five categories of dimensions in operator expressions. The ``Exp.'' column is the example dimensions from \autoref{tab:expression}. \label{tab:dimension}}
%      %\vspace{-0.5cm}
% \end{table}

Permutation invariant dimensions are ubiquitous in deep learning computations. 
We study permutation invariant of tensor dimensions by classifying the dimensions into three categories: sporadic dimension, prevalent dimension, and compound dimension. 1) Sporadic dimension is the dimension that exists in one or more tensors of a tensor expression, but does not span in all tensors. For example, $m$, $n$, $k$, $f$, $l$ of the tensor expressions in \autoref{tab:expression} are sporadic dimension. 2) Prevalent dimension is the dimension that exists in all the tensors (\ie input and output tensors) of a tensor expression. Examples of prevalent dimension are $p$ and $b$ in \autoref{tab:expression}. 3) Compound dimension is the dimension that is involved in an arithmetic expression. For example in \autoref{tab:expression}, $x$ and $i$ in Convolution are involved in the arithmetic expression $x+i$. Similarly, $y$ and $j$ are involved in $y+j$. Thus, $x$, $y$, $i$, and $j$ are compound dimension.

Permutation invariant has different application rules for different types of dimension. First, when permutation invariant is applied on only one dimension of a tensor expression, the dimension can be sporadic dimension or prevalent dimension, but not compound dimension. Because permuting a compound dimension violates its corresponding arithmetic expression. Second, when permutation invariant is applied on multiple dimensions of a tensor expression, there are two application rules: 1) When the permuted dimensions are all sporadic dimension, each dimension can only have a single permutation function. For example, a tensor $X[i,j]$ where $i$ and $j$ are sporadic dimension, the permutation function for each vector $X[i,:]$ (\ie on $j$ dimension) should be the same. 2) When the permuted dimensions include a prevalent dimension, the permutation function on each element of the prevalent dimension could be different. For example, a tensor $X[i,j]$ where $i$ is prevalent dimension, the permutation function for each vector $X[i,:]$ can be different. This is because the computation on each element of prevalent dimension has no data dependency.
% We classify tensor dimensions into five categories as shown in \autoref{tab:dimension}. 
% Except the compound dimensions $C_p$, it is easy to verify that the $R_s$, $R_c$, $S_p$, and $S_s$ dimensions are \adjp{}. Two characteristics guarantee this permutation invariant:  (1) the computation of reduction (\eg the $k$ dimension in Matmul) is commutative, and (2) the computations of the values in an output tensor (\eg $C$ in Matmul) are spatially commutative (\eg along $m$ or $n$ dimension).

% The first one is that the reduction operation involved is order-independent accumulation. And the other is that the loop body only depends on its current iteration value and is irrelevant to other values.


% Whether a dimension is permutation invariant is firstly determined by the compute represented in the loop bodies inside it. The compute containing order-dependent operations, \eg Expotional Moving Averaging (EMA), is not permutation invariant. 

% The permutation invariance is also affected by the operation of data reusing. For example, the compound dimensions $C_p$ in \autoref{tab:dimension} depends on the continuity between current value and previously iterated values to save the cost of data loading. Random permutation breaks such continuity and make the computation generates unexpected results. Thus compound dimensions $C_p$ are classified as permutation variant accordingly.

\para{\property{}.} The permutation invariant offers extra opportunities to efficiently handle sparsity. Given a dimension $k$ of a tensor expression, if some of its elements are dropped (masked), this dimension is defined as a sparse dimension and the dropped elements are called redundant elements. With permutation invariant, we can construct a permutation function $\mathcal{P}$ to move all the redundant elements to the end while all the non-redundant elements to the front. The redundant elements can be safely removed to build a shorter $k$ dimension.
Such transformation is denoted as \property{}, it builds a connection between sparse and dense computation, brings the opportunity of leveraging dense computation kernels for sparse computation.

% \para{\property{}.} The permutation invariance offers extra opportunities to efficiently handle sparsity. Given a dimension $k$ of the above tensor expression, if some of its values can be dropped (skipped) without loss of correctness, then this dimension $k$ is defined as a sparse dimension and the dropable values are called redundant values. 
% % The number of redundant values is denoted as $r_k$.
% If a sparse dimension $k$ is \adjp{}, we can construct a permutation $\alpha\in\mathcal{P}(d_k)$ which moves all the redundant values to the end while all the non-redundant values to the front. By applying the operation $\mathcal{S}_{k,\alpha}(\cdot)$ then removing the redundant values of $k$ (from the end), dimension $k$ can be safely replaced by a new dimension $k_{nr}$ of only non-redundant values.
% % length $d_k-d_r$.
% Such transform is denoted as \property{} (\shortp{}), because the new dimension $k_{nr}$ behaves similarly to a dense dimension and is compatible with the optimizations applicable for dense compute.
% % For simplicity, the transform $P_{k,\alpha[:d_k-r_k]}(\cdot)$, which converts the sparse axis $k$ to new axis $k_{nr}$, is called Sparse-Dense Transform (\shortp{}) and its reverse transform is called Inverse \shortp{} (I\shortp{}).
% \property{} brings the opportunities of leveraging dense computing kernels to do sparse computation. For example, by applying the transform to a sparse dimension $m$ of MatMul, existing dense kernels can be directly reused. 


% % In the absence of data dependence, a dimension's \property{} can be independently made for every different value of other dimensions.
% \YQ{Not clear}
% In addition to standard transform, there is an extended transform type called \textit{conditional transform}, which allows applying a separate transform to a dimension given every element of other dimension(s). 
% For example, the dimension $l$ of ReduceSum in \autoref{tab:expression} can have different transforms given different element on dimension $p$.
% Conditional transform can fully utilize the fine-grained sparsity, but it needs to be aware of the data dependency. 
% % ???Safe transforms guaranteeing correctness need to be aware of the data dependency. 
% \autoref{tab:dimension} summarizes two scenarios to safely take advantage of conditional transform, they are (a) $S_p$ dimensions allowing other dimensions to be independently transformed for every element on $S_p$, and (b) transformation on $R_s$ dimensions that is  independently every element of other dimensions. 
% % For example, the dimension $l$ of ReduceSum in \autoref{tab:expression} belongs to solo reduction and thus can be safely applied with arbitrary transforms. 
% % Independent transform offers much more flexibility to handle sparsity. 
% % However, data dependency will make the independent transform unsafe. For dimensions summarized in 

% \para{\property{} for Tiles.} Directly applying \property{} on a dimension of an operator can naturally support sparsity at the granularity of a dimension, which is not efficient enough for commodity accelerators optimized for tile-level computation.  % Supporting the dimension level sparsity is not enough. 
% \property{} is powerful that can be applied at different computing granularities, including both dimensions and computing tiles.
% The tiling technique splits an operator's computation into many small pieces. The transform can be applied to each small piece independently.
% By applying the transform to a sparse data tile, we can obtain an equivalent dense computation at the tile level. 

% Conversely, the transform enables to cover more data with fixed-size compute. %process the sparsity inside the tile, and make the compute more compact. Conversely, the transform enables to cover more data with fixed-size compute. 
%By applying the transform to a data tile, we can process the sparsity inside the tile, and make the compute more compact. Conversely, the transform enables to cover more data with fixed-size compute. 
% The compute in Definition~\ref{def:sdt} is not limited to the original operators. In the computing tiles level, sparse-dense transformation can be applied to each tile independently. 
% This property largely enables the ability of \property{}, because the probability of an axis to be sparse increases when it comes to a finer granularity. 



% Take the MatMul $C=A*B$ (\autoref{tab:expression}) as instance, where $A$ is sparse with $\mathbf{a_{1,2}} \in \mathcal{R}^{1\times d_k}$. By identifying $m$ to be \adjp{}, it's possible to condense $A$ to $A^{(nz)}$ and leverage existing dense kernels directly.

% \begin{equation}
% \label{eq:simple-example}
%     \begin{aligned}
%     &\underbrace{\left[\begin{array}{c}
%          \mathbf{a_1}\\
%          \mathbf{0}  \\
%          \mathbf{a_2} \\
%          \mathbf{0} 
%     \end{array}\right]}_{A_{4\times d_k}}
%     \xrightarrow[]{\shortp{}}
%     &\underbrace{\left[\begin{array}{c}
%          \mathbf{a_1} \\
%          \mathbf{a_2} \\
%     \end{array}\right]}_{A^{(nz)}}
%     \times B_{d_k\times d_n}
%     \xrightarrow[]{I\shortp{}}
%     \underbrace{\left[\begin{array}{cc}
%          \mathbf{a_1 B} \\
%          \mathbf{0}  \\
%          \mathbf{a_2 B} \\
%          \mathbf{0} \\
%     \end{array}\right]}_{C_{4\times d_n}}    
% \end{aligned}
% \end{equation}


% \comments{yuqing}{previous \textit{compute invariance} part in 3.2}



% from the perspective of loop optimization. In these dimensions, each loop iteration only use one index of each dimension, and there are no dependencies between iterations except for the index-irrelevant reduction operation (if exists). \comments{yuqing}{do we need to give more proof?}

% \begin{claim}
% \label{claim:unique}
%     % For dimensions corresponding to the outer loops, if there is no dependencies (data reuse) between iterations, the \shortp{} dimensions corresponding to the inner loops can have different transformation for each iteration. 
%     % Different type of dimensions has different degree of freedom to have independent sparse-dense transform.
    
% \end{claim}



% Different type of dimension has different constraints on applying the mapping functions.
% According to the compute and data reusing types, different type of dimensions has different behaves when do the transform.
% Such extra degree of freedom offers more opportunities to make the computing more efficient.
% We summarize the below rules to describe such extra freedom.

% \begin{itemize}[leftmargin=*]
%   \setlength\itemsep{-0.4em}
%   \item For a multi-dimension tensor $T$ which has an $S_p$ dimension, the mapping function $f$ of the sparse matrix (or vector) $T[:,x,:]$ can be different for different $x$ values, where $x$ is on $S_p$ dimension.
%   \item For a multi-dimension tensor $T$ which has a $R_s$ dimension, the mapping function $f$ of the sparse vector $T[x,y,:]$ can be different for different values of $x,y$, where ``:'' is the $R_s$ dimension.
%   \item For a multi-dimension tensor $T$ which has $R_c$ and $S_s$ dimensions, the mapping function $f$ of sparse vector $T[x,:]$ should be the same for different values of $x$, where $x$ is on $S_s$ dimension and ``:'' is $R_c$ dimension.
%   \item Mapping function $f$ cannot be applied on $C_p$ dimension.
% \end{itemize}



% Here is an example of $C=AB$ (\autoref{fig:stile}) where $m$ is no longer sparse in operator level ($\mathbf{a_{1,..,4}}\in \mathcal{R}^{1\times \frac{d_k}{2}}$ and $\mathbf{b_{1,2}}\in \mathcal{R}^{\frac{d_k}{2}\times d_n}$). 
% By applying \shortp{} in $m$ and split $k$, the compute can still be optimized by dense MatMul kernels. 
% \begin{equation}
%     \underbrace{\left[\begin{array}{c|c}
%          \mathbf{a_1} & \mathbf{0}\\
%          \mathbf{0} & \mathbf{a_3} \\
%          \mathbf{a_2} & \mathbf{0}\\
%          \mathbf{0} & \mathbf{a_4}
%     \end{array}\right]}_{A_{4\times d_k}}
%     \xrightarrow[]{\shortp{}}    &\underbrace{\left[\begin{array}{c|c}
%          \mathbf{a_1} & \mathbf{a_3} \\
%          \mathbf{a_2} & \mathbf{a_4} \\
%     \end{array}\right]}_{A^{(nz)}}
%     \underbrace{\left[\begin{array}{cc}
%          \mathbf{b_1}  \\
%          \hline
%          \mathbf{b_2} 
%     \end{array}\right]}_{B}
%     \xrightarrow[]{I\shortp{}}    \underbrace{\left[\begin{array}{cc}
%          \mathbf{a_1 b_1} & \mathbf{0} \\
%          \mathbf{0} & \mathbf{a_3 b_2} \\
%          \mathbf{a_2 b_1} & \mathbf{0} \\
%          \mathbf{0} & \mathbf{a_4 b_2} \\
%     \end{array}\right] }_{C_{4\times d_n}}
% \end{equation}


==> property_loop.tex <==
\subsection{PIT Transformation Policy} \label{sec:permutation}

%Tensor Expression (TE) is a common method for describing deep learning computations in existing deep learning compilers, as demonstrated in works such as TVM~\cite{tvm} and Ansor~\cite{zheng2020ansor}. It provides a concise description of how each element in the output tensor is computed from corresponding elements of input tensors, and can cover most operators for deep learning models. \autoref{tab:expression} lists some commonly used TE examples for deep learning computations. We introduce the concept of permutation invariance in tensor expressions and its derived property, denoted as \property{}.

In this chapter, we first introduce a mathematical property called \adjp{}~\cite{balan2022permutation}, and use it to derive a related property called \property{} in Tensor Expressions (abbreviated as TE). \autoref{tab:expression} lists some common operators in deep learning and their corresponding TE. Different axes in TE (such as m, n, k in matrix multiplication) describe how to access the data in the input and output, and are typically assumed to be iterated continuously. However, we observe that shuffling the indices along certain axes does not affect the correctness of the program. For example, in Vector Addition, we can permute the p-axis arbitrarily and still obtain the same result. We refer to such axes as having the \adjp{} property. We introduce \adjp{} into TE and formally define it as follows:
\begin{table}[h]
    {\centering
    \footnotesize{
    \begin{tabular}{l|c}
    \Xhline{2\arrayrulewidth}
    \textbf{Operator} & \textbf{Tensor Expression} \\ \hline
    ReduceSum & $C[p]$ += $A[p, l]$ \\
    Vector Addition & $C[p]$ = $A[p]$ + $B[p]$ \\
    MatMul & $C[m,n]$ += $A[m,k]$ * $B[k,n]$ \\
    BatchMatmul & $C[b,m,n]$ += $A[b,m,k]$ * $B[b,k,n]$ \\
    Convolution & $C[n,f,x,y]$ += $A[n,m,x+i,y+j]$ * $B[f,m,i,j]$ \\ \hline
    \end{tabular}}
    \par}
    \caption{Example tensor expressions.\label{tab:expression}}
     %\vspace{-0.5cm}
\end{table}
% \para{Permutation invariant.}
%Dimension (\eg $m,n,k$ of MatMul) is one of the key concepts in tensor expression. It implies the way how data is accessed, which is often assumed to be consecutively iterated. However, we argue that in many cases, the order of data access along a dimension does not affect computation correctness. This type of dimension is called \adjp{} dimension. 
% We formally define \adjp{} as follows.
%by the operation of permutation (data shuffle) along a dimension. 
% A definition can be formulated by the operation of permutation (data shuffle) along a dimension. 
\begin{definition}
\label{defn:adjp}
In a tensor expression $Y \leftarrow f(X_1,\ldots,X_n)$, where $f$ is an operator, $X_i$ and $Y$ are its input and output tensors respectively. A axis $k$ in the operator is \adjp{} if it satisfies:
\begin{equation}
\label{eq:PI}
\begin{aligned}
    &\forall~\mathcal{P}\in \Phi_{k}, ~\exists~\mathcal{P^\prime} \in \Phi_{k}\\
    s.t.~~&\mathcal{P^\prime}(f(\mathcal{P}(X_1),\ldots,\mathcal{P}(X_n)) = Y,
\end{aligned}
\end{equation}
where $\Phi_{k}$ is the set of all permutation functions on $k$ axis. $\mathcal{P}(X)$ means a permutation function $\mathcal{P}$ is applied on the $k$ axis of the tensor $X$, to shuffle the elements on $k$ axis to a new order. If $k$ axis does not exist in $X$, $\mathcal{P}(X)=X$.
\end{definition}

%An intuitive explanation of this definition is that, for a permutation invariant dimension (\eg $m$ in Matmul), when permutation is applied on this dimension of the input tensors (\eg $A$ in Matmul), there exists a reverse permutation on the output tensor (\eg $C$ in Matmul) to make the result the same as the original computation.
% \begin{definition}
% \label{defn:adjp}
% In a tensor expression $Y \leftarrow f(X_1,\ldots,X_n)$, a dimension $k$ is \adjp{} if it satisfies:
% \begin{equation}
% \label{eq:PI}
% \begin{aligned}
%     &\forall~\alpha\in \mathcal{P}(d_k), ~\exists~\beta \in \mathcal{P}(d_k)\\
%     s.t.~~&\mathcal{S}_{k,\beta}(f(\mathcal{S}_{k,\alpha}(X_1),\ldots,\mathcal{S}_{k,\alpha}(X_n)) = Y,
% \end{aligned}
% \end{equation} where $d_k$ is the length of the dimension $k$, $\mathcal{P}(x)$ is the set of all permutations of the sequence $[0,\ldots,x-1]$, and $\alpha, \beta$ are two sampled sequence of $\mathcal{P}(d_k)$. $\mathcal{S}_{k,\alpha}(X)$ denotes the data shuffle of tensor $X$ along dimension $k$ with the sequence $\alpha$. If $k$ is not $X$'s dimension, $\mathcal{S}_{k,\alpha}(X)=X$. %Without loss of generality, if $k$ is not $X$'s dimension (\eg $m$ is not $B$'s dimension in MatMul), $P_{k,\alpha}(X)=X$.
% \end{definition}
% Let $k$ be a dimension of length $d_k$ in a given tensor expression $Y \leftarrow f(X_1,\ldots,X_n)$ and satisfy 

% then dimension $k$ is \adjp{}.

%Here $\mathcal{P}(x)$ denotes all the possible permutation of sequence $[0,\ldots,x-1]$ and $\alpha, \beta$ are two sampled sequence of $\mathcal{P}(d_k)$. The operation $\mathcal{S}_{k,\alpha}(X)$ denote the data shuffle of tensor $X$ along dimension $k$ with the sequence $\alpha$. Without loss of generality, if $k$ is not $X$'s dimension (\eg $m$ is not $B$'s dimension in MatMul), $P_{k,\alpha}(X)=X$.
% \begin{table}[t]
%     {\centering
%     \footnotesize{
%     \begin{tabular}{l|c|c}
%     \Xhline{2\arrayrulewidth}
%     \textbf{Dimension Type} & \textbf{Description} & \textbf{Exp.} \\ \hline
%     Solo reduction $R_s$ & \makecell[l]{The reduction dimension that exists in \\ only one tensor} & $l$ \\
%     Cross reduction $R_c$ & \makecell[l]{The reduction dimension that spans in \\ multiple tensors} & $k$ \\
%     Prevalent spatial $S_p$ & \makecell[l]{The dimension that exists in all the \\ tensors} & $b$,$p$ \\
%     Sporadic spatial $S_s$ & \makecell[l]{The spatial dimension that co-exists \\ with $R_c$ in the same tensor and is not $S_p$} & $m$,$n$,$f$ \\
%     Compound $C_p$ & \makecell[l]{The dimensions in a compound \\ dimension (\eg $x+i$, $y+j$)} & $x$,$y$,$i$,$j$ \\ \hline
%     \end{tabular}}
%     \par}
%     \caption{Five categories of dimensions in operator expressions. The ``Exp.'' column is the example dimensions from \autoref{tab:expression}. \label{tab:dimension}}
%      %\vspace{-0.5cm}
% \end{table}

The intuitive explanation of this definition is that for an axis X that is \adjp{}, if we permute the X-axis of the input tensor, there must exist a corresponding inverse permutation on the X-axis of the output tensor to ensure that the input-output results remain consistent before and after the permutation. Permutation-invariant axes are widely present in deep learning computations.

%Permutation invariant dimensions are ubiquitous in deep learning computations. 
We study the permutation invariant of tensor dimensions by classifying the dimensions into three categories: sporadic dimension, prevalent dimension, and compound dimension. 1) Sporadic dimension is the dimension that exists in one or more tensors of a tensor expression, but does not span in all tensors. For example, $m$, $n$, $k$, $f$, $l$ of the tensor expressions in \autoref{tab:expression} are sporadic dimension. 2) Prevalent dimension is the dimension that exists in all the tensors (\ie input and output tensors) of a tensor expression. Examples of prevalent dimension are $p$ and $b$ in \autoref{tab:expression}. 3) Compound dimension is the dimension that is involved in an arithmetic expression. For example in \autoref{tab:expression}, $x$ and $i$ in Convolution are involved in the arithmetic expression $x+i$. Similarly, $y$ and $j$ are involved in $y+j$. Thus, $x$, $y$, $i$, and $j$ are compound dimension.

Permutation invariant has different application rules for different types of dimension. First, when permutation invariant is applied on only one dimension of a tensor expression, the dimension can be sporadic dimension or prevalent dimension, but not compound dimension. Because permuting a compound dimension violates its corresponding arithmetic expression. Second, when permutation invariant is applied on multiple dimensions of a tensor expression, there are two application rules: 1) When the permuted dimensions are all sporadic dimension, each dimension can only have a single permutation function. For example, a tensor $X[i,j]$ where $i$ and $j$ are sporadic dimension, the permutation function for each vector $X[i,:]$ (\ie on $j$ dimension) should be the same. 2) When the permuted dimensions include a prevalent dimension, the permutation function on each element of the prevalent dimension could be different. For example, a tensor $X[i,j]$ where $i$ is prevalent dimension, the permutation function for each vector $X[i,:]$ can be different. This is because the computation on each element of prevalent dimension has no data dependency.
% We classify tensor dimensions into five categories as shown in \autoref{tab:dimension}. 
% Except the compound dimensions $C_p$, it is easy to verify that the $R_s$, $R_c$, $S_p$, and $S_s$ dimensions are \adjp{}. Two characteristics guarantee this permutation invariant:  (1) the computation of reduction (\eg the $k$ dimension in Matmul) is commutative, and (2) the computations of the values in an output tensor (\eg $C$ in Matmul) are spatially commutative (\eg along $m$ or $n$ dimension).

% The first one is that the reduction operation involved is order-independent accumulation. And the other is that the loop body only depends on its current iteration value and is irrelevant to other values.


% Whether a dimension is permutation invariant is firstly determined by the compute represented in the loop bodies inside it. The compute containing order-dependent operations, \eg Expotional Moving Averaging (EMA), is not permutation invariant. 

% The permutation invariance is also affected by the operation of data reusing. For example, the compound dimensions $C_p$ in \autoref{tab:dimension} depends on the continuity between current value and previously iterated values to save the cost of data loading. Random permutation breaks such continuity and make the computation generates unexpected results. Thus compound dimensions $C_p$ are classified as permutation variant accordingly.

\para{\property{}.} The permutation invariant offers extra opportunities to efficiently handle sparsity. Given a dimension $k$ of a tensor expression, if some of its elements are dropped (masked), this dimension is defined as a sparse dimension and the dropped elements are called redundant elements. With permutation invariant, we can construct a permutation function $\mathcal{P}$ to move all the redundant elements to the end while all the non-redundant elements to the front. The redundant elements can be safely removed to build a shorter $k$ dimension.
Such transformation is denoted as \property{}, it builds a connection between sparse and dense computation, brings the opportunity of leveraging dense computation kernels for sparse computation.

% \para{\property{}.} The permutation invariance offers extra opportunities to efficiently handle sparsity. Given a dimension $k$ of the above tensor expression, if some of its values can be dropped (skipped) without loss of correctness, then this dimension $k$ is defined as a sparse dimension and the dropable values are called redundant values. 
% % The number of redundant values is denoted as $r_k$.
% If a sparse dimension $k$ is \adjp{}, we can construct a permutation $\alpha\in\mathcal{P}(d_k)$ which moves all the redundant values to the end while all the non-redundant values to the front. By applying the operation $\mathcal{S}_{k,\alpha}(\cdot)$ then removing the redundant values of $k$ (from the end), dimension $k$ can be safely replaced by a new dimension $k_{nr}$ of only non-redundant values.
% % length $d_k-d_r$.
% Such transform is denoted as \property{} (\shortp{}), because the new dimension $k_{nr}$ behaves similarly to a dense dimension and is compatible with the optimizations applicable for dense compute.
% % For simplicity, the transform $P_{k,\alpha[:d_k-r_k]}(\cdot)$, which converts the sparse axis $k$ to new axis $k_{nr}$, is called Sparse-Dense Transform (\shortp{}) and its reverse transform is called Inverse \shortp{} (I\shortp{}).
% \property{} brings the opportunities of leveraging dense computing kernels to do sparse computation. For example, by applying the transform to a sparse dimension $m$ of MatMul, existing dense kernels can be directly reused. 


% % In the absence of data dependence, a dimension's \property{} can be independently made for every different value of other dimensions.
% \YQ{Not clear}
% In addition to standard transform, there is an extended transform type called \textit{conditional transform}, which allows applying a separate transform to a dimension given every element of other dimension(s). 
% For example, the dimension $l$ of ReduceSum in \autoref{tab:expression} can have different transforms given different element on dimension $p$.
% Conditional transform can fully utilize the fine-grained sparsity, but it needs to be aware of the data dependency. 
% % ???Safe transforms guaranteeing correctness need to be aware of the data dependency. 
% \autoref{tab:dimension} summarizes two scenarios to safely take advantage of conditional transform, they are (a) $S_p$ dimensions allowing other dimensions to be independently transformed for every element on $S_p$, and (b) transformation on $R_s$ dimensions that is  independently every element of other dimensions. 
% % For example, the dimension $l$ of ReduceSum in \autoref{tab:expression} belongs to solo reduction and thus can be safely applied with arbitrary transforms. 
% % Independent transform offers much more flexibility to handle sparsity. 
% % However, data dependency will make the independent transform unsafe. For dimensions summarized in 

% \para{\property{} for Tiles.} Directly applying \property{} on a dimension of an operator can naturally support sparsity at the granularity of a dimension, which is not efficient enough for commodity accelerators optimized for tile-level computation.  % Supporting the dimension level sparsity is not enough. 
% \property{} is powerful that can be applied at different computing granularities, including both dimensions and computing tiles.
% The tiling technique splits an operator's computation into many small pieces. The transform can be applied to each small piece independently.
% By applying the transform to a sparse data tile, we can obtain an equivalent dense computation at the tile level. 

% Conversely, the transform enables to cover more data with fixed-size compute. %process the sparsity inside the tile, and make the compute more compact. Conversely, the transform enables to cover more data with fixed-size compute. 
%By applying the transform to a data tile, we can process the sparsity inside the tile, and make the compute more compact. Conversely, the transform enables to cover more data with fixed-size compute. 
% The compute in Definition~\ref{def:sdt} is not limited to the original operators. In the computing tiles level, sparse-dense transformation can be applied to each tile independently. 
% This property largely enables the ability of \property{}, because the probability of an axis to be sparse increases when it comes to a finer granularity. 



% Take the MatMul $C=A*B$ (\autoref{tab:expression}) as instance, where $A$ is sparse with $\mathbf{a_{1,2}} \in \mathcal{R}^{1\times d_k}$. By identifying $m$ to be \adjp{}, it's possible to condense $A$ to $A^{(nz)}$ and leverage existing dense kernels directly.

% \begin{equation}
% \label{eq:simple-example}
%     \begin{aligned}
%     &\underbrace{\left[\begin{array}{c}
%          \mathbf{a_1}\\
%          \mathbf{0}  \\
%          \mathbf{a_2} \\
%          \mathbf{0} 
%     \end{array}\right]}_{A_{4\times d_k}}
%     \xrightarrow[]{\shortp{}}
%     &\underbrace{\left[\begin{array}{c}
%          \mathbf{a_1} \\
%          \mathbf{a_2} \\
%     \end{array}\right]}_{A^{(nz)}}
%     \times B_{d_k\times d_n}
%     \xrightarrow[]{I\shortp{}}
%     \underbrace{\left[\begin{array}{cc}
%          \mathbf{a_1 B} \\
%          \mathbf{0}  \\
%          \mathbf{a_2 B} \\
%          \mathbf{0} \\
%     \end{array}\right]}_{C_{4\times d_n}}    
% \end{aligned}
% \end{equation}


% \comments{yuqing}{previous \textit{compute invariance} part in 3.2}



% from the perspective of loop optimization. In these dimensions, each loop iteration only use one index of each dimension, and there are no dependencies between iterations except for the index-irrelevant reduction operation (if exists). \comments{yuqing}{do we need to give more proof?}

% \begin{claim}
% \label{claim:unique}
%     % For dimensions corresponding to the outer loops, if there is no dependencies (data reuse) between iterations, the \shortp{} dimensions corresponding to the inner loops can have different transformation for each iteration. 
%     % Different type of dimensions has different degree of freedom to have independent sparse-dense transform.
    
% \end{claim}



% Different type of dimension has different constraints on applying the mapping functions.
% According to the compute and data reusing types, different type of dimensions has different behaves when do the transform.
% Such extra degree of freedom offers more opportunities to make the computing more efficient.
% We summarize the below rules to describe such extra freedom.

% \begin{itemize}[leftmargin=*]
%   \setlength\itemsep{-0.4em}
%   \item For a multi-dimension tensor $T$ which has an $S_p$ dimension, the mapping function $f$ of the sparse matrix (or vector) $T[:,x,:]$ can be different for different $x$ values, where $x$ is on $S_p$ dimension.
%   \item For a multi-dimension tensor $T$ which has a $R_s$ dimension, the mapping function $f$ of the sparse vector $T[x,y,:]$ can be different for different values of $x,y$, where ``:'' is the $R_s$ dimension.
%   \item For a multi-dimension tensor $T$ which has $R_c$ and $S_s$ dimensions, the mapping function $f$ of sparse vector $T[x,:]$ should be the same for different values of $x$, where $x$ is on $S_s$ dimension and ``:'' is $R_c$ dimension.
%   \item Mapping function $f$ cannot be applied on $C_p$ dimension.
% \end{itemize}



% Here is an example of $C=AB$ (\autoref{fig:stile}) where $m$ is no longer sparse in operator level ($\mathbf{a_{1,..,4}}\in \mathcal{R}^{1\times \frac{d_k}{2}}$ and $\mathbf{b_{1,2}}\in \mathcal{R}^{\frac{d_k}{2}\times d_n}$). 
% By applying \shortp{} in $m$ and split $k$, the compute can still be optimized by dense MatMul kernels. 
% \begin{equation}
%     \underbrace{\left[\begin{array}{c|c}
%          \mathbf{a_1} & \mathbf{0}\\
%          \mathbf{0} & \mathbf{a_3} \\
%          \mathbf{a_2} & \mathbf{0}\\
%          \mathbf{0} & \mathbf{a_4}
%     \end{array}\right]}_{A_{4\times d_k}}
%     \xrightarrow[]{\shortp{}}    &\underbrace{\left[\begin{array}{c|c}
%          \mathbf{a_1} & \mathbf{a_3} \\
%          \mathbf{a_2} & \mathbf{a_4} \\
%     \end{array}\right]}_{A^{(nz)}}
%     \underbrace{\left[\begin{array}{cc}
%          \mathbf{b_1}  \\
%          \hline
%          \mathbf{b_2} 
%     \end{array}\right]}_{B}
%     \xrightarrow[]{I\shortp{}}    \underbrace{\left[\begin{array}{cc}
%          \mathbf{a_1 b_1} & \mathbf{0} \\
%          \mathbf{0} & \mathbf{a_3 b_2} \\
%          \mathbf{a_2 b_1} & \mathbf{0} \\
%          \mathbf{0} & \mathbf{a_4 b_2} \\
%     \end{array}\right] }_{C_{4\times d_n}}
% \end{equation}


==> property_perm.tex <==
\section{\property{}}

\begin{table}[t]
    {\centering
    \footnotesize{
    \begin{tabular}{l|c}
    \Xhline{2\arrayrulewidth}
    \textbf{Operator} & \textbf{Operator Expression} \\ \hline
    ReduceSum & $C[p]$ += $A[p, l]$ \\
    Addition & $C[p]$ = $A[p]$ + $B[p]$ \\
    MatMul & $C[m,n]$ += $A[m,k]$ * $B[k,n]$ \\
    BatchMatmul & $C[b,m,n]$ += $A[b,m,k]$ * $B[b,k,n]$ \\
    Convolution & $C[n,f,x,y]$ += $A[n,m,x+i,y+j]$ * $B[f,m,i,j]$ \\ \hline
    \end{tabular}}
    \par}
    \caption{Example operator expressions.\label{tab:expression}}
     %\vspace{-0.5cm}
\end{table}

\begin{table}[t]
    {\centering
    \footnotesize{
    \begin{tabular}{l|c|c}
    \Xhline{2\arrayrulewidth}
    \textbf{Dimension Type} & \textbf{Description} & \textbf{Exp.} \\ \hline
    Solo reduction $R_s$ & \makecell[l]{The reduction dimension that exists in \\ only one tensor} & $l$ \\
    Cross reduction $R_c$ & \makecell[l]{The reduction dimension that spans in \\ multiple tensors} & $k$ \\
    Prevalent spatial $S_p$ & \makecell[l]{The dimension that exists in all the \\ tensors} & $b$,$p$ \\
    Sporadic spatial $S_s$ & \makecell[l]{The spatial dimension that co-exists \\ with $R_c$ in the same tensor and is not $S_p$} & $m$,$n$,$f$ \\
    Compound $C_p$ & \makecell[l]{The dimensions in a compound \\ dimension (\eg $x+i$, $y+j$)} & $x$,$y$,$i$,$j$ \\ \hline
    \end{tabular}}
    \par}
    \caption{Five categories of dimensions in operator expressions. The ``Exp.'' column is the example dimensions from \autoref{tab:expression}. \label{tab:dimension}}
     %\vspace{-0.5cm}
\end{table}

As shown in \autoref{tab:expression}, the compute in DNN models are commonly defined by \textit{Tensor Expression} (TE, \aka Operation Expression, \eg einsum[]) with dimensions (\eg $m,n,k$ of MatMul).
In the existing common practices, such dimensions are defined as consecutive axis and the subsequent optimizations (schedules) are based on this assumption. Thus this optimization framework can't be compatible with the sparsity cases.
% , they have to create special techniques (\eg SparseTIR ??) to handle sparsity.

We propose a powerful property called \property{}, which can naturally leverage the existing dense optimization skills to optimize sparse compute. 

\subsection{Definition}
Let $k$ be a dimension of length $d_k$ and $X$ be a multiple-dimension tensor with dimension $k$. The permutation along $k$ given that $\alpha$ is a permutation of sequence $(0,\ldots,d_k-1)$ is defined as below
\begin{equation}
    P_{k,\alpha}(X) = X[..,\alpha,..] 
    \quad \forall~\alpha \in Perm(k)
\end{equation}
here $Perm(k)$ is the set of all the possible permutations of sequence $(0,\ldots,d_k-1)$.
% \footnote{$Perm(k) = \{s:s=\text{numpy.random.permutation}(d_k)\}$}. 
Without loss of generality, if $k$ is not $X$'s dimension (\eg $m$ is not $B$'s dimension in MatMul), $P_{k,\alpha}(X)=X$.

\begin{definition}%[\textbf{\property{}}]
\label{def:sdt}
    Let $k$ be a dimension in a given tensor expression $Y \leftarrow f(X_1,\ldots,X_n)$ and satisfy 
    \begin{equation}
    \label{eq:PI}
    \begin{aligned}
        &\forall~\alpha\in Perm(k) ~ \exists~\beta \in Perm(k)\\
        &s.t.\\
        &P_{k,\beta}(f(P_{k,\alpha}(X_1),\ldots,P_{k,\alpha}(X_n)) \equiv Y
    \end{aligned}
    \end{equation}
    , then dimension $k$ is \adjp{}.
    % and $\beta$ is the reverse \shortp{} permutation of $\alpha$.
\end{definition}
\textbf{Explanation}. For a sparse dimension $k$ in an expression, there are some redundant indexes that can be dropped without affecting the correctness of the compute. 
Let $r_k$ be the number of redundant indexes and $\alpha\in Perm(k)$ be a permutation which moves all the redundant indexes to the end while all the non-redundant indexes to the front. 
If $k$ satisfies \shortp{} condition,
% (let $\beta$ be the reverse \shortp{} permutation of $\alpha$), 
according to the permutation invariant property in \autoref{eq:PI} and the fact that the last $r_k$ indexes of $\alpha$ is redundant, dimension $k$ can be safely replaced by a new dimension $k_{nr}$ by only keeping the first $d_k-r_k$ indexes of $\alpha$.
For simplicity, the transform $P_{k,\alpha[:d_k-r_k]}(\cdot)$, which converts the sparse axis $k$ to new axis $k_{nr}$, is called Sparse-Dense Transform (\shortp{}) and its reverse transform is called Inverse \shortp{} (I\shortp{}).
% denoted as $\Gamma_k(\cdot)$ while the reverse operation $P_{k,\beta}(\cdot)$ is denoted as $\Gamma_k^{-1}(\cdot)$.

Take the MatMul $C=A*B$ (\autoref{tab:expression}) as instance, where $A$ is sparse with $\mathbf{a_{1,2}} \in \mathcal{R}^{1\times d_k}$. By identifying $m$ to be \adjp{}, it's possible to condense $A$ to $A^{(nz)}$ and leverage existing dense kernels directly.

\begin{equation}
\label{eq:simple-example}
    \begin{aligned}
    &\underbrace{\left[\begin{array}{c}
         \mathbf{a_1}\\
         \mathbf{0}  \\
         \mathbf{a_2} \\
         \mathbf{0} 
    \end{array}\right]}_{A_{4\times d_k}}
    \xrightarrow[]{\shortp{}}
    &\underbrace{\left[\begin{array}{c}
         \mathbf{a_1} \\
         \mathbf{a_2} \\
    \end{array}\right]}_{A^{(nz)}}
    \times B_{d_k\times d_n}
    \xrightarrow[]{I\shortp{}}
    \underbrace{\left[\begin{array}{cc}
         \mathbf{a_1 B} \\
         \mathbf{0}  \\
         \mathbf{a_2 B} \\
         \mathbf{0} \\
    \end{array}\right]}_{C_{4\times d_n}}    
\end{aligned}
\end{equation}

\subsection{Properties}
\comments{yuqing}{previous \textit{compute invariance} part in 3.2}

\begin{claim}
    Sparse-dense transformable dimensions are ubiquitous in deep learning computations. 
\end{claim}

We classify tensor dimensions into five categories as shown in \autoref{tab:dimension}. It's easy to verify that the $R_s$, $R_c$, $S_p$, and $S_s$ dimensions are \adjp{} from the perspective of loop optimization. In these dimensions, each loop iteration only use one index of each dimension, and there are no dependencies between iterations except for the index-irrelevant reduction operation (if exists). \comments{yuqing}{do we need to give more proof?}

\begin{claim}
\label{claim:unique}
    % For dimensions corresponding to the outer loops, if there is no dependencies (data reuse) between iterations, the \shortp{} dimensions corresponding to the inner loops can have different transformation for each iteration. 
    Different type of dimensions has different degree of freedom to have independent sparse-dense transform.
\end{claim}

% Different type of dimension has different constraints on applying the mapping functions.
According to the compute and data reusing types, different type of dimensions has different behaves when do the transform. For example, the dimension $l$ of ReduceSum in \autoref{tab:expression} can apply different transform for every different value of dimension $p$. Such extra degree of freedom offers more opportunities to make the computing more efficient.
We summarize the below rules to describe such extra freedom.

\begin{itemize}[leftmargin=*]
  \setlength\itemsep{-0.4em}
  \item For a multi-dimension tensor $T$ which has an $S_p$ dimension, the mapping function $f$ of the sparse matrix (or vector) $T[:,x,:]$ can be different for different $x$ values, where $x$ is on $S_p$ dimension.
  \item For a multi-dimension tensor $T$ which has a $R_s$ dimension, the mapping function $f$ of the sparse vector $T[x,y,:]$ can be different for different values of $x,y$, where ``:'' is the $R_s$ dimension.
  \item For a multi-dimension tensor $T$ which has $R_c$ and $S_s$ dimensions, the mapping function $f$ of sparse vector $T[x,:]$ should be the same for different values of $x$, where $x$ is on $S_s$ dimension and ``:'' is $R_c$ dimension.
  \item Mapping function $f$ cannot be applied on $C_p$ dimension.
\end{itemize}

\begin{claim}
    \property{} can be applied to multiple computing granularities, including both the operators and the different hierarchies of computing tiles.
\end{claim}
The compute in Definition~\ref{def:sdt} is not limited to the original operators. In the computing tiles level, sparse-dense transformation can be applied to each tile independently. 

This property largely enables the ability of \property{}, because the probability of an axis to be sparse increases when it comes to a finer granularity. 

Here is an example of $C=AB$ (\autoref{fig:stile}) where $m$ is no longer sparse in operator level ($\mathbf{a_{1,..,4}}\in \mathcal{R}^{1\times \frac{d_k}{2}}$ and $\mathbf{b_{1,2}}\in \mathcal{R}^{\frac{d_k}{2}\times d_n}$). 
By applying \shortp{} in $m$ and split $k$, the compute can still be optimized by dense MatMul kernels. 
\begin{equation}
    \underbrace{\left[\begin{array}{c|c}
         \mathbf{a_1} & \mathbf{0}\\
         \mathbf{0} & \mathbf{a_3} \\
         \mathbf{a_2} & \mathbf{0}\\
         \mathbf{0} & \mathbf{a_4}
    \end{array}\right]}_{A_{4\times d_k}}
    \xrightarrow[]{\shortp{}}    &\underbrace{\left[\begin{array}{c|c}
         \mathbf{a_1} & \mathbf{a_3} \\
         \mathbf{a_2} & \mathbf{a_4} \\
    \end{array}\right]}_{A^{(nz)}}
    \underbrace{\left[\begin{array}{cc}
         \mathbf{b_1}  \\
         \hline
         \mathbf{b_2} 
    \end{array}\right]}_{B}
    \xrightarrow[]{I\shortp{}}    \underbrace{\left[\begin{array}{cc}
         \mathbf{a_1 b_1} & \mathbf{0} \\
         \mathbf{0} & \mathbf{a_3 b_2} \\
         \mathbf{a_2 b_1} & \mathbf{0} \\
         \mathbf{0} & \mathbf{a_4 b_2} \\
    \end{array}\right] }_{C_{4\times d_n}}
\end{equation}


==> stile.tex <==
\subsection{The \stile{} Abstraction}\label{sec:stileabs}

We derive a new type of computation tile, called sparse tile \ie \stile{}, by applying \property{} on dense computation tile. An \stile{} is a group of non-redundant elements following a specific type of layout, associated with a dense computation tile. The non-redundant element is called the data tile which represents the sparsity granularity. The scattered data tiles can be condensed to be a dense tile. In reverse, a dense tile can correspond to different \stile{}s with different permutation functions. \autoref{fig:stile} shows four example \stile{}s associated with the same dense computation tile. Assuming the dense tile is $T_C=T_A*T_B$, whose shapes are $[4, 3]=[4, 5]*[5, 3]$. The \stile{} on the top left of \autoref{fig:stile} allows the rows of $T_A$ to be scattered in non-continuous rows of matrix $A$. The data tile of this \stile{} is the size of $T_A$'s one row (\ie $1\times5$), which can be seen as the effective sparsity granularity. The data tiles can be condensed to a dense tensor during loading from lower-level to upper-level memory (\eg from global memory to shared memory), then the computation is performed on the dense tile. Similarly, the data tile can be vertical in matrix $A$ (\ie $4\times1$) by applying a permutation function on $k$ dimension as shown on the top right of \autoref{fig:stile}. More aggressively, the data tile could become smaller like the bottom two \stile{}s in \autoref{fig:stile}, where both dimensions $m$ and $k$ have their own permutation function.

The design of \stile{} naturally decouples sparse data (\ie the data tiles) encoding/decoding and computation. The computation (\ie computation tile) operates on dense data without traditional sparse data indexes, which greatly improves computation efficiency. The preparation of the dense data happens on the fly during data movement across memory hierarchies.

\subsection{\stile{} Kernel Generation}\label{sec:stilegen}

\stile{} enables a new kernel skeleton of sparse computation, where the sparse computation is decomposed into the separated data rearrangement phase and the dense computation phase. We introduce two primitives \sload{} and \swrite{} for the data rearrangement. \sload{} maps sparse data tiles in input tensors to dense data block, while \swrite{} writes the output dense data block to the specified output data format, which could be sparse or dense. The kernel skeleton is shown in \autoref{fig:stile_kernel} in CUDA~\cite{cuda} style. \sload{} and \swrite{} are the additional overhead in the sparse kernel (line \ref{line:sparsekernel}) compared to the dense computation (line \ref{line:densecomp}). However, we can eliminate the overhead by leveraging the memory hierarchy of modern devices.

